CLIPLoss and Norm-Based Data Selection Methods for Multimodal Contrastive Learning

Data selection has emerged as a core issue for large-scale visual-language model pretaining (e.g., CLIP), particularly with noisy web-curated datasets. Three main data selection approaches are: (1) leveraging external non-CLIP models to aid data selection, (2) training new CLIP-style embedding models that are more effective at selecting high-quality data than the original OpenAI CLIP model, and (3) designing better metrics or strategies universally applicable to any CLIP embedding without requiring specific model properties (e.g., CLIPScore is one popular metric). While the first two approaches have been extensively studied, the third remains under-explored. In this paper, we advance the third approach by proposing two new methods. Firstly, instead of classical CLIP scores that only consider the alignment between two modalities from a single sample, we introduce surrogate-CLIPLoss (s-CLIPLoss), a CLIP loss-inspired method that adds the alignment between one sample and its contrastive pairs as an extra normalization term for better quality measurement. Secondly, when downstream tasks are known, we propose a new norm-based metric, NormSim, to measure the similarity between pretraining data and target data. We test our methods on the data selection benchmark, DataComp~\cite{gadre2023datacomp}. Compared to the best baseline using only OpenAI's CLIP-L/14, our methods achieve a 5.3\% improvement on ImageNet-1k and a 2.8\% improvement on 38 downstream evaluation tasks. Moreover, both s-CLIPLoss and NormSim are compatible with existing techniques. By combining our methods with the current best methods DFN and HYPE, we can boost average performance on downstream tasks by 0.9\%, achieving a new state-of-the-art on the DataComp-medium benchmark.

==> dmlr_icml_2024_content/abstract.tex <==
\begin{abstract}
% In recent years, data selection has emerged as a core issue for large-scale visual-language model pretraining, especially on noisy web-curated datasets. One widely adopted strategy assigns quality scores such as CLIP similarity for each sample and retains the data pairs with the highest scores. However, these approaches are agnostic of data distribution and always fail to select the most informative samples. 
% To solve this problem, we propose a simple yet theoretically principled metric named \textbf{V}ariance \textbf{A}lignment \textbf{S}core (\textsf{VAS}), which has the form $\langle \Sigma_{\text{test}}, \Sigma_i\rangle$.
% Here, $\Sigma_{\text{test}}$ represents the target (cross-)covariance matrix we aim to align, potentially based on prior knowledge, while $\Sigma_i$ denotes the tensor product of single or multi-modal representations for the $i$-th sample.
% We further design a new data selection method that maximizes the total \textsf{VAS}.
% We provide theoretical analysis in a simplified setting to demonstrate the theoretical advantage of \textsf{VAS} over random or other existing data selection.
% Experimentally, applying VAS and CLIP scores together can outperform baselines by a margin of $1.3\%$ average on 38 evaluation sets for noisy dataset DataComp and $2.5\%$ on VTAB for high-quality dataset CC12M. Additionally, our ablation study also shows visual features are better than text for calculating VAS, and the related classical experimental design methods may fail under this context.

\iffalse
In recent years, data selection has emerged as a core issue for large-scale visual-language model pretraining, especially on noisy web-curated datasets. Classical approaches to data selection have traditionally depended on the OpenAI pretrained CLIP model for computing CLIP scores or employed heuristic methods like semantic matching, both of which have shown only marginal improvements.   \yifang{TODO: subject to change} On the other hand, state-of-the-art data filtering methods involve using external models or high-quality multi-modal pairs to train more powerful models for data selection. While effective, these methods fail to fully exploit the potential of "less powerful information" accessible from the OpenAI CLIP model alone, leading to the suboptimal utilization of their own trained models. 

This research addresses such gaps by revisiting the classical methods and proposing a novel approach that replaces the CLIPScore with negCLIPLoss incurring almost no additional computation cost. We also introduce a highly efficient \normsim metric when downstream tasks prior are accessible. Our methods achieve close-to-SOTA results on the widely used DataComp benchmark even without leveraging those external resources used by existing SOTA methods -- compared with the best baseline that utilizes only OpenAI's CLIP, we achieve $6.0\%$ and $3.0\%$ improvement on ImageNet-1k and 38 downstream evaluation tasks.  More importantly, we emphasize that our proposed negCLIPLoss metric is universally applicable to any given CLIP embedding or data filtering model trained via more advanced methods. For example, by combining with SOTA Data filtering network methods \citep{fang2023data}, we further boost its average performance on downstream tasks by 1.0\%. This work highlights the need for universal data selection strategies that can effectively leverage all available information to improve multi-modal model performance.
\fi

\iffalse
Data selection has emerged as a core issue for large-scale visual-language model pretraining in recent years, especially on noisy web-curated datasets. 
A popular approach is to rely on OpenAI's pretrained CLIP model to score data and only include those examples that exceed a threshold. 
% or employing other heuristic methods offer only limited improvements. 
More recently proposed techniques have relied on  advanced external models or 
% high-quality multi-modal pairs to 
re-training more powerful teacher models which have shown to be effective, but require at least 10x more computational resources than calculating CLIP scores.
% \yifang{I delete things like "semantic matching" since its not important. I delete "larger computational cost than training" because it may confuse people why it is a problem. Not every know that "with enough computational resouce, we should choose all data"}
To address these challenges, this paper revisits the use of OpenAI CLIP-based methods. Firstly, classical quality measurement metrics like CLIP scores only consider the alignment between two modalities from the \textit{single sample}. Inspired by the loss function of CLIP, we propose a more robust metric called negCLIPLoss by adding the alignment between \textit{one sample and its contrastive pairs as a normalization term}, with negligible computational overhead. In addition,we introduce a highly efficient \normsim { }metric. 
% when downstream tasks prior are accessible. 
Combining these two techniques yields near-SOTA results on the DataComp benchmark, with comparable computation cost to computing the CLIP score, and surpassing the best OpenAI CLIP-based baseline by 5.3\% on ImageNet-1k and 2.8\% on average across 38 downstream tasks. By integrating with SOTA data filtering method (DFN)\citep{fang2023data}, we further boost its performance by an additional 1.0\% over using DFN alone. 
Crucially, negCLIPLoss, as a replacement to CLIP scores, is orthogonal to other approaches and therefore can be universally applied to any CLIP embedding-based methods.
\fi


\noindent Data selection has emerged as a core issue for large-scale visual-language model pretaining (e.g., CLIP), particularly with noisy web-curated datasets. Three main data selection approaches are: (1) leveraging external non-CLIP models to aid data selection, (2) training new CLIP-style embedding models that are more effective at selecting high-quality data than the original OpenAI CLIP model, and (3) designing better metrics or strategies universally applicable to any CLIP embedding without requiring specific model properties (e.g., CLIPScore is one popular metric).
% While the first two approaches have been extensively studied, the third remains under-explored. 
% In this paper, we advance the third approach by proposing a new loss function inspired quality-measuring metric, \textbf{negCLIPLoss} when only pre-training data is available, and a new target similarity measurement, {\textbf{\normsim}}, when downstream tasks are known. 
% Compared to classical CLIP scores which only consider the alignment between two modalities from the \textit{single sample}, negCLIPLoss adds the alignment between \textit{one sample and its contrastive pairs as an extra normalization term} to avoid systematic bias in individual sample. Furthermore, {\normsim} greedily maximize the similarity between pretraining set and target using norm-based metric.
% \simon{Add a sentence or two to describe these two methods.}
While the first two approaches have been extensively studied, the third remains under-explored. In this paper, we advance the third approach by proposing two new methods. Firstly, instead of classical CLIP scores that only consider the alignment between two modalities from a single sample, we introduce \textbf{negCLIPLoss}, a CLIP loss-inspired method that adds the alignment between one sample and its contrastive pairs as an extra normalization term for better quality measurement. Secondly, when downstream tasks are known, we propose a new norm-based metric, \textbf{\normsim}, to measure the similarity between pretraining data and target data.
We test our methods on the data selection benchmark, DataComp~\citep{gadre2023datacomp}.
Compared to the best baseline using only OpenAI's CLIP-L/14, our methods achieve a 5.3\% improvement on ImageNet-1k and a 2.8\% improvement on 38 downstream evaluation tasks. 
Moreover,
% our proposed \textbf{negCLIPLoss} metric is applicable to any new embeddings obtained from the second approach, and 
both \textbf{negCLIPLoss} and  {\textbf{\normsim}} are compatible with existing techniques. 
By combining our methods with the current best methods DFN~\citep{fang2023data} and HYPE~\citep{kim2024hype}, we can boost average performance on downstream tasks by 0.9\%, achieving a new state-of-the-art.
% For instance, by combining our selected data with the current SOTA method DFN~\citep{fang2023data} and HYPE~\citep{kim2024hype}, we can boost average performance on downstream tasks by an additional 0.9\%.



\end{abstract}

==> dmlr_icml_2024_content/conclusion.tex <==
\vspace{-1.2em}
\section{Conclusion and Reproducibility Statement}
\vspace{-0.5em}

In this paper, we introduce negCLIPLoss and {\normsim} to enhance data selection in multimodal contrastive learning without relying on external resources. negCLIPLoss provides a more accurate quality metric compared to the commonly used CLIPScore, while NormSim measures the similarity between pretraining data and target data for known downstream tasks. Experiments show that our method demonstrates both effectiveness (Table~\ref{tab: D1 compare}-\ref{tab: D2D3 compare}) and efficiency (Table~\ref{fig: compute cost}). Additionally, negCLIPLoss and {\normsim} are compatible with existing top techniques, allowing us to achieve a new state-of-the-art by combining them. All experiments are reproducible using code {\tt https://github.com/ypwang61/VAS/tree/negcliploss\_normsim}. 

% A notable limitation of our study is the exclusion of larger pretraining datasets, such as the large and xlarge scales of DataComp. However, DataComp-medium is the most commonly used benchmark for data selection in CLIP pretraining, and Future directions include exploring better ways to merge data selected by different methods and incorporating our methods into data scheduling scenarios.


% In this paper, we propose a new quality metric negCLIPLoss and a target similarity measure {\normsim}

% In the paper, we propose a Variance Alignment Score (VAS) to measure the informativeness of each sample and show that VAS is a parallel metric to image-text alignment focused score like CLIP score. Based on VAS, we design a informative + quality focused strategy that achieves the best average performance over 38 downstream test tasks compared to various existing baseline. Moreover, we also provide a theoretical guarantees to explain the intuition behind our strategy.

==> dmlr_icml_2024_content/experiment_results.tex <==


% \begin{table}[h]
% \centering
% \caption{}
% \label{tab:example}
% \begin{tabular}{|c|c|}
% \hline
% \multirow{2}{*}{yyc} & 1 \\ \cline{2-2}
%  & 2 \\ \hline
% 3 & 4 \\
% \hline
% \end{tabular}
% \end{table}




\vspace{-0.8em}
\section{Experimental Results}
\vspace{-0.8em}
\label{sec: experiment}
In this section, we evaluate the performance of negCLIPLoss and NormSim, aiming to address the following questions:
\textbf{Q1:} Given a fixed CLIP teacher model, can our methods more effectively utilize CLIP embeddings for data filtering?
\textbf{Q2:} Are our methods applicable to diverse CLIP teacher models with varying architectures or different pretrained datasets?
\textbf{Q3:} 
How does our method compare to other leading approaches that utilize external models or multimodal datasets? Could our method be compatible with these methods?

% Compared to prior approaches that employ external models or multimodal datasets, could our method behave
% can our methods further enhance filtering performance? Specifically, are external resources necessary, or can similar benefits be achieved without them? If necessary, are our methods compatible with those approaches?
\vspace{-0.8em}
\subsection{Setup}
\vspace{-0.5em}
We adhere to the standardized training and evaluation protocols of the DataComp benchmark~\citep{gadre2023datacomp}.
% , which fixes the CLIP training pipeline and aims to select a subset from the given training pool to maximize the model performance. 
% Details are as follows. 
% .
% \textbf{Training configuration.} 
We employ the medium-scale training configuration of DataComp (DataComp-medium). It provides a substantial dataset comprising 128 million low-quality, web-curated image-text pairs to be filtered. Once the data subset is obtained by some data filtering strategy, it will be used to train a fixed CLIP-B/32 model in a fixed training budget that allows the model to pass 128 million data points an epoch. Therefore, smaller subsets will be repeated more frequently, ensuring a fair comparison.
We note that the size of the DataComp dataset becomes smaller over time since some URLs of images become invalid\footnote{See https://github.com/mlfoundations/datacomp/issues/3 and similar issues in \cite{maharana2023d2}.
}, and we only successfully downloaded about 110M data. Therefore, the results of baselines on the leaderboard do not apply to our datasets. So we reproduce top baselines on the leaderboard with their public UIDs of the selected data\footnote{The results of MLM~\citep{wang2024finetuned} are from their paper.}. More details about evaluation tasks and architecture are in Appendix~\ref{supp: sec detail setup}.

% \yifang{Talk about how we merge new data from large ...}


\iffalse
\subsection{Baselines}
\label{sec:baselines}
% \yiping{I wonder if we can let it be a single section. I think this kind of classification is also an interesting part for reader to get the lines of works.}
Recall that we previously identified three main research directions: \simon{this order is different from what we use in the intro.} (D1) using OAI CLIP alone while optimizing embedding employment strategies, (D2) training and using a more advanced CLIP embedding model based on external data, and (D3) utilizing non-CLIP external models to aid data selection. It's important to note that D2 and D3 may also incorporate strategies from D1. For example, CLIPScore (D1) has been used in almost all the top methods. Therefore, we categorize baselines by the largest possible category they encompass and further separate them according to their demand on target downstream tasks and external resources as follows.
% 
Specifically, D1 can be further divided based on whether knowledge of target downstream tasks is known or not. From a practical perspective, D2 and D3 can be regarded as different ways of using models or data outside the resources provided by DataComp. Please refer to Appendix~\ref{sub: baselines} for details.
\simon{can shorten this paragraph if necessary}\yiping{will fix this after fixing intro}
% Recall that there are three main research directions as we stated before: (D1) Use OAI CLIP only while optimizing embedding employment strategies. (D2) Train and use a more advanced CLIP embedding model based on external data. (D3) Utilize nonCLIP external models to aid data selection.
% We mention that {D2 and D3 may also use strategies in D1}, for example, \textit{CLIPScore (D1)} mentioned before \textit{has been used in almost all the top methods}. Therefore, we mark baselines with the largest possible category. \yiping{Double check if we can say it like this.}
% as an initial filtering. \yiping{initial filtering is not accurate for dfn and t-mars}

% Based on these three directions, we further separate our baseline into the following categories according to their demand on target downstream tasks and external resources as follows.
% Specially, D1 can be further divided into whether knowledge of target downstream tasks is known or not. The latter D2 and D3, from a practical perspective, can all be regarded as different ways of using models or data outside the resources provided by DataComp. Please refer to Appendix~\ref{sub: baselines} for details.

\textbf{D1: OAI CLIP embedding only.} The learner can only access the pretrained training set, training data of target downstream task, and the original OAI CLIP teacher model that is used to extract embeddings, without using any existing external models or a newly trained CLIP model based on external multi-modal data. Under this setting, we can further separate the baseline into
\begin{itemize}[leftmargin=*]
\vspace{-8px}
    \item \textbf{C1: No target task knowledge is available.} 
    % When only the training set is accessible, we compare our method with 
    % This category includes (1) \textbf{Rule-based methods}, which filters data based on heuristic rules like text length (e.g., more than 2 words or 5 characters.), frequency of texts (e.g., occurring less than 1000 times), or image size (e.g., aspect ratio in $[0.33, 3.33]$). The last two rules are adopted by \textbf{Devil}~\citep{yu2023devil}. (2) \textbf{CLIPScore}, which selects the data with the top image-text similarity calculated by the CLIP embeddings generated from the teacher model.
    % (3) \textbf{$\mathbb{D}^2$ Pruning}~\citep{maharana2023d2}, which represents the dataset as an undirected graph and selects the data by combining difficulty and diversity. They use the CLIP score to initialize their graph.
    This category includes (1) \textbf{CLIPScoreOnly}, which only uses CLIPScore as we mentioned before.
    % selects the data with the top image-text similarity calculated by the CLIP embeddings generated from the teacher model. Notice that CLIPScore has also been \textit{used in almost all the top methods} as an initial filtering.
    % , except the Image-based filtering.
    (2) \textbf{$\mathbb{D}^2$ Pruning}~\citep{maharana2023d2}, which represents the dataset as an undirected graph and selects the data by combining difficulty and diversity. They use the CLIP score to initialize their graph. (3) Rule-based methods, which filter data based on heuristic rules like text length, frequency of texts, or image size. Rule-based techniques are less effective when used alone so we will not compare with them here.  
\vspace{-2px} 
    \item \textbf{C2: Knowledge of downstream task is available.} 
    % Incorporating downstream target data is a widely used approach for data filtering.An example is \textbf{Image-based filtering} proposed in DataComp~\citep{gadre2023datacomp}. It uses the training data of ImageNet-1K as target data, first runs the k-means algorithm to cluster the image embeddings of DataComp training data, and then selects the clusters closest to one of the image embeddings of ImageNet-1K target data. Another method is \textbf{(CIDS)}, which is integrating into \textbf{Devil}~\citep{yu2023devil}. It 
    % follows a similar idea of Image-based filtering to estimate the importance of each cluster, and it uses all available 22 training sets from downstream tasks as target data instead of ImageNet only. It's worth saying that the number of all available downstream training data is always only about 2M, which is much less than the training set size of DataComp-medium (128M) or other external datasets like HQITP-350M.
    Leveraging downstream target training data, whose size is much smaller than the pretraining data set, is widely used in data filtering. This category includes (1) \textbf{Image-based filtering} proposed in \citep{gadre2023datacomp}, which uses ImageNet-1K training data as the target. It applies k-means clustering to the image embeddings of training data and selects clusters closest to the ImageNet-1K embeddings. (2) CIDS, integrated into Devils~\citep{yu2023devil}, uses a similar cluster-based approach but targets all 22 training sets from downstream tasks instead of just ImageNet-1K.
    Since Devils also includes external models, we will put it into D3 category 
    \underline{not compare} with it in this category. \simon{but we compare them in 4.3.3?}
    % It's worth saying that the total available downstream training data amounts to only about 2M, which is significantly smaller than the dataset sizes of DataComp-medium (128M) and other external datasets like HQITP-350M.
\vspace{-16px}
\end{itemize}
% \yiping{working on this...}
\vspace{1em}
\textbf{D2, D3: Accessible external model and multi-modal data.} All the current top baselines enable the learner to utilize external resources, either to train a better CLIP teacher model or to help filtering using existing models' properies. In detail, 
% (1) \textbf{Text-based filtering}~\citep{gadre2023datacomp} selects only English captions (according to language detector fasttext~\citep{joulin2016bag}) that contain words from ImageNet-21K class synsets. 
(1) \textbf{DFN}~\citep{fang2023data} which trains another CLIP data filtering network via external high-quality data. Their currently public model (\textbf{DFN-P}) is trained on CC12M~\citep{changpinyo2021conceptual12} + CC3M~\citep{sharma2018conceptual3} + SS15M~\citep{nguyen2022quality}, while the best DFN is trained on nonpublic HQITP-350M~\citep{fang2023data}. 
(2) \textbf{HYPE}~\citep{kim2024hype} which leverages hyperbolic embeddings (different from CLIP embedding) and the concept of entailment cones to filter out samples with meaningless or underspecified semantics, enhancing the specificity of each sample.
(3) \textbf{HYPE} $\cup$ \textbf{DFN} proposed by \citep{kim2024hype}, which samples subset separately for each method and then merge them with duplication.
(4) Other methods including \textbf{T-MARS}~\citep{maini2023t}, \textbf{Devils}~\citep{yu2023devil}, \textbf{MLM}~\citep{wang2024finetuned}, which leverage external models such as FAST~\citep{chen2021fast}, BLIP-2~\citep{li2023blip} and LLaVA-1.5~\citep{liu2023improved,chiang2023vicuna} to heuristically select the more helpful data like non-text-only pictures or images with MNIST-style digits.\simon{why non-helpful?}\yiping{fixed} (Details in \yifang{cite}.)
% (3) \textbf{T-MARS}~\citep{maini2023t} uses a text detection model like FAST~\citep{chen2021fast} to filter out the data that only contain the texts of caption in the image and don't have other useful image features.  
% (3) \textbf{Devils}~\citep{yu2023devil} adopts lots of heuristic methods including removing non-English captions and using the external image-captioning model BLIP-2~\citep{nguyen2024improving} to recognize the digit. It also adopts rule-based methods and CIDS as we talked before.
% (4) \textbf{MLM}~\citep{wang2024finetuned} prompts GPT-4V to construct instruction data and use it to fine-tune a vision-language model like LLaVA-1.5~\citep{liu2023improved, chiang2023vicuna} into a filtering network.
\fi
\vspace{-0.8em}
\subsection{Baselines}
\label{sec:baselines}
\vspace{-0.5em}
% \simon{can shorten this paragraph if necessary}\yiping{rewrite it, you can check it}
We restate the three current research directions mentioned before based on how much external resources are employed: 
% \simon{this order is different from what we use in the intro.}\yiping{Change the sentence, is it ok?} 
(D1) using OAI CLIP alone while optimizing embedding employment strategies, (D2) training and using a more advanced CLIP embedding model based on external data, and (D3) utilizing non-CLIP external models to aid data selection\footnote{Note that D2 and D3 may also incorporate strategies from D1. For example, CLIPScore (D1) has been used in almost all the top methods. Therefore, we categorize baselines by the largest possible category they encompass.}. 
% and further separate them according to their demand on target downstream tasks and external resources as follows.
% 
% Specifically, D1 can be further divided based on whether knowledge of target downstream tasks is known or not. 
% From a practical perspective, D2 and D3 can be regarded as different ways of using models or data outside the resources provided by DataComp. Please 
In our experiment parts, we consider baselines following the above categorization: \underline{\textbf{(1) D1}}, including 
\textbf{CLIPScore}~\citep{hessel2021clipscore}, \textbf{Image-based filtering}~\citep{gadre2023datacomp}, \textbf{$\mathbb{D}^2$ Pruning}~\citep{maharana2023d2}.
\underline{\textbf{(2) D2, D3}}, including 
\textbf{DFN}~\citep{fang2023data},
\textbf{HYPE}~\citep{kim2024hype},
\textbf{HYPE} $\cup$ \textbf{DFN} (previous state-of-the-art), \textbf{T-MARS}~\citep{maini2023t}, \textbf{Devils}~\citep{yu2023devil}, and \textbf{MLM}~\citep{wang2024finetuned}.
Please refer to Fig.~\ref{sup fig: ill d}, Appendix~\ref{supp: ill d}, and Appendix~\ref{sub: baselines} for more details.
% We make these separations for fair comparison. 
Intuitively, performance should be ranked as 
\textbf{D2, D3} > \textbf{D1}. 
However, our results show that cross-setting comparisons are possible and our D1 methods can perform similar or even better than most of D3 methods.
% \yiping{TODO: add baselines}

% Recall that there are three main research directions as we stated before: (D1) Use OAI CLIP only while optimizing embedding employment strategies. (D2) Train and use a more advanced CLIP embedding model based on external data. (D3) Utilize nonCLIP external models to aid data selection.
% We mention that {D2 and D3 may also use strategies in D1}, for example, \textit{CLIPScore (D1)} mentioned before \textit{has been used in almost all the top methods}. Therefore, we mark baselines with the largest possible category. \yiping{Double check if we can say it like this.}
% as an initial filtering. \yiping{initial filtering is not accurate for dfn and t-mars}

% Based on these three directions, we further separate our baseline into the following categories according to their demand on target downstream tasks and external resources as follows.
% Especially, D1 can be further divided into whether knowledge of target downstream tasks is known or not. The latter D2 and D3, from a practical perspective, can all be regarded as different ways of using models or data outside the resources provided by DataComp. Please refer to Appendix~\ref{sub: baselines} for details.


\iffalse
\paragraph{Accessible external resources} Here we allow the learner to leverage the external resources to either train a better CLIP teacher model or to detect specific elements in data for more fine-grained filtering. Under this setting, we compare our method with (1) \textbf{DFN} which trains another CLIP data filtering network via external high-quality data (2) \textbf{T-MARS} which filters out the data whose text is the only feature correlated with the49
caption using FAST  (3) \textbf{MLM} which use carefully designed GPT prompt data to build a vision-language model as a filtering network. (4) \textbf{Devils} which adopts a lot of heuristic methods including using external image-captioning model BLIP-2 to recognize the digit and language detector fasttext~\citep{joulin2016bag} to remove non-English text. Notably, \textbf{DFN} is the current state-of-art that we will mainly compete with.
\fi


% \textbf{Cross-setting comparison .} We make these separations for fair comparison because, intuitively, performance should be ranked as \textbf{External-resources-accessible} > \textbf{Downstream-task-aware} > \textbf{Only-trainset-available} \yiping{maybe \textbf{External-resources-accessible} > \textbf{OAI CLIP only}?}, while the cost for data preprocessing and new model training is the opposite. However, our results show that cross-setting comparisons are possible and our "no-external-resources-used" methods \yiping{I guess someone may argue that target data is also external resources..., maybe prevent use `resources'?} can perform similarly to or even better than those using external resources.

\begin{table*}[t]
\small
\centering
\vspace{-1.4em}
\caption{
Results on DataComp-medium from methods that use only OpenAI's CLIP-L/14 model, i.e., all methods are from the \textbf{D1} category. The ``dataset size'' represents the size of the subset obtained from different approaches.
{\normsim}(IN-1k) denotes using the training data of ImageNet-1k as the target while {\normsim}(Target) represents using that of all 24 available downstream tasks. Complete Results in Appendix~\ref{supp: sec D1 complete}.
% \yiping{maybe need mention {\normsimD} in the main part}
} 
\label{tab: D1 compare}
\vspace{-0.6em}
\label{tab:OAI_only_L14_result}
\centering
\begin{tabularx}{\textwidth}{@{}l@{\hskip 8pt}c@{\hskip 8pt}c@{\hskip 8pt}c@{\hskip 8pt}c@{\hskip 8pt}c@{\hskip 8pt}c@{}}
% \small
\toprule
\multirow{2}{*}{\textbf{Filtering Strategy}} & \textbf{Dataset} & \textbf{IN-1k} & \textbf{IN Shift} & \textbf{VTAB} & \textbf{Retr.} & \textbf{Avg.} \\
 & \textbf{Size} & (1 task) & (5) & (11) & (3) & (38)\\
\midrule
No filtering~\citep{gadre2023datacomp} & 110M & 17.3 & 15.0 & 25.2 & 21.3 & 25.6 \\
CLIPScore (20\%)~\citep{hessel2021clipscore} & 22M & 25.4 & 22.7 & 31.8 & 22.0 & 31.0 \\
CLIPScore (30\%)~\citep{hessel2021clipscore} & 33M & 26.4 & 23.6 & 32.6 & 24.5 & 32.2 \\
Image-based~\citep{gadre2023datacomp} & 24M & 25.5 & 21.9 & 30.4 & 24.6 & 29.9 \\
CLIPScore (30\%) $\cap$ Image-based & 11M & 27.4 & 23.9 & 31.9 & 21.4 & 30.8\\
$\mathbb{D}^2$ Pruning~\citep{maharana2023d2} & 22M & 23.2 & 20.4 & 31.4 & 18.7 & 29.5\\
\midrule
negCLIPLoss (20\%) & 22M & 27.4 & 23.8 & 33.7 & 23.7 & 32.5\\
negCLIPLoss (30\%) & 33M & 27.9 & 24.6 & 33.2 & 25.1 & 32.9\\
% \midrule
% CLIPScore (30\%) $\cap$ \twonormsimD & 22M & 28.3 & 25.0 & 34.5 & 22.7 & 32.9\\
% % negCLIPLoss (30\%) $\cap$ \twonormsimD & 22M & 28.9 & 25.5 & 34.1 & 23.3 & 33.2\\
% negCLIPLoss (30\%) $\cap$ \twonormsimD & 22M & 29.8 & 26.1 & 34.8 & 24.6 & 34.1\\
\midrule
% CLIPScore (30\%) $\cap$ \twonormsim(IN-1k) & 22M & 29.1 & 25.4 & \underline{35.8} & 24.1 & 33.4\\
% CLIPScore (30\%) $\cap$ \twonormsim(Target) & 22M & 28.9 & 25.1 & 32.7 & 23.6 & 32.5\\
CLIPScore (30\%) $\cap$ \infnormsim(IN-1k) & 22M & 29.7 & 25.9 & 33.7 & 24.1 & 33.7\\
CLIPScore (30\%) $\cap$ \infnormsim(Target) & 22M & 30.2 & 26.2 & 35.0 & 23.4 & 33.9\\
\midrule
% negCLIPLoss (30\%) $\cap$ \twonormsim(IN-1k) & 22M & 30.4 & 26.4 & 35.4 & \underline{25.6} & 34.3\\
% negCLIPLoss (30\%) $\cap$ \twonormsim(Target) & 22M & 30.6 & 26.2 & 35.2 & 25.5 & 33.9\\
negCLIPLoss (30\%) $\cap$ \infnormsim(IN-1k) & 22M & \textbf{31.9} & \textbf{27.3} & 34.8 & 25.0 & \underline{34.4}\\
negCLIPLoss (30\%) $\cap$ \infnormsim(Target) & 22M & \underline{31.7} & \underline{27.2} & \textbf{36.0} & \textbf{26.0} & \textbf{35.0}\\
\bottomrule
\end{tabularx}
% \vspace{0.1em}
% \caption*{(a) C1: No target knowledge is available.}
\vspace{-1.8em}
\end{table*}
% \textbf{Cross-setting comparison.} 
% \textbf{External-resources-accessible} > \textbf{Only-OAI-CLIP-available} and \textbf{Downstream-task-aware} > \textbf{Only-trainset-available}.
% while the cost of data preprocessing and new model training is higher. \yiping{maybe not needed here?}
\vspace{-1.0em}
\subsection{Main Results and Discussions}
% \begin{table*}[ht]
% \small
% \centering
% \vspace{-1em}
% \caption{Results on DataComp-medium from the top methods that use only OpenAI's CLIP-B/32 model or public version of DFN (DFN-P). 
% % Here in the DFN-P part, since utilizing DFN-P embedding to calculate {\infnormsim} performs suboptimal, we also try OpenAI's B-32 for calculating {\infnormsim} and denote it as `$\text{NormSim}_{\infty}^{\text{B/32}}$'.
% \yiping{Still working on DFN-P...}
% % For DFN-P, we set the subset size as $17.5\%$ and $15\%$
% }
% \label{tab: cliploss unversality}
% % \vspace{0.3em}
% \label{tab:OAI_combined_result}
% % \begin{tabularx}{}{@{}lcccccl@{}}
% \begin{tabularx}{1.0\textwidth}{@{}l@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}l@{}}
% \toprule
% % \textbf{Filtering Strategy} & \textbf{Dataset Size} & \textbf{IN-1k} & \textbf{IN Dist. Shift} & \textbf{VTAB} & \textbf{Retrieval} & \textbf{Average} \\
% \multirow{2}{*}{
% \textbf{\textbf{OAI CLIP-B/32}}} & \textbf{Dataset} & \textbf{IN-1k} & \textbf{IN Dist. Shift} & \textbf{VTAB} & \textbf{Retrieval} & \textbf{Avg.} \\
%  & \textbf{Size} & (1 sub-task) & (5) & (11) & (3) & (38)\\
% \midrule
% % \multicolumn{7}{l}{\textbf{CLIP-B/32}} \\
% % \textbf{OAI CLIP-B/32} & & & & & & \\
% CLIPScore (20\%) & 22M & 27.0 & 23.8 & 33.0 & 22.9 & 32.2 \\
% CLIPScore (30\%) & 33M & 27.6 & 24.2 & 33.6 & 25.1 & 33.3 \\
% \midrule
% negCLIPLoss (20\%) & 22M & 28.9 & 24.8 & 34.3 & 24.3 & 33.0\\
% negCLIPLoss (30\%) & 33M & 28.8 & 25.1 & 33.7 & 26.6 & 33.6\\
% % negCLIPLoss (30\%) $\cap$ \twonormsim(IN-1k) & 22M & & & & & \\
% \midrule
% negCLIPLoss (30\%) $\cap$ \infnormsim(Target) & 22M & \textbf{32.4} & \textbf{27.4} & \textbf{35.9} & \textbf{26.3} & \textbf{35.2}\\
% \bottomrule
% \toprule
% \textbf{DFN-P} & & & & & & \\
% \midrule
% % \multicolumn{7}{l}{\textbf{CLIP + DFN-P (CLIP-B/32)}} \\
% % CLIPScore (15\%) & & & & & & \\
% CLIPScore (17.5\%) & 19M & 30.2 & 26.8 & 34.1 & 26.5 & 33.8 \\
% CLIPScore (20\%) & 22M & 29.7 & 26.8 & 33.0 & 27.0 & 33.1 \\
% % maybe rerun clipscore 20
% CLIPScore (30\%) & 33M & 28.4 & 24.7 & 33.2 & 26.8 & 32.7\\
% \midrule
% % negCLIPLoss (15\%) & & & & & & \\
% negCLIPLoss (17.5\%) & 19M & \textbf{31.2} & \textbf{27.5} & \textbf{35.7} & 27.0 & \textbf{34.7}\\
% negCLIPLoss (20\%) & 22M & 30.7 & 27.4 & 33.6 & \textbf{27.5} & 33.8\\
% negCLIPLoss (30\%) & 33M & 28.9 & 25.5 & 33.4 & 27.3 & 33.2\\
% % negCLIPLoss (30\%) $\cap$ \twonormsim(IN-1k) & 19M & & & & & \\
% \midrule
% negCLIPLoss (30\%) $\cap$ \infnormsim(Target) & 22M & 29.4 & 23.6 & 33.5 & 24.2 & 32.5 \\
% % negCLIPLoss (17.5\%) $\cap$ \infnormsim(Target) & & & & & & \\
% % negCLIPLoss (17.5\%) $\cap$ $\text{NormSim}_{\infty}^{\text{B/32}}$(Target) & & & & & & \\
% \bottomrule
% \end{tabularx}
% \vspace{-1em}
% \end{table*}

% \textit{Finally}, for the choice of target data, if you use {\twonormsim}, then ImageNet-1k is a better choice than all 24 downstream tasks, while the opposite holds if use {\infnormsim}. The reason may be that {\twonormsim} serves as principal component selection, which requires target data to be more balanced to provide better target variance estimation, while {\infnormsim} relies less on the balance of target distribution, and thus in general the more target data, the better it can achieve.\yiping{will this be confusing?} \yifang{Hmmm yea a little confusing..}
% ImageNet-1k can  for 

\subsubsection{D1 Category (Q1)}
% \textbf{Answer to Q1: Our methods leverage OAI CLIP-L/14 better.} 
\vspace{-0.5em}
In Table~\ref{tab: D1 compare}, we compare D1 methods where only the OAI CLIP model is allowed to be used.
We show that \textbf{our Methods leverage OAI CLIP-L/14 better.}
\textit{First}, negCLIPLoss outperforms CLIPScore on \emph{all metrics}, regardless of whether it is used alone or combined with other methods. These results support our claim that negCLIPLoss can more accurately estimate the data quality. \textit{Second}, when target knowledge is available, {\infnormsim} can further improve filtering  significantly. 
Especially, compared with the best baseline ``CLIPScore (30\%)'', our ``negCLIPLoss $\cap$ \infnormsim(Target)'' improves \textbf{5.3\%} on \textbf{ImageNet-1k} and \textbf{2.8\%} on average \textbf{38 downstream tasks}, respectively. 
Later in Table~\ref{tab: D2D3 compare} we will see that this result outperforms all the D3 baselines except DFN $\cup$ HYPE. And we can also see that using ImageNet-1k-only target data can still produce good results. 

\begin{wraptable}{ht}{0.5\textwidth}
\small
\vspace{-3.0em}
\caption{Results on DataComp-medium from the top methods that use only OpenAI's CLIP-B/32 model or public version of DFN (DFN-P). 
% ``$\text{NormSim}_{\infty}^{\text{B/32}}$'' represents using OAI CLIP-B/32 to calculate {\infnormsim}.
}
\vspace{-1.8em}
\label{tab: cliploss unversality}
\begin{center}
\setlength{\tabcolsep}{1.6mm}{\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
% \textbf{Filtering} & \textbf{Subset} & \multirow{2}{*}{\textbf{IN-1k}} & \multirow{2}{*}{\textbf{VTAB}} & \multirow{2}{*}{\textbf{Avg.}}\\
\textbf{Strategy} & \textbf{Size} & \textbf{IN-1k} & \textbf{VTAB} & \textbf{Avg.}\\
\midrule
\textbf{OAI CLIP-B/32} \\
\midrule
CLIPScore (20\%) & 22M & 27.0 & 33.0 & 32.2\\
CLIPScore (30\%) & 33M & 27.6 & 33.6 & 33.2\\
\midrule
negCLIPLoss (20\%) & 22M & 28.9 & 34.3 & 33.0\\
negCLIPLoss (30\%) & 33M & 28.8 & 33.7 & 33.6\\
\midrule
negCLIPLoss (30\%) & \multirow{2}{*}{22M} & \multirow{2}{*}{\textbf{32.4}} & \multirow{2}{*}{\textbf{35.9}} & \multirow{2}{*}{\textbf{35.2}} \\
$\cap$ \infnormsim(Target) & & \\
\bottomrule
\toprule
\textbf{DFN-P} \\
\midrule
CLIPScore (15\%) & 16M & 25.9& 32.9& 31.6 \\
CLIPScore (17.5\%) & 19M & 30.2 & 34.1 & 33.8\\
CLIPScore (20\%) & 22M & 29.7 & 33.0 & 33.1\\
CLIPScore (30\%) & 33M & 28.4 & 33.2 & 32.7\\
\midrule
negCLIPLoss (15\%) & 16M & \underline{31.3} & \underline{35.8} & 34.6 \\
negCLIPLoss (17.5\%) & 19M & {31.2} & {35.7} & \underline{34.7}\\
negCLIPLoss (20\%) & 22M & 30.7 & 33.6 & 33.8\\
negCLIPLoss (30\%) & 33M & 28.9 & 33.4 & 33.2\\
\midrule
negCLIPLoss (30\%) & \multirow{2}{*}{22M} & \multirow{2}{*}{29.4} & \multirow{2}{*}{33.5} & \multirow{2}{*}{32.5} \\
$\cap$ \infnormsim(Target) & & \\
negCLIPLoss (17.5\%) & \multirow{2}{*}{16M} & \multirow{2}{*}{\textbf{31.6}} & \multirow{2}{*}{\textbf{37.2}} & \multirow{2}{*}{\textbf{35.7}}\\
 $\cap$ $\text{NormSim}_{\infty}^{\text{B/32}}$(Target) & & \\
\bottomrule
\end{tabular}
}
\vspace{-3em}
}
\end{center}
\end{wraptable}

% \textit{Second}, even when target knowledge is unavailable, use {\twonormsimD} together with negCLIPLoss can still improve the filtering performance by 1.9\% on average 38 downstream tasks.







\iffalse
\vspace{-1em}
\subsubsection{Try Other Teacher Models (Q2)}
\vspace{-0.6em}
% \textbf{Comparison and Setup.} 
To evaluate whether our method applies to other CLIP teacher models, we replaced OAI CLIP-L/14 with OAI CLIP-B/32 and DFN-P as embedding models. We compare the best baseline ``CLIPScore'' with our ``negCLIPLoss'' and best strategy ``negCLIPLoss $\cap$ {\infnormsim}(Target)'' as shown in Table~\ref{tab: cliploss unversality} and Appendix~\ref{supp: universality }. Note that the original DFN paper selects a subset comprising 19.2M data points, which accounts for approximately $17.5\%$ of the dataset we downloaded, we incorporate the same ratio into our comparison. 
% We have the main conclusions are as follows.


\textbf{negCLIPLoss can be applied to different CLIP embedding models.}
Our proposed negCLIPLoss, as a replacement of CLIPScore, not only leads to better performance compared to all the other baselines using OAI CLIP-L/14 as shown in Table~\ref{tab: D1 compare}, but also achieves universal improvement on the other two CLIP embedding models, OAI CLIP-B/32 and DFN-P as shown in Table~\ref{tab: cliploss unversality}. 
For different filtering ratios and models, our methods can consistently outperform all downstream tasks, like a 0.5\%-1.9\% increase on ImageNet-1k. 



\textbf{Embedding required by {\normsim} should have good downstream performance.} 
When combining negCLIPLoss with {\infnormsim}, OAI CLIP-B/32 and DFN-P have completely different behaviors. The former obtains results even better than that in Table~\ref{tab: D1 compare} which uses OAI CLIP-L/14 as the teacher model, while DFN-P achieves results even worse than using negCLIPLoss alone. The reason is that, unlike OAI CLIP-B/32, DFN-P is specially designed for data filtering \textit{at the expense of the downstream task performance}, as claimed by its author.  (e.g., the ImageNet-1k accuracy for DFN-P, OAI CLIP-B/32, and OAI CLIP-L/14 are 45\%, 63\%, and 75\%, respectively). This indicates that the embedding obtained from DFN on target data might be highly unreliable, leading to inaccurate similarity calculations between training and target data. A future direction worth exploring is utilizing a better CLIP teacher model for calculating {\normsim}.
\fi

\vspace{-0.8em}
\subsubsection{Universality (Q2)}
\vspace{-0.6em}
% \textbf{Comparison and Setup.} 
To evaluate whether our method applies to other CLIP teacher models, we replaced OAI-L/14 with OAI-B/32 and DFN-P as embedding models. Results are in Table~\ref{tab: cliploss unversality} and Appendix~\ref{supp: universality }.\footnote{The original DFN paper selects a subset comprising 19.2M data points, which accounts for approximately $17.5\%$ of our dataset and $15\%$ of their dataset, we incorporate these sampling ratios into our comparison.} We conclude that
% We have the main conclusions are as follows.
\textbf{(1) negCLIPLoss can be applied to different CLIP embedding models.}
Our proposed negCLIPLoss can consistently outperform CLIPScore on all downstream tasks for different filtering ratios and models, like a 0.5\%-5.4\% increase on ImageNet-1k. 
\textbf{(2) Embedding required by {\normsim} should have good downstream performance.} 
When combining negCLIPLoss with {\infnormsim}, OAI-B/32 obtains results even better than those using OAI-L/14 (Table~\ref{tab: D1 compare}), while DFN-P achieves results even worse than using negCLIPLoss alone. The reason is that, unlike OAI CLIP, DFN-P is specially designed for data filtering \textit{at the expense of downstream task performance}\footnote{For example, the ImageNet-1k accuracy for DFN-P, OAI CLIP-B/32, and OAI CLIP-L/14 are 45\%, 63\%, and 75\%, respectively.}. This indicates that the embeddings obtained from DFN on target data might be highly unreliable, leading to inaccurate {\normsim}. Furthermore, if we use DFN-P for negCLIPLoss but OAI-B/32 for {\normsim} ("negCLIPLoss (17.5\%) $\cap$ $\text{NormSim}_{\infty}^{\text{B/32}}$(Target)"), we can achieve the best results. 
% Its average performance on 38 tasks is even higher than utilizing the best DFN (trained on HQITP-350M) with CLIPScore, as shown in Table~\ref{tab: D2D3 compare}.
% A future direction worth exploring is utilizing a better CLIP teacher model for calculating {\normsim}.


% \yifang{Change the words, please check}

% On the other hand, {\normsim} aims to measuring the similarity between training data and target data, from a wide range of categories, and thus requires a strong downstream performance for correctly assigning similarity score. Therefore, DFN-P fails to be used in {\normsim}. Nevertheless, if the embedding model is not specifically designed for data selection, then {\normsim} can still give consistent improvement as OAI CLIP-B/32.

% We believe that since DFN-P rarely sees some low-quality data during training, it's not as robust as the OAI CLIP model on noisy data, and thus will give low CLIPScore (or negCLIPLoss) on them

% \yifang{double check after running all the experiments} In addition, \yifang{TODO: see the result of DFN, it is not good we say that, if embedding model is not specifically designed for data selection, then norsim also give consistent performance blabla}

\vspace{-0.4em}

\subsubsection{Comparison with D2 \& D3 Categories (Q3)}
\vspace{-0.4em}
\label{sec: D2 D3}
In this part, we compare all the D2 \& D3 baselines mentioned in Sec.~\ref{sec:baselines} together with our best strategy in Table~\ref{tab: D2D3 compare}.
\footnote{For ``A $\cup$ B'' mentioned in Table~\ref{tab: D2D3 compare}, we follow the way of Kim et al.~\citep{kim2024hype} to merge the data, which generates the subset separately for each method and then merge them. This will result in oversampling the shared data, which is intuitively more important. 
% For the dataset size of ``A$\cup$B'', we count the number of the unique data in the dataset followed HYPE~\citep{kim2024hype}.
} We claim:
\vspace{-0.2em}
\textbf{(1) Our methods can outperform most of the D3 methods.}
In Table~\ref{tab: D2D3 compare}, we show that without using any external models or data, our best combination, i.e., using OAI-B/32 for ``negCLIPLoss (30\%) $\cap$ {\infnormsim}(Target)'' (\textbf{Ours (20\%)}), still outperforms all methods except DFN and ``DFN $\cup$ HYPE''. This answers the first part of Q3 and further indicates that some external models may be redundant since CLIP embeddings already contain necessary information.
\textbf{(2) We can further improve the SOTA method.} 
% On the other hand, training a data-selection-specific model like DFN still provides complementary benefits compared to our methods (like in Table~\ref{tab: cliploss unversality}). 
We can further boost the performance of the current SOTA method ``HYPE $\cup$ DFN'' by 0.9\% on both ImageNet-1k and on average 38 downstream tasks, and close results can be achieved even without combining HYPE which utilizes the external embedding model MERU~\citep{desai2023hyperbolic}.
Here we use the data selected by both OAI-B/32 and L/14, which we found is more robust than using one of them alone. 
Our better results answer the second part of Q3, that is, our methods can be compatible with other D2\&D3 methods. 

\begin{table*}[t]
\small
\centering
\vspace{-1.2em}
\caption{Results of all D1\&D2\&D3 top methods on DataComp-medium. 
``Ours (20\%)'' refers to use ``negCLIPLoss (30\%) $\cap$ \infnormsim(Target)'' to get 20\% of original data, while ``Ours (10\%)'' denotes applying ``negCLIPLoss (20\%) $\cap$ \infnormsim(Target)'' to get 10\%. And we use ``*'' to indicate the case where we choose the intersection of the data selected by using OAI CLIP-B/32 and OAI CLIP-L/14 separately, which results in about 15M data for ``Ours (20\%)*'' and 7.4M data for ``Ours (10\%)*''. 
% ``Ours'' refers to the data obtained by ``negCLIPLoss $\cap$ \infnormsim(Target)''. 
% Details in the text description of Sec.~\ref{sec: D2 D3}.
% \simon{} \yiping{fixed}
% , and ``Ours2'' refers to the intersection of selected data obtained separately from OAI CLIP-L/14 and OAI CLIP-B/32 with ``negCLIPLoss (20\%) $\cap$ \infnormsim(Target) (10\%)''.\simon{ Having both Ours1 and Ours2 look weird.}
% Method1 ($\alpha\%$) $\cap$ Method2 ($\beta\%$) denotes first use Method1 to filter to $\alpha\%$, then use Method 2 to filter to $\beta\%$ with respect to the original whole pool.
}
\vspace{-0.5em}
\label{tab: D2D3 compare}
\begin{tabular}{@{}llcccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Type}} & \multirow{2}{*}{\textbf{Filtering Strategy}} & \multirow{2}{*}{\textbf{Size}} & \textbf{IN-1k} & \textbf{IN Shift} & \textbf{VTAB} & \textbf{Retr.} & \textbf{Avg.} \\
 & &  & (1) & (5) & (11) & (3) & (38)\\
 \midrule
D2 & DFN~\citep{fang2023data} & 16M & {36.0} & {30.1} & {36.2} & {27.0} & {35.4}\\
% D3 & Text-based~\citep{gadre2023datacomp} & 26M & 24.8 & 22.2 & 30.1 & 24.2 & 29.5 \\
D3 & T-MARS~\citep{maini2023t} & 22M & 30.8 & 26.3 & 34.8 & 25.4 & 34.1 \\
D3 & Devil~\citep{yu2023devil} & 20M & 31.0 & 26.7& 35.9 & 24.7 & 34.5\\
D3 & MLM~\citep{wang2024finetuned} & 38M & 30.3 & 25.6 & 36.0 & \textbf{29.0} & 34.5\\
D3 & HYPE~\citep{kim2024hype} & 10M & 30.3 & 25.8 & 34.3 & 22.2 & 31.9\\
% HYPE is 10.7M on our server
D3 & DFN $\cup$ HYPE~\citep{kim2024hype} & 20M & \underline{36.4} & {30.8} & \underline{38.5} & {28.0} & {36.8}\\
\midrule
D1 & \textbf{Ours (20\%)} & 22M & {32.4} & {27.4} & {35.9} & {26.3} & {35.2}\\
% D3 & DFN* $\cup$ \textbf{Ours1} & 21M & \textbf{36.5} & \textbf{30.9} & \underline{36.4} & {27.6} & \underline{36.4} \\
D3 & DFN $\cup$ \textbf{Ours (20\%)*} & 23M & \underline{36.4} & \underline{30.9} & \textbf{38.6} & \underline{28.1} & \underline{37.6} \\
D3 & DFN $\cup$ HYPE $\cup$ \textbf{Ours (10\%)*} & 22M & \textbf{37.3} & \textbf{31.4} & \underline{38.5} & 27.6 & \textbf{37.7} \\
\bottomrule
\end{tabular}
\vspace{-1.7em}
\end{table*}


% for ``\textbf{Ours (10\%)}'', we select about 7.4M data which are both selected by using OAI CLIP-B/32 and OAI CLIP-L/14 on ``negCLIPLoss (20\%) $\cap$ \infnormsim(Target) (10\%)''. We found that this is more robust than using OAI CLIP-L/14 alone. 
% It will be an interesting future direction for analyzing the implicit difference between different teacher models.\yiping{check this}
% by 1\% over the original DFN (as shown in DFN* $\cup$ \textbf{Ours1}), when merging our selected data with the output of DFN. 
% \yifang{Wait for hype.}
% \yiping{delete the details in table.}
% \yiping{Do we need the computation cost table here?}










==> dmlr_icml_2024_content/introduction.tex <==
\section{Introduction}
% \yiping{can we make the introduction shorter?}

Curating large-scale visual-language datasets from web-sourced data has become common for pretraining multi-modal models. However, the quality of these web-curated data pairs remains a critical bottleneck. Research has shown that the choice of dataset significantly impacts model performance, irrespective of the models and training techniques employed~\citep{radford2021learning, schuhmann2022laion, cherti2023reproducible, bai2023qwen}, and this motivates the development of various data selection strategies. This paper focuses on optimizing subset selection from a fixed data pool to train a CLIP model \citep{radford2021learning} that achieves superior performance on zero-shot downstream tasks.

Classical methods \textit{rely solely on OpenAI's pretrained CLIP model} (i.e., a teacher model) and focus on better utilizing the embeddings. The most commonly used one is calculating CLIPScore~\citep{hessel2021clipscore}, which measures the cosine similarity between the visual and language embeddings of the CLIP model for the same sample, to eliminate low-quality data with mismatches between text and image. Other works also leverage heuristic distribution alignment techniques to select samples relevant to downstream tasks, such as image-based filtering~\citep{gadre2023datacomp}. 
% and CIDS~\citep{yu2023devil}. 
These approaches are generally viewed as providing only limited enhancements. However, we argue that the potential of those embeddings has been heavily under-explored. 
This work seeks a universal method to better employ any given embeddings, not only from OpenAI's (OAI) CLIP, but also from other CLIP-style models.

% On the other hand, existing leading data filtering methods allall involve using external models or high-quality multi-modal data pairs to train a new model that aids in data selection. There are primarily two directions to using external resources. The first line of works utilizes existing non-CLIP models to identify specific elements within the noisy dataset, \yifang{if we want to add hype without DFN we may need rephrase this} facilitating later filtering. For example, T-MARS \citep{maini2023t} removes images where the text is the only feature correlated with the caption using FAST \citep{chen2021fast}, an off-the-shelf OCR text detection model. Devil \citep{yu2023devil}  applies fasttext~\citep{} to remove non-English texts and use BLIP-2~\citep{} model as digit recognition to keep useful digits images. The second direction, represented by Data Filtering Network (DFN) \citep{fang2023data}, involves training a new CLIP-style teacher model that using high-quality datasets like CC12M and HQITP-350M. Although this model performs worse than the OAI CLIP in downstream tasks, it is particularly good at filtering out low-quality data. However, these methods fail to fully exploit the potential of the "less powerful embedding" obtained from the OAI CLIP model alone -- embeddings not explicitly designed for data filtering but for improving downstream tasks. They mainly use CLIP embeddings to calculate CLIPScore and apply the aforementioned heuristic distribution alignment, leading to suboptimal utilization of the CLIP teacher model. We assert that there are universal and more effective strategies for utilizing any CLIP teacher model, regardless of its architecture (e.g., B/32 or L/14) or the dataset it was trained on (e.g., OAI-WIT-400M or DFN's high-quality dataset). These strategies should be orthogonal to the use of other external models such as FAST and BLIP-2.

On the other hand, recent leading data filtering methods, instead of focusing on improving embedding utilization stategy itself, mainly follow the other two directions, both employing external resources. They either (1) use \textit{external non-CLIP models} that aid in data selection, (2) or use \textit{external high-quality multi-modal data} to train a \textit{better CLIP-style embedding model} than the original OAI CLIP to filter out low-quality data. Specifically, in the first line of works, HYPE~\citep{kim2024hype} leverages embeddings from hyperbolic models instead of the classical Euclidean-based CLIP to measure how each data point has semantically overlaps with other data points and filters out data with low specificity. T-MARS~\citep{maini2023t} removes images where the text is the only feature correlated with the caption using FAST \citep{chen2021fast}, an off-the-shelf OCR text detection model. Devil~\citep{yu2023devil}  applies fasttext~\citep{joulin2016bag} to remove non-English texts and use BLIP-2~\citep{li2023blip} model for digit recognition to keep useful images with digits. The second direction, represented by Data Filtering Network (DFN) \citep{fang2023data}, involves training a new CLIP-style teacher model that uses high-quality datasets like HQITP-350M. Although the embeddings extracted from this model perform worse than the OAI CLIP in downstream tasks, it is particularly good at filtering out low-quality data. Notably, some of these methods can be combined and indeed, merging the selected data from DFN and HYPE achieves current state-of-art as shown in HYPE paper \citep{kim2024hype}.

% Previous works mainly focus on improving the CLIP embedding quality or utilizing an external model to do filtering but employ the CLIP embedding in a suboptimal way by only using classical methods like CLIPScore. In contrast, 
In this work, we focus on improving the filtering methods themselves for any given CLIP embedding rather than mainly relying on external models or multi-modal datasets. 
% All these leading methods, however, fail to fully exploit the potential of the "less powerful embedding" obtained from the original OAI CLIP model alone, as they merely plug in those classical methods (e.g. CLIPScore, heuristic distribution alignment) mentioned above. In this paper, we make a deep investigation along the direction that is orthongonal to those leading approaches:
%     \textit{How to better employ any given CLIP embeddings (not only OAI CLIP)?}
We show that there are universal and more effective strategies for utilizing any CLIP teacher model, regardless of its architecture (e.g., B/32 or L/14) or the dataset it was trained on (e.g., OpenAI-WIT-400M or DFN's high-quality dataset). These strategies should always be orthogonal to the use of any newly trained CLIP-style models like DFN and might also be compatible with methods using external models like FAST and BLIP-2.

\textbf{Our Contributions.} We introduce two innovative approaches for data quality characterization in multi-modal contexts: \textbf{negCLIPLoss} and \textbf{Norm Similarity Score (\normsim)}. \textbf{negCLIPLoss} addresses the limitations of traditional CLIPScores by normalizing scores using the similarity between a sample and its contrastive pairs, effectively reducing biases such as those introduced by generic terms like "image". This method applies universally across various embedding models (see Fig.~\ref{fig:CLIPLoss_vs_CLIPScore}). On the other hand, \textbf{\normsim} leverages available knowledge about downstream tasks to enhance data filtering. It computes the vision similarity between a training sample and a target dataset using a $p$-norm, where significant parameters are typically $p=2$ or $\infty$. 
% Unlike methods that maintain diversity by clustering, \textbf{\normsim} focuses on closeness to any target sample, streamlining the selection process . 
Both metrics, \textbf{negCLIPLoss} and \textbf{\normsim}, complement each other in optimizing data selection for specific tasks (see 
Fig.~\ref{fig:sim_vs_quality}).

To illustrate the effectiveness of our methods, we use a widely used benchmark DataComp~\citep{gadre2023datacomp}. We show that, by simply replacing CLIPScores with \textbf{negCLIPLoss} and utilizing \textbf{\normsim}, 
% We show that, by simply replacing the CLIPScores with \textbf{negCLIPLoss} which better characterize the data quality and designing a new distribution measurement metric p-Norm Similarity Score (\textbf{\normsim}) when knowledge about downstream tasks is available, 
we can exceed the best OAI-CLIP(L/14)-based baseline by 5.3\% on ImageNet-1k and 2.8\% on average across 38 downstream tasks, which is similar or even better than the performance achieved by many external-resources-based methods. 
% Notably, even if the target downstream tasks are not available, we demonstrate that using {\normsim} on a proxy downstream task constructed from the training set, called {\textbf{\twonormsimD}}, combined with negCLIPLoss, can also gain a 1.9\% improvement on 38 downstream evaluation.
% \yifang{Number}.  
Moreover, 
% the improvements achieved by our methods are not limited to OAI CLIP-based methods but can also be obtained by combining our methods with advanced models that require external resources. 
\textit{by merging the subset selected by \textbf{negCLIPLoss} and \textbf{{\normsim}} with the subset selected by current state-of-the-art method ``HYPE $\cup$ DFN'', we can further improve it by 0.9\% on both ImageNet-1k and on average 38 downstream tasks.
We can also achieve a 0.8\% improvement on average 38 tasks over "HYPE $\cup$ DFN" using only the data selected by DFN and our strategies.}
% Firstly, by merging the subset selected by \textbf{negCLIPLoss} and \textbf{{\normsim}} with the subset selected by DFN, we achieve an additional 1\% increase in performance. 
% This performance is very close to current SOTA (i.e. HYPE+DFN) without training an extra hyperbolic model as in HYPE. 
% More importantly, we demonstrate that negCLIPLoss, as a replacement for CLIPScore, can be applied to any embedding models like OAI-L/14, OAI-B/32, and DFN-B/32. 
% universally boosting performance from 0.4\% to 3.0\% on an average of 38 tasks.
% , even when the model itself does not perform well on downsteam tasks.
% 
% This result is not only technically insightful for understanding the information available in embeddings but also practically significant. 
Besides, compared to existing methods, our approach saves a significant amount of computational time on data reprocessing as shown in Table~\ref{fig: compute cost}.
% For example, \yifang{time for HYPE?} when the CLIP embeddings are obtained (cost about 45 hours for CLIP-B/32), both {T-MARS} \citep{maini2023t} and {MLM} \citep{wang2024finetuned} still require more than 900 hours data pre-processing time to extract the required information from 110M size dataset of DataComp-medium, while we only need about 5 hours.  On the other hand, DFN, although has a similar forward speed (i.e. preprocessing time), requires retraining a new CLIP teacher model on the HQITP-350M, which is larger than DataComp-medium. \yifang{If we don't plan to emphasize the computational efficiency, we can delete this part? }




% \textbf{V}ariance \textbf{A}lignment \textbf{S}core (\textsf{VAS}) which aims to find the most informative subset of the training data whose (cross-)covariance between the image-text pairs most aligns with the (cross-)covariance of a reference distribution. This reference distribution could be the approximate distribution of test set (if we have access) or even the entirety of the pool.


\iffalse
\section{Introduction}

Curating web-scale visual-language datasets for pretraining models has become a widely adopted approach to improve visual model performance. Many studies have demonstrated that, despite the use of fixed models and training methods, the final performance of a model is significantly impacted by the choice of data \citep{radford2021learning, schuhmann2022laion, cherti2023reproducible, bai2023qwen}. Consequently, various data selection strategies have been proposed to tackle the challenges posed by large datasets with varied data quality and limited computational resources. These strategies, also known as filtering, subset selection, or pruning in the literature, each focus on slightly different objectives. Some strategies prioritize screening out unhelpful samples to maximize the final model performance without budget constraints, while others aim to maximize performance compared to other randomly sampled subsets within the same budget limit. Practically, these strategies are not mutually exclusive, and in this paper, we will evaluate our proposed strategies in both contexts.
% 
% \yifang{Right now it is a little ambiguous when we say filtering/subset selection. In datacomp, seems our ultimate goal is filtering to achieve better performance than the pool but the method we are using is inspired by subset selection. On the cc12M we are strictly using subset selection setting. I plan to make it clear in the later introduction.}

One line of effective approaches treats each sample independently by assigning a quality score to each individual and only training on the samples that received the highest scores.
For example, the baseline CLIP score filtering method uses a pretrained CLIP model to calculate the cosine similarity score between image and text embeddings, and then discards those pairs that are less aligned. Some follow-up works \citep{nguyen2023improving,mahmoud2023sieve,maini2023t,fang2023data} which propose more advanced image-text alignment scoring methods by using other pretrained classification models or more carefully crafted rule-based approaches. Please refer to related works Sec.~\ref{sec: related work} for a more detailed description.

All those works, however, failed to consider the selection strategy from data distribution perspective. This disadvantage becomes more significant with limited computational resources, as high-quality data are not always the most informative or representative. In some cases, certain feature can be easily learnt under much less samples than other features, so adding more high quality data with such feature can hardly further improve the ultimate model. In other cases, certain features rarely occur in our targeted test distribution, and therefore, adding the corresponding samples will have less effect on test performance. Thus, our work proposes a \textit{data-distribution-aware} strategy that can be combined with existing strategies focused on individual data quality. 

One of the most relevant works to ours is \citet{maharana2023d2}, which also considers the example difficulty and  diversity by using forward and
reverse message passing over a constructed dataset graph.  Their approach, however, is designed for general learning frameworks for both supervised and unsupervised (i.e. contrastive) learning without considering the special impact of data distribution in \textit{multi-modal contrastive learning}. 
% 
Another relevant strategy is using the external image-set as data prior proposed by \citet{gadre2023datacomp}, which clusters the image embedding of the candidate pool and selects the samples whose cluster center is the nearest center for at least one ImageNet-1K training example. 
But this method also comes from more heuristic inspiration without considering the particular learning method, and is therefore more hyper-parameter sensitive.
% 
In contrast to both approaches, our strategy is inspired by recent theoretical progress in those contrastive representation learning works \citep{nakada2023understanding,ji2023power}. As a results, our work achieves much better average performance over the 38 downstream tasks compared to these two and is almost hyper-parameter-free.

\begin{figure*}[t]
    \centering
    \small
    \includegraphics[width=1.0\textwidth]{fig/vis3.pdf}
    \vspace{-1.2em}
    \caption{Illustration of our VAS on DataComp. $\bar f$ means the embeddings calculated by the pre-trained model, and $\Sigma_{\text{prior}}$ matrix is the test prior co-variance matrix, can be chosen as the co-variance matrix of the image embeddings from ImageNet-1k or DataComp itself. (a) Visualization of data with different Variance Alignment Score (VAS) and CLIP score in DataComp. CLIP score does not efficiently evaluate the informativeness of image-text pairs. Data from OCR tasks or unconventional visual tasks (Type 4) can have high quality but little useful visual information. However, VAS can select the data with more meaningful image features (Type 1 and Type 2).
    (b) Illustration of a rough comparison of sampling data for different filtering methods. Using VAS $\cap$ CLIP score filtering can balance the informativeness and quality and increase the proportion of Type 2 data, which are the most helpful data for training image-text models. Please refer to Appendix.~\ref{sec: add_vis} for more visualization results.}
    % \label{fig:vis}
    \label{fig:vas_cs}
    \vspace{-1.0em}
\end{figure*}


Specifically, we propose \textbf{V}ariance \textbf{A}lignment \textbf{S}core (\textsf{VAS}) which aims to find the most informative subset of the training data whose (cross-)covariance between the image-text pairs most aligns with the (cross-)covariance of a reference distribution.
For example, the reference distribution could be the entirety of the pool from which a subset is being chosen, or some other more task-dependent dataset.  
We also combine VAS with a method based on an individual quality metric as it provides a boost in performance empirically. (Sec.~\ref{sec: main})
To validate the effectiveness of our strategy, we primarily leverage the DataComp benchmark \citep{gadre2023datacomp}. Compared with the existing best strategies, it improves 1.3\% averagely on 38 evaluation sets for DataComp without budget constraints and improves averagely 0.4\% for CC12M with budget constraints (see Sec.~\ref{sec: experiment}).
% \yifang{I originally plan to talk about computational efficiency also but now I find the difference it not that significant? All the base-line method do selection < 1h. So I delete it.}
% \yiping{OK for me}


In addition to empirical results, we provide a theoretical justification for our strategy under a linear model assumption. Firstly, assuming we are given a perfect embedding model and proper data prior, we show that choosing the subset to minimize the multi-modal contrastive loss, including the CLIP loss, can be reduced to the problem of maximizing the total VAS score of the subset. Secondly, we prove a generalization bound when the embedding model and data prior are non-perfect (see Sec.~\ref{sec:theory}).

\iffalse
In addition to proposing this distribution-aware, multi-modal contrastive learning focused data selection strategy, we also gain several insights during the design:
\begin{itemize}[leftmargin=*] 
    \item We observe the widely-used CLIP score filtering does not have a close relation with the data informativeness. Therefore, we should be more careful when interpreting scores generated by some external embedding models.
    \item Our empirical findings confirm the previous result that the image embeddings from Imagnet-1K are effective data prior. Nevertheless, we also find a heuristic subset selection method which only relies on training data itself as detailed in equation~\ref{eq:tr_S}. We believe it worth further investigation in the future.\yiping{should we mention alation study and say image is better prior than text?} \yifang{Maybe.. Simon: do those are necessary ?}
    \item Furthermore, we find our strategy is principally contradict to the classical diversity-forced optimal design approach. In fact, we empirically show that the classical A-optimal and V-optimal approaches fails in CLIP training setting, which can be further investigated.
    % \yiping{Add, please check}
    % \yifang{Talk about how this contradicts the classical G-optimal design ?}
\end{itemize}
\fi

\fi

==> dmlr_icml_2024_content/problem_setup.tex <==
\vspace{-1em}
\section{Problem Setup}
\vspace{-0.3em}

\textbf{Data Filtering on Multimodal Dataset.}
We are given a training dataset $D_\text{train} = \{x^{v}, x^{l}\}$, where $(x^{v}, x^{l}) \in \mathbb{R}^D$ is the image-text (vision-language) training pair. 
% For convenience, we will let superscript $vl$ denote either modality so that, for example, $x^{vl} \in {x^{v}, x^{l}}$. 
Our goal is to identify a subset $S \subset D_\text{train}$ that maximizes the zero-shot accuracy of the CLIP model on some downstream tasks when $S$ is used to train the CLIP model. 
\textbf{CLIP.} 
% Recent efforts, such as LAION \citep{schuhmann2022laion} and DataComp \citep{gadre2023datacomp}, use OpenAI’s CLIP ViT-L/14 model \citep{radford2021learning} as a teacher model to obtain quality score. Here 
We denote the teacher CLIP model as $\bar{f}_{vl}$.
% 
For any pair $x^{vl}$, the model outputs a normalized unit-vector $\bar{f}_{vl}(x^{vl})$. 
If $X^{vl} := \{x_1^{vl}, \ldots, x_m^{vl}\}$ denotes a dataset containing $m$ samples, then we define $\bar{f}_{vl}(X^{vl}) = [\bar{f}_{vl}(x_1^{vl}),\ldots, \bar{f}_{vl}(x_m^{vl})]^\top \in \R^{m \times d}$.
The popular filtering metric ``CLIPScore'' is defined as $\langle  \bar{f}_v(x^v), \bar{f}_l(x^l) \rangle \in [-1,1]$.
% It is commonly believed that pairs with higher clip scores are more likely to be effective samples since the image is aligned with the text. However, one of our main contributions shows that considering the absolute value of CLIP score instead of relative values inside a cluster is less effective. 
\textbf{Dataset and model.} We follow the pipeline of Datacomp \citep{gadre2023datacomp} to standardize the training and evaluation process as previous papers~ \citep{nguyen2023improving,maharana2023d2,maini2023t,fang2023data,mahmoud2023sieve,bai2023qwen}.More in Sec.~\ref{sec: experiment}.

\iffalse
We are given a training dataset $D_\text{train} = {x^{v}, x^{l}}$, where $(x^{v}, x^{l}) \in \mathbb{R}^d$ is the image-text (vision-language) training pair. For convenience, we will let superscript $vl$ denote either modality so that, for example, $x^{vl} \in {x^{v}, x^{l}}$. We aim to identify a subset $S \subset D_\text{train}$, with or without subset size constraints, that maximizes the zero-shot accuracy of the CLIP model on some downstream tasks when $S$ is used to train the CLIP model.

\textbf{CLIP score and embedding.} Recent efforts, such as LAION \citep{schuhmann2022laion} and DataComp \citep{gadre2023datacomp}, use OpenAI’s CLIP ViT-L/14 model \citep{radford2021learning} as a teacher model to obtain quality score. Here we denote this vanilla CLIP model as $\bar{f}_{vl}$.
% 
For any pair $x^{vl}$, the model outputs a normalized unit-vector $\bar{f}_{vl}(x^{vl})$. 
Then ``CLIPScore'' of data pair $i$ is defined as $\langle  \bar{f}_v(x_i^v), \bar{f}_l(x_i^l) \rangle \in [-1,1]$.
% Let $\bar{s}_{ij} := \langle  \bar{f}_v(x_i^v), \bar{f}_l(x_j^l) \rangle \in [-1,1]$ denote the pairwise cosine similarity between $i$-th image and $j$-th text. 
% In the subsequent sections, we will refer to $\bar{s}_{ii}$ as the “CLIP score” from an existing-pretrained ``vanilla'' model publicly available. \yiping{double check if we need $s_ii$ and the later sentence.}
It is commonly believed that pairs with higher clip scores are more likely to be effective samples since the image is aligned with the text. However, one of our main contribution shows that considering the absolute value of CLIP score instead of relative values inside a cluster is less effective. 
\vspace{-1em}
\paragraph{Dataset and model.} Here we follow the pipeline of Datacomp \citep{gadre2023datacomp} to standardize the training and evaluation process. This is a testbed for dataset experiments aiming to open-source and further improve the vanilla CLIP model and is widely adopted in previous data selection papers~ \citep{nguyen2023improving,maharana2023d2,maini2023t,fang2023data,mahmoud2023sieve,bai2023qwen}. We will give more details in Sec.~\ref{sec: experiment}.\yiping{We don't need this paragraph here?}
\fi
% \vspace{-1em}

==> dmlr_icml_2024_content/strategy_overview.tex <==
\begin{figure*}[t]
    \centering
    \small
    \includegraphics[width=0.85\textwidth]{fig/p4.pdf}
    \vspace{-0.6em}
    \caption{Illustration of negCLIPLoss. CLIPScore may underestimate (bottom left) or overestimate (bottom right) the quality of image-text pairs. 
    However, this issue can be mitigated by simply adding a normalization term like negCLIPLoss. 
    % negCLIPLoss employs the teacher model to calculate the negative CLIP loss on training data and serves as a more accurate metric. 
    ``Top X\%'' denotes that the score represents the top X\% \textit{high} values within the entire dataset.}
    \label{fig:intro_CLIPLoss}
    \vspace{-1.5em}
\end{figure*}
\vspace{-1em}
\section{Data Filtering Strategy}
\subsection{negCLIPLoss: A Better Metric than CLIPScore}
\label{subsec: negCLIPLoss}
% \yifang{If we don't need those theory we can further simpplify the notations..}

In this section, we introduce a better and statistically interpretable quality metric called negCLIPLoss, which directly replaces the common metric CLIPScore. Fig.~\ref{fig:intro_CLIPLoss} illustrates how negCLIPLoss works. 
% This new metric only requires negligible extra computational costs and no additional external data collection costs. 
% Its effectiveness has been shown in Figure~\ref{fig:CLIPLoss_vs_CLIPScore}.
As the name suggested, this metric is inspired by the standard CLIP loss used in the actual training process of the teacher CLIP model:
\begin{equation}
\small
    \ell_{B^*}(x_i^{vl}) = -\frac{1}{2}\left[\log \frac{\text{exp}( \bar{f}_v(x_i^v)^\top \bar{f}_l(x_i^l)/\tau)}{\sum_{j \in B^*} \text{exp}(\bar{f}_v(x_i^v)^\top \bar{f}_l(x_j^l)/\tau)}
    + \log \frac{\text{exp}(\bar{f}_v(x_i^v)^\top \bar{f}_l(x_i^l))/\tau}{\sum_{j \in B^*} \text{exp}( \bar{f}_v(x_j^v)^\top \bar{f}_l(x_i^l)/\tau)}\right]
\end{equation}
Here $B^*$ is the random batch where $i$-th sample belongs during the final training step, and $\tau$ is the learnable temperate parameter. 
Notably, the teacher loss differs from CLIPScore primarily by a normalization term $\mathcal{R}^*$ as follows:
\begin{equation*}
\small
    - \tau \cdot \ell_{B^*}(x_i^{vl})
    = \underbrace{\bar{f}_v(x_i^v)^\top \bar{f}_l(x_i^l)}_{\text{CLIPScore}} -  \underbrace{\frac{\tau}{2}\left[\log \sum_{j \in B^*} \exp(\frac{\bar{f}_v(x_i^v)^\top \bar{f}_l(x_j^l)}{\tau}) +  \log \sum_{j \in B^*} \exp(\frac{\bar{f}_v(x_j^v)^\top \bar{f}_l(x_i^l)}{\tau})\right]}_{\text{normalization term } \mathcal{R}^*}
    % \vspace{0.1em}
\end{equation*}
In practice, since the training dataset of teacher CLIP models, like OAI-WIT400M~\citep{radford2021learning}, and the actual batch divisions $B^*$ is inaccessible, 
we randomly select $K$ batches from the student model's training data and use the averaged results from 
$\{B_k\}_{i=1}^K$ to estimate the normalization term $\mathcal{R}^*$ on $B^*$, as shown in 
Eqn.~\ref{eq: negcliploss}:
\begin{equation}\label{eq: negcliploss}
    \small
    \text{negCLIPLoss}(x_i^{vl}) := -\frac{\tau}{K}\sum_{k=1}^K\ell_{B_k}(x_i^{vl}) \ \approx \ \text{CLIPScore}(x_i^{vl}) - \mathcal{R}^*
\end{equation}

\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-2em}
\centering
\includegraphics[width=0.45\textwidth]{fig/comparison_CLIPScore_vs_negCLIPLoss2.pdf}
\vspace{-1.2em}
\caption{Comparison of negCLIPLoss and CLIPScore across different downsampling ratios on DataComp-medium. 
% \yiping{TODO: change name}
}
\label{fig:CLIPLoss_vs_CLIPScore}
\vspace{-1.5em}
\end{wrapfigure}

\noindent Here $\{B_k\}_{i=1}^K$ are some batches randomly selected from the student model's training data and $x_i \in B_k, \forall k$. We choose $K=10$ in our experiments, but any sample size larger than 5 is sufficiently stable (Appendix~\ref{supp: stability of K}). In Appendix~\ref{supp: computation cost} we also show that the computational cost introduced by $\mathcal{R}$ remains negligible compared to other baselines. Temperature $\tau$ and batch size $|B^*|$ can be directly obtained from the pretrained teacher model, and the algorithm process of calculating negCLIPLoss is in Appendix~\ref{supp: negcliploss detail}.

\noindent\textbf{Motivation behind negCLIPLoss.} Existing works like LESS~\citep{xia2024less} in NLP, CoDis~\citep{Xia_2023_combatting} in CV, and RHO~\citep{pmlr-v162-mindermann22a-prioritized} in data scheduling utilize loss-guided data selection. Despite that, the suitability of this approach for multi-modal contrastive learning remains uncertain. We address this by demonstrating that {negCLIPLoss} consistently performs as well as or better than CLIPScore (see Fig.~\ref{fig:CLIPLoss_vs_CLIPScore}).
The reason is that 
{negCLIPLoss} incorporates a normalization term that corrects the biases inherent in CLIPScore (Fig.~\ref{fig:intro_CLIPLoss}). This term adjusts for cases where text or image embeddings match with multiple contrastive pairs, not just their intended counterparts. For instance, terms like "Image" or "Photo" may result in falsely high CLIPScores as they can match various visual contents. Similarly, simple visual elements can align with numerous general descriptors, lowering their relative negCLIPLoss despite high initial CLIPScores. In contrast, specific words, such as "Islands Harbor" and "American football", have fewer potential matches, resulting in a higher relative negCLIPLoss. 
This illustrates how {negCLIPLoss} provides a more accurate measure in multi-modal contexts.



\iffalse
Since it is impossible to access the actual batch divisions $B^*$ during teacher model training, we randomly sample $K$ different batch divisions $B_k$ on the student model's training data and compute the average CLIP loss across these divisions.  Formally, we define our metric $\text{\textbf{negCLIPLoss}}(x_i^{vl})$ for any $x_i$ as:
\iffalse
\begin{align*}
    \text{negCLIPLoss}(x_i^{vl})
    & = 
    - \frac{\tau}{2}\log \left(\frac{1}{K}\sum_{k=1}^K \text{exp}(-\ell_B(x_i^{vl})) \right)\\
    & \approx \bar{f}_v(x_i^v)^\top \bar{f}_l(x_i^l) -  \underbrace{\frac{\tau}{2}\left[\log \sum_{j \in B(i) \setminus i} e^{\bar{f}_v(x_i^v)^\top \bar{f}_l(x_j^l)/\tau} +  \log \sum_{j \in B(i) \setminus i} e^{\bar{f}_v(x_j^v)^\top \bar{f}_l(x_i^l)/\tau}\right]}_{\text{normalization term} \mathcal{R}}
\end{align*}
\begin{align*}
    \text{negCLIPLoss}(x_i^{vl})
    & = 
    - \frac{\tau}{K}\sum_{k=1}^K \ell_{B_k}(x_i^{vl})\\
    & \approx \bar{f}_v(x_i^v)^\top \bar{f}_l(x_i^l) -  \underbrace{\frac{\tau}{2}\left[\log \sum_{j \in B^*} e^{\bar{f}_v(x_i^v)^\top \bar{f}_l(x_j^l)/\tau} +  \log \sum_{j \in B^*} e^{\bar{f}_v(x_j^v)^\top \bar{f}_l(x_i^l)/\tau}\right]}_{\text{normalization term } \mathcal{R}}
\end{align*}
\fi
\begin{align*}
    - \frac{\tau}{K}\sum_{k=1}^K \ell_{B_k}(x_i^{vl})
    \approx \bar{f}_v(x_i^v)^\top \bar{f}_l(x_i^l) -  \underbrace{\frac{\tau}{2}\left[\log \sum_{j \in B^*} e^{\bar{f}_v(x_i^v)^\top \bar{f}_l(x_j^l)/\tau} +  \log \sum_{j \in B^*} e^{\bar{f}_v(x_j^v)^\top \bar{f}_l(x_i^l)/\tau}\right]}_{\text{normalization term } \mathcal{R}}
\end{align*}
where temperature $\tau$ and batch size $|B_*|$ can be directly obtained from the parameters of the pretrained teacher model. 
\yiping{Give an example here. We still need some intuition for negCLIPLoss!}
\fi


% \yiping{Need add detail about temperature and batch size.} \yifang{I add one sentence.}


% \begin{figure*}[t]
%     \centering
%     \small
%     \includegraphics[width=0.6\textwidth]{fig/comparison_CLIPScore_vs_CLIPLoss2.pdf}
%     \vspace{-1.2em}
%     \caption{CLIPLoss behaves better or on pair of CLIPScore among different downsampling ratios. \yiping{TODO: change name}}
%     \label{fig:CLIPLoss_vs_CLIPScore}
%     \vspace{-1.0em}
% \end{figure*}




\begin{figure*}[t]
    \centering
\includegraphics[width=0.85\textwidth]{fig/vis2.pdf}
    % \vspace{-1.2em}
    \caption{Illustration of {\normsim} on DataComp. 
    % $\bar f$ represents the embedding extracted by the pretrained model, $X_\text{target}^v$ is the images of the target prior data, and similarly $x^v$ denotes the image of the train data. 
    % $X_\text{target}$ is the target prior data.
    % ``Top X\%'' denotes that the score represents the top X\% {high} values within the entire dataset.
    (a) Visualization of data with different {\normsim} and negCLIPLoss. Here we use {\twonormsim}(ImageNet-1k) as an example.
    Although both Type 2 and Type 4 data have high negCLIPLoss and thus high quality, data with low {\twonormsim} (Type 4) are more irrelevant to downstream tasks such as ImageNet (like they contain many images dominated by text of captions) and make little contribution to improving downstream performance. (b) Using ``$\text{negCLIPLoss} \cap \text{\normsim}$'' filtering can balance the quality and relevance to downstream tasks, thus sampling more Type 2 data. 
    % (Refer to Appendix~\ref{supp: add_vis} for more visualization.)
    % \yifang{TODO: change the name val to target in figure}
    % \yiping{TODO: add appendix}
    } 
    \label{fig:sim_vs_quality}
    \vspace{-1.2em}
\end{figure*}
\vspace{-0.5em}
\subsection{\normsim: A New Training-Target Similarity Metric}
\vspace{-0.5em}
\label{subset: normsim}
% \yiping{I think $x_j$ and $x_i$ for val/train is confusing, working on changing some symbols. Need to combine some symbols. }

Our proposed negCLIPLoss is a universal approach to improve filtering performance by estimating quality better, and it
does not rely on any downstream task. Now, if we can access some knowledge of the downstream tasks, we could further improve the performance by using a vision-only \textit{$p$-norm similarity to target data} metric to measure the relationship between each training sample and the downstream target data. We will discuss the reason to use vision-only embedding later in this section.
% \simon{why vision-only?}\yiping{Add a sentence, is this ok?}

Specifically, we assume access to the target set of downstream tasks and denote them as $X_\text{target} = \{x_{\text{target},(1)}, \ldots, x_{\text{target},(m)}\}$, where each $x_{\text{target},(i)} \in \mathbb{R}^d$ is \textit{i.i.d.}-sampled 
from the target downstream distribution $\mathcal{P}_\text{target}$\footnote{Although out-of-distribution tasks like ``WILDS'' have distribution shift between training data and test data, they still provides useful information of the test data.}, 
but without overlapping with the test set.
Then, for each training sample $x^{vl}$ and the corresponding target set $X_\text{target}$, \text{NormSim} is defined as:
\vspace{-0.5em}
\begin{equation}
% 
\small
\text{\normsim}_p(X_\text{target}, x)
:= \|\bar{f}_v(X_\text{target}^v) \bar{f}_v(x^v) \|_p
% = \left(\sum_{x_{t} \in X_\text{target}} \left|\langle \bar{f}_v(x_{{t}}^v), \bar{f}_v(x^v) \rangle\right|^p\right)^{1/p}
% \vspace{-0.5em}
\end{equation}
We select the subset $S$ of size $N$ by greedily choosing the samples with the largest \text{NormSim} scores. 
% The choice of the norm type $p$ can be based on the data distribution and training process. 
We consider $p=\infty$ in the main paper and left $p=2$ in Appendix~\ref{supp: sec normsim dis}. 
When $p = \infty$, a training sample will be selected if it has enough high similarity to \textit{any target sample}. Note that this is different from the nearest-neighbor-based method used in image-based filtering~\citep{gadre2023datacomp}, where they are trying to find the nearest training sample of \textit{every target sample}. In detail, {\infnormsim} can be regarded as:
\begin{equation}
\small
S = \arg \max_{|S| = N} \sum_{i \in S} \max_{x_t \in X_\text{target}}\bar f_v(x_t^v)^\top \bar f_v(x^v_i)
\end{equation}
In Appendix~\ref{supp sec: inf norm better than nn}, we also show that our {\infnormsim} can outperform the nearest neighbor selection on the downstream target tasks.
Here, we show an example selected via the \twonormsim(ImageNet-1k) in Fig.~\ref{fig:sim_vs_quality} (Refer to Appendix~\ref{supp: add_vis} for more visualization.), showing that this vision-target-aware method is complementary to the quality-based one. Please refer to Appendix~\ref{supp: sec normsim dis} for more discussions.


% \yifang{Add some sketch here if we have extra space.}\yiping{I think maybe just mention our main conclusion here. something like {\twonormsim} is the best strategy under the linear CLIP case? Also worth mentioning that the concurrent work Joshi et al.~\citep{pmlr-v238-joshi24a} also has similar theoretical results, but they focus more on corset selection where the training set has high data quality}


% Here is an intuitive explanation: The $\vx^{vl}$ we observed comes from the high dimensional representation function mapping from low-dimensional latent vectors. The motivation behind measuring the distance between training and downstream distributions relies on a good embedding model $\bar{f}_{vl}$ that can recover this latent vector. Hence, if there exists some perfect $\bar{f}_{vl}$, then choosing both visual and language information (i.e. $m_1,m_2 = v,l$) leads to best selection. In practice, however, it is well known that the text quality from common crawl is bad since most text are used as a brief caption of the image instead of detailed description. Consequently, 









\iffalse
\section{Data Filtering Strategy (archive)} 
\label{sec: main}
Fig.~\ref{fig:vas_cs} gives an overview of our strategy. We give more details below.




\subsection{Variance Alignment Score (VAS)}


Most existing data selection strategies focus on individual sample quality by measuring the similarity between image and text features (e.g., CLIP score). Yet, they fall short in evaluating how each data point contributes to the model's ability to learn meaningful representations in the context of a target distribution and \emph{other} points included in the set. To measure the informativeness of an individual sample for the overall multi-modal contrastive training, we introduce a novel, data-distribution-aware metric named Variance Alignment Score (VAS) defined as
\begin{align}\label{eq:def_VAS}
    & \text{VAS}_i(m_1,m_2) = \bar f_{m_1}(\vx_i^{m_1})^\top \bar{\Sigma}_\text{test} \bar f_{m_2}(\vx_i^{m_2}) \\
    & \text{where }
    \bar{\Sigma}_\text{test} =  \E_{\vx \sim \vD_\text{test\_proxy}} \bar{f}_{m_1}(\vx^{m_1}) \bar{f}_{m_2}(\vx^{m_2})^\top \nonumber
\end{align}
Here $m_1,m_2$ are the modalities we choose and can be visual or language. And $\vD_{\text{test\_proxy}}$ is some proxy test data distribution when the actual downstream tasks are unknown, which is also called ``data prior" in some previous work as we mentioned in Sec.~\ref{sec: related work}. 
%
The specific choice of $\bar{\Sigma}_{\text{test}}$ and $m_1,m_2$ is crucial and we left details in the next Sec.~\ref{subsec: main strategy}. Here we provide a high level intuition behind VAS.

According to the no-free-lunch theorem, it is impossible to optimize the learning of every feature equally well within a limited budget. In other words, we cannot find a universally optimal strategy for any arbitrary test distribution. Therefore, we tend to select samples that contain effective features in test distributions. Given our focus on this particular multi-modal contrastive learning framework, we leverage insights from previous theoretical generalization bounds as discussed in \citet{ji2023power,nakada2023understanding}. These works suggest that, under a good embedding model $\Bar{f}$, the variance or cross-variance term, denoted as $\frac{1}{N}\sum_i\bar{f}_{m_1}(\vx_i^{m_1}) \bar{f}_{m_2}(\vx_i^{m_2})^\top$, is a suitable criterion for indicating informativeness.
% 
For the rigorous theoretical justification, please refer Lemma~\ref{lem: main} .


\subsection{Main Strategy}
% \vspace{-0.5em}
\label{subsec: main strategy}
% Comment now
% \begin{algorithm}
% \caption{VAS-based strategy}
% \label{algo: main}
% \begin{algorithmic}[ht]
%     \STATE \textbf{Step 1:} \textit{Conservatively} remove low CLIP score samples. (i.e., almost certain low-quality samples)
%     \STATE \textbf{Step 2.1:} Choose proper $\vD_{\text{test\_proxy}}$
%     \STATE \textbf{Step 2.2:} Select $S = \arg \max_{|S| = N} \sum_{i \in S}\text{VAS}_i(v,v)$
% \end{algorithmic}
% \end{algorithm}
\vspace{-0.8em}
We then propose a simple two-stage pruning strategy in Algo.\ref{algo: main} that considers both individual quality and overall distribution by combining the CLIP score with VAS. 

In step 1, we first remove those easily distinguishable low-quality samples, such as low-resolution images or mismatched text (Type 1 and Type 3 data in Fig.~\ref{fig:vas_cs}).
% \simon{we can refer to Figure 1 left here.}\yiping{fix} 
However, unlike the native CLIP score filter in \citet{gadre2023datacomp}, which greedy eliminates 70\% of the data in both DataComp and CC12M datasets, we remove much less data (e.g. around half of the data). Note the overall performance is not sensitive to small variation in removal ratio. 
Subsequently, in step 2, we select a data prior, $\vD_{\text{test\_proxy}}$, either by choosing the external ImageNet-1K or heuristically selecting a subset from the pre-training set which only contains high-frequency features (Details in Eqn.~\ref{eq:tr_S} and \ref{eq:tr_S2}). Based on the selected $\vD_{\text{test\_proxy}}$, we compute the vision-only VAS score and select a subset of size $N$ with the highest scores. Detailed discussions and ablation study results are provided to highlight the significance of these three designs.
\vspace{-0.8em}
\paragraph{CLIP score does not indicate informativeness.} While it is intuitive that extremely low CLIP scores suggest low sample quality, the converse that high CLIP scores suggest high sample quality is not necessarily true. 
For example, if an image contains words that also appear in the caption, that may produce a high CLIP score but not necessarily the kind of relationship between image and caption that we hope to learn. 
In Fig.~\ref{fig:vas_cs}, we observe that data with similar CLIP scores can obtain very different VAS. Some high CLIP score samples can have low VAS and these samples are more related to OCR tasks and unconventional visual features which are intuitively non-helpful.
Therefore, we adopt a two-stage approach wherein the first stage we remove samples with very low CLIP scores, and then apply VAS to the remaining data to perform a more fine-grained selection.

\vspace{-0.8em}
\paragraph{Choice of $\bar{\Sigma}_\text{test}$.} Although the resulting model is evaluated over 38 different downstream tasks that are unknown to the learner in advance, we find out that using ImageNet-1k \citep{deng2009imagenet} as the test proxy achieves good performance. Similar effectiveness has also been observed in \citet{gadre2023datacomp, xu2023cit}. We conjecture that this due to the similar variance distribution between ImageNet-1k and other downstream tasks. In other words, despite different tasks, they all share similar effective features. 

% \kevin{This is a mess and I predict reviewers will not like it, but maybe its just me.}\yiping{just rewrite, is it better?}
Besides using the external dataset ImageNet-1k, we also propose a heuristic method called VAS-D (dynamic) which \textit{only} uses the training data itself as prior. We called it ``dynamic'' because in this method we have that $\bar{\Sigma}_\text{test}$ is dynamically updating based on selected $S$ as in Eqn.~\ref{eq:tr_S}. The high-level principle is still similar. For some hyper-parameter $N$, 
\begin{align}\label{eq:tr_S}
    % & S = \arg \max_{|S| = N} \sum_{i \in S}\Tr\left(\bar f_v(\vx_i^v)^\top \bar{\Sigma}_{\text{test}} \bar f_v(\vx_i^v)\right) \\ \label{eq:tr_S}
    % & \bar{\Sigma}_{\text{test}} = \sum_{j \in S}\bar f_v(\vx_j^v)\bar f_v(\vx_j^v)^\top
    & S = \arg \max_{|S| = N} \sum_{i \in S}\bar f_v(\vx_i^v)^\top \bar{\Sigma}_{\text{test}} \bar f_v(\vx_i^v) \\ 
    & \bar{\Sigma}_{\text{test}} = \frac{1}{|S|}\sum_{j \in S}\bar f_v(\vx_j^v)\bar f_v(\vx_j^v)^\top \nonumber
\end{align}
And it is obviously that (\ref{eq:tr_S}) is equivalent to
% \yiping{No $\sum_i$ ?}
% \yiping{If $\bar\Sigma_{\text{test}}^2$ is better?}
\begin{equation}\label{eq:tr_S2}
    S = \arg \max_{|S| = N} 
    % \sum_{i \in S} 
    \Tr\left((\sum_{j \in S}\bar f_v(\vx_j^v)\bar f_v(\vx_j^v)^\top)^2\right)
\end{equation}
Surprisingly, (\ref{eq:tr_S2}) is conflicted with the general principle in target-agnostic optimal experiment design, which emphasizes the diversity of selected data~\citep{pukelsheim2006optimal}. However, in the Experimental parts (Sec.~\ref{sec: experiment}) we will show that in the context of data selection for training CLIP, the idea of optimal experiment design does not work well.
For the theoretical justification on how the choice of $\bar{\Sigma}_\text{test}$ affects the final performance, please refer to Theorem~\ref{them: main}. 

\vspace{-0.8em}
\paragraph{Necessity of using visual-only information.} The $\vx^{vl}$ we observed comes from the high dimensional representation function mapping from low-dimensional latent vectors. The motivation behind using VAS relies on a good embedding model $\bar{f}_{vl}$ that can recover this latent vector. Hence, if there exists some perfect $\bar{f}_{vl}$, then choosing both visual and language information (i.e. $m_1,m_2 = v,l$) leads to best selection. In practice, however, we found out that visual CLIP model yield much better performance, which may suggest the text embedding is less accurate in recovery. Therefore, we choose to use vision-only information. Also, for the rigorous theoretical justification on how the performance of teacher CLIP model affect the final performance, please refer to  Theorem~\ref{them: main} in Sec.~\ref{sec:theory}.  






\iffalse
\yifang{========Below subject to further modification =============}
Since CLIP score just measures the relevance between image and text embedding, it does not evaluate the information of each data to help the model learn useful representation. We enhance a non-negative quantity named visual \emph{ variance alignment score (VAS)}  defined as:
\begin{equation}
    \text{VAS}(\Sigma, i) = \langle\bar f(\vx_i^v), \Sigma \bar f(\vx_i^v)\rangle
\end{equation}
We denote $\Sigma_{\text{self}}$ and $\Sigma_{\text{img1k}}$ as the variance matrix for image embedding of the training data from the pre-training set itself and external ImageNet-1K datasets, respectively. Thus, VAS measures how well the visual features of the data match the visual distribution of the particular datasets.
And in Fig.~\ref{fig:vas_cs} we visualize the data pairs in the top \yiping{TODO} \% ratio data, and it simply convey two message:
\begin{enumerate}
    \item \emph{Data with similar CLIP scores can obtain very different VAS}. Yhid means that they have different level of useful visual features. For example, the data contain abundant words or unconventional features are always less helpful for training CLIP model.
    \item \emph{DataComp produces similar VAS compared with ImageNet-1k.} Although the data from DataComp may be very different compared with ImageNet-1k, they still have similar variance distribution, which means that they recognize some similar visual features to be the most effective.
\end{enumerate}

In general, we first use the CLIP score filter to filter out some data that has a strong mismatch between image and text, and then select the data with top VAS, i.e.,  curate the subset by 
\begin{equation}\label{eq:obj}
    S_{\text{VAS}} = \arg \max_{|S| = N} \sum_{i \in S}\text{VAS}(\Sigma, i)
\end{equation}
\yiping{Need more illustration, will add soon.}

If we choose $\Sigma = \Sigma_{\text{self}}$, then we can choose a variant of our original object function call as \emph{VAS-D (dynamic)}. To capture the more useful variance direction, we remove the data with low VAS one by one and then change $\Sigma_{\text{self}}$ as the variance matrix of the subset, which means that
\begin{eqnarray}
    S_{\text{VAS-D}} &=& \arg \max_{|S| = N} \sum_{i \in S}\text{VAS}(\Sigma_{S}, i)\\
    &=&\arg \max_{|S| = N}  \sum_{i \in S}\Tr(\Sigma_{S}\cdot \bar f(\vx_i^v) \bar f(\vx_i^v)^\top)\\
    &=& \arg \max_{|S| = N} \Tr(\Sigma_{S}^2) \label{eq:tr_S}
\end{eqnarray}
And we use the greedy remove method to achieve (\ref{eq:tr_S}). Obviously, if we set the greedy step to only one, VAS-D will return to the vanilla VAS method. In the later parts, we will show that this simple algorithm is not only effective but theoretically provable.

\fi
\fi

==> dmlr_icml_2024_content/theory.tex <==

\section{Theoretical Interpretation}\label{sec:theory}

In this section, we give a theoretical justification on the {\normsim} metric when $p=2$ under the linear model assumptions when low quality image and mismatched text has already been removed. In other words, we mainly focus on the following strategy.
\begin{equation}
\small
S = \arg \max_{|S| = N} \sum_{i \in S}\bar f_v(x_i^v)^\top \underbrace{\left(\frac{1}{|X_\text{target} |}\sum_{x_t \in X_\text{target}}\bar f_v(x_t^v)\bar f_v(x_{t} ^v)^\top \right)}_{\Bar{\Sigma}_\text{target\_proxy}}\bar f_v(x_i^v)
\end{equation}

\subsection{Theoretical Setup}

\paragraph{Training data.} For any $\vx^{v}, \vx^{l} \in \R^d$ observable image and text training pairs, we define $\vz^{v}, \vz^{l}$ to be the corresponding latent vectors which contain all semantically pertinent information about our tasks of interest. Similar to previous theoretical work \citep{nakada2023understanding},
we assume each i.i.d pair $\vz^{vl}$ follows zero-mean sub-gaussian distribution whose cross-covariance satisfies
\begin{align*}
    & \text{Cov}(\vz^v,\vz^l) 
    % = \E_{\vz^v_i,\vz^l_j \sim \gD_\text{train}} \left[\vz^v (\vz^l)^\top\right]
    = \Sigma_\text{train} = \text{diag}(\sigma_1,\sigma_2, \ldots),
    & \|\vz^{vl}\| = 1
\end{align*}
and each $\vx^{vl}$ is generated based on a linear model such that
\begin{align*}
    \vx^{vl} = G^*_{vl} \vz^{vl} + \vxi^{vl}.
\end{align*}
Here $G^*_{vl} \in O_{d\times r}$ is the othonormal ground truth representation mapping from the latent vector space to the input space, and $\xi^{vl} \sim \mathcal{N}(0, I_d)$ are \textit{i.i.d.} random noise. 

Also we denote the cross covariance of any finite dataset $S'$ (e.g. the given train set $D_\text{train}$) as $\Sigma_{S'}$.

\paragraph{Test data.} For any zero-shot downstream task, we assume it shares almost same data generation process as the training set, except its the cross-covariance $\Sigma_\text{target}$ does not necessarily equal $\Sigma_\text{train}$, which necessitate the choice of $\Bar{\Sigma}_{\text{target\_proxy}}$.


% \paragraph{CLIP embedding model as teacher} Unlike classical data selection problem where we can only observe $x$ (i.e image, text), here we have a teacher model $\bar{G}_{vl}$, whose generated clip embedding can partially recover the ground truth hidden vector $\vz^{vl}$ with error $\epsilon_{vl}$,
% \begin{align*}
%     \E_{\vz^{vl}, \vx^{vl} \sim \gD_\text{train}} \langle \bar{G}_{vl}\vx^{vl}, \vz^{vl} \rangle \geq 1-\epsilon_{vl}
% \end{align*}
% \yifang{TODO: norm matters if choose 1}
% where $\gD_\text{train}$ is the join training distribution as described in the training data generation process. When $\bar{G}_{vl} = \bar{G}_{vl}^*$, the clip embedding is equivalent to hidden vector. 
% \yifang{Expectation is not strong enough.. maybe need to define over any $|S|$ sampling}

\paragraph{CLIP embedding model as teacher.} Under the linear model assumption, we have a teacher model $\bar{f}_{vl} = \bar{G}_{vl}$, whose generated clip embedding can partially recover the ground truth hidden vector $\vz^{vl}$ with error. 

Formally, we say teacher has $\epsilon_{v}^n$ error if for all possible $n$ budget subsets $S \subset D_\text{train}$,
\begin{align*}
    \frac{1}{|S|} \left\| \sum_{\vx^{vl} \in S} \bar{G}_v^\top \vx^v (\vx^v)^\top \Bar{G}_v - \sum_{\vx^{vl} \in S} \vz^v (\vz^v)^\top \right\|_* \leq \epsilon_{v}^n
\end{align*}
where the same notation applies for the language modal. 
By the orthonormal assumption on the ground truth matrix $G_{vl}^*$, we see that $\bar{G}_v^\top$ is aiming to inverting the map.
In addition, we say the teacher has $\epsilon_{v*l}^n$ cross modal error
\begin{align*}
   \frac{1}{|S|}\| \sum_{\vx^{vl} \in S} \bar{G}_v^\top \vx^v (\vx^l)^\top \Bar{G}_l - \sum_{\vx^{vl} \in S} \vz^v (\vz^l)^\top \|_*  \leq \epsilon_{v*l}^n
\end{align*}
When all $\epsilon_v^n, \epsilon_l^n, \epsilon_{v*l}^n \to 0$ as $n \rightarrow \infty$, then we say the teacher is strong for both modalities. But it might also be possible that only one modal, for example, visual is strong. That is $\epsilon_v^n \to 0,  \epsilon_l^n, \epsilon_{v*l}^n \gg \epsilon_v^n$.
% \footnote{It is possible to represent $\epsilon_{v*l}^n$ using $\epsilon_v^n, \epsilon_l^n$. However, our primary objective in this section is to conceptually interpret our empirical results. Therefore, we will maintain this simpler version for ease of understanding.}




\paragraph{Model and training.} 
According to Lemma 4.1 in \citep{nakada2023understanding}, using the CLIP loss to optimize the linear model has approximately the same training dynamics as using the regularized linear loss. Therefore, here we assume that we are learning $G_v, G_l$ by maximizing the clip score gap between the contrastive pairs, plus a regularizer, 
\begin{align*}\label{eq:linearloss}
    \min_{G_v, G_l} \gL_S^\rho (G_v, G_l)
    % & := \min_{G_v, G_l} \frac{\sum_{i \in S} \sum_{j \in S \setminus \{i\}}(s_{ij} - s_{ii})}{n(n-1)} 
    % + R(G_v, G_l) 
    := \min_{G_v, G_l} \frac{\sum_{i \in S} \sum_{j \in S}(s_{ij} - s_{ii})}{|S|(|S|-1)} 
    +  \frac{\rho}{2}\frac{|S|}{|S|-1}\|G_vG_l^\top\|_F^2
\end{align*}
where  $s_{ij} := \langle  G_v^\top \vx^v_i, G_l^\top \vx^l_j \rangle$ and $\rho > 0$ is some regularizer-related \textit{constant}.
Note that this objective maximizes self-similarity and minimizes similarity between disparate pairs. 
Note that this ``loss'' can be negative, avoiding the trivial null solution of all zeros. 
We denote this training process from any given $S$ as $G_{vl} = \gA^\rho(S)$.


\paragraph{Goal and metric.} 
Under the same principle as our training loss function, we measure the performance of any learnt $G_v, G_l$ on some downstream task with distribution $\gD_\text{target}$ as test loss $\gL_{\text{target}} (G_v, G_l):=$
\begin{align*} 
     \E_{\substack{\vx^{vl}\sim \gD_\text{target}\\\vx^{vl}_2 \sim \gD_\text{target}}} (\langle G_v^\top\vx^v, G_l^\top\vx_2^{l}\rangle- \langle G_v^\top\vx^v, G_l^\top\vx^l\rangle) 
\end{align*}
% Here $ \gD_\text{target}^\epsilon$ denotes the discretized $\epsilon$-covering of continuous distribution  $ \gD_\text{target}$. 
% \yifang{TODO: Simon can you check if this notation is right ? or can we just use $\E_{\vx^{vl} \sim \gD_\text{target}} \E_{\vx^{vl}_2 \sim \gD_\text{target}}$}
This is inspired by the following classification accuracy. Assume that the test data including $C$ class, and the class distribution is $\mathcal{C}$. For every class $c$, the training data $\vx = (\vx^v, \vx^l)$ satisfies distribution $\mathcal{P}_c$. We further assume the corresponding classification templates are $\{\vx_c\}_{c=1}^C$. Thus we define classification accuracy as
% \begin{equation*}
%     \text{AC}(G_v, G_l) = \E_{c \sim \mathcal{C}}\left[\E_{\vx_i \sim \mathcal{P}_c}\mathbf{1} [s_{ic} > \max_{c' \neq c }\{s_{ic'}\}]\right]
% \end{equation*}
\begin{equation*}
    \text{AC}(G_v, G_l) = \E_{c,c' \sim \mathcal{C} \times  \mathcal{C}}\left[\E_{\vx_i \sim \mathcal{P}_c} \mathbf{1}[s_{ic} > s_{ic'}]\right]
\end{equation*}
Therefore our goal is to minimize its gap between the best hind-side subset, for any $\rho$, without budget constraints,
\begin{align*}
    \Delta^\rho(S) = \gL_\text{target}(\hat{G}_{vl}) - \min_{S' \in D_\text{train}} \gL_\text{target}(\gA^\rho(S')), \hat{G}_{vl} = \gA^\rho(S)
\end{align*}
\vspace{-1em}
% We will show that it's connected to the classification accuracy. Assume that there are T tasks distribution over $D_\text{task}$,  each task a binary class, and the class distribution is $C_t$. For every class $c \in \{0,1\}$, the training data $\vx = (\vx^v, \vx^l)$ satisfies distribution $\mathcal{P}_c^t$. We further assume the corresponding classification templates are $\mathcal{A}_C :=\{\vx_c\}_{c=1}^C$. And we defined classification accuracy as
% \begin{equation*}
%     \text{AC}(G_v, G_l) = \E_{t \sim D_\text{task}}\E_{c \sim C_t}\left[\E_{\vx_i \sim \mathcal{P}_c^t}\Pr (s_{ic} > \max_{c' \neq c }\{s_{ic'}\})\right]
% \end{equation*}
% Therefore let $\hat{G}_{vl}$ be the learnt representation from our selected subset $S$ and the $G_{vl}^{\text{random}}$ be the one from a random sampled subset under the same budget, our goal is to maximize
% \begin{align*}
%     \Delta(S) = \gL_\text{target}(\hat{G}_{vl}^{\text{random}}) - \gL_\text{target}(\hat{G}_{vl})
% \end{align*}
% \kevin{So we're committing to compariing ourselves to an IID sample versus the ``best'' subset? This leaves us somewhat vulnerable to the criticism that the CLIP screening could perform even better we just don't know} \yifang{Working on it}

% \yifang{I think another way to write this is as follows.}
% {
% \color{olive}

% Instead of define $\Sigma_\text{best}$ as in the current lemma, we define it as
% \begin{align*}
%         & \Sigma_\text{best} = \argmax_{\Sigma} [\Tr \left( \Sigma_{\text{target}}\Sigma \right)
%             - \frac{...}{\sqrt{|S|}}]\\
%         \text{s.t.} \quad 
%         & \Sigma = \frac{1}{|S|}\sum_{\vz^{vl} \in S} \vz^v (\vz^l)^\top,
%           S\subset D_{train}.
% \end{align*}
% here $-\frac{...}{\sqrt{|S|}}$ comes from noisy $\xi$. In this case we are considering all the possible subset without fixing budget. But we can argue that the first term will decrease when the $-\frac{...}{\sqrt{|S|}}$ increase but with decreasing increase rate. So after surpassing certain $|S|$ budget, the first term become dominating and we can regard this as a fixed budget subset selection problem.
% }
\vspace{-1em}
\subsection{Generalization Guarantees}

We now provide theoretical guarantees and postpone our proof into Appendix~\ref{app: proof}.
\textbf{Firstly, we are going to prove the intuition behind \twonormsim score.} 
% by decomposing $\Delta(S)$ into the error from strategy term where \twonormsim comes from and the unavoidable terms from the natural hardness of the problem itself.

\begin{lemma}[Intuition behind \twonormsim]
\label{lem: main}
    With high probability at least $1-\frac{1}{|S|d}$, suppose the  hind-side best subset has at least $\underline{n}$ number of samples, then we have 
    % \begin{align*}
    %     \Delta^\rho(S) 
    %     &= \underbrace{\frac{1}{\rho}\max_{S' \in D_\text{train}} \left( \Tr\left( \Sigma_{\text{target}} (\Sigma_{S'} - \Sigma_{S}) \right) \right)}_\text{\twonormsim related term}\\
    %     & + \quad \underbrace{\gO \left(\sqrt{\frac{d\log(d|S|)}{\underline{n}}} + \sqrt{\frac{d\log(d|S|)}{|S|}}\right)}_\text{noise}
    % \end{align*}
    \begin{align*}
        \Delta^\rho(S) 
        &= \underbrace{\frac{1}{\rho}\max_{S' \in D_\text{train}} \left( \Tr\left( \Sigma_{\text{target}} (\Sigma_{S'} - \Sigma_{S}) \right) \right)}_\text{\twonormsim related term}+ \quad \underbrace{\gO \left(\sqrt{\frac{d\log(d|S|)}{\underline{n}}} + \sqrt{\frac{d\log(d|S|)}{|S|}}\right)}_\text{noise}
    \end{align*}
\end{lemma}

\begin{proof} [Proof sketch]
% (Sketch version)\\
    \ding{182} Under the assumption that both $\vz^{vl}, \xi_{vl}$ is zero-mean, maximizing the clip score gap is equivalent to maximizing the clip score of the same sample. 
    \vspace{-3px}
    \begin{align*}
         \gL_{\text{target}} (\hat{G}_v, \hat{G}_l):= - \E_{\vx^{vl} \sim \vD_\text{target}}\langle \hat{G}_v^\top\vx^v, \hat{G}_l^\top \vx^l \rangle
    \end{align*}
    \ding{183} By minimizing the regularized training loss $\gL_S^\rho (G_v, G_l)$ using Eckart-Young-Mirsky Theorem, we get a closed form solution of $\hat{G}$ as 
    \vspace{-3px}
    \begin{align*}
        \hat G_v \hat G_l^\top \approx \frac{1}{\rho} G_v^* \Sigma_S \cdot (G_l^*)^\top + \text{noise depend on $S$}
    \end{align*}
     \ding{184} Combining the result in \ding{183} and \ding{182}, we have 
     \vspace{-3px}
    \begin{align*}
        & \gL_{\text{target}} (\hat{G}_{vl}) \approx  - \frac{1}{\rho}\Tr\left( \Sigma_{\text{target}}\Sigma_S \right) -\text{noise depend on $S$}
    \end{align*}
    The same analysis can be applied on $\min_{S' \in D_\text{train}} \gL_\text{target}(\gA(S'))$ as well. Rearranging these two equations gives us the final result.
\end{proof}

This lemma shows the the $\Delta(S)$ is depend on the \twonormsim-related term and the noise term which comes from $\xi$. When $\underline{n}$ and $|S|$ is large enough, then the \twonormsim-related term will become dominant. This aligns with our practice experience that the final performance is less sensitive to the small variation in the number of select data as long as that is sufficient.
% 
Moreover, in some special cases where test distribution has identity cross-variance, then sampling by greedily choosing CLIP score might be enough.

\textbf{Now we are ready to give a proof on the choice of $\bar{\Sigma}_{\text{target}}$ and visual-only information.}
Specifically, the strategy error mainly comes from (1). The unknown test distribution shift from training. (2). The unobservable ground truth $\Sigma_S$. To tackle error (1), we assume some prior knowledge on test by using the proxy test variance $\bar{\Sigma}_{\text{target}}$. To tackle the error (2), there are two possible solutions as shown below. Based on the theoretical interpretation, we should choose different strategy based on the property of the teacher embedding model.
\vspace{-5px}
\begin{align*}
    & S_{\text{vision+language}} = \argmax_{S} \Tr\left(\bar{\Sigma}_{\text{target}} (\sum_{\vx^{vl} \in S} \bar{G}_v^\top \vx^v (\vx^l)^\top \Bar{G}_l) \right)  \\
    &  S_{\text{vision only}} = \argmax_{S} \Tr\left(\bar{\Sigma}_{\text{target}} (\sum_{\vx^{vl} \in S} \bar{G}_v^\top \vx^v (\vx^v)^\top \Bar{G}_v) \right)
\end{align*}


\begin{theorem}[Main] 
\label{them: main}
    Under the assumption of Lemma~\ref{lem: main},
    \begin{align*}
       \Delta^\rho(S)
        & \leq \text{noise} +  \frac{1}{\rho}\|\bar{\Sigma}_{\text{target}} - \Sigma_{\text{target}} \| \|\Sigma_S - \Sigma_{\text{best}}\|_* \\
        & + \frac{1}{\rho}
        \begin{cases}
            \epsilon_{v * l}^S  \quad \text{(vision+language)} \\
            \epsilon_v^S +  \sqrt{1 - \frac{1}{|S|}\sum_{i \in [S]} \langle \vz^v,\vz^l \rangle)} \quad \text{(vision only)}
        \end{cases}
    \end{align*}
\end{theorem}

Firstly, it is evident that the greater the difference between $\bar{\Sigma}_{\text{target}}$ and $\Sigma_{\text{target}}$, the less improvement we can expect. Moreover, in scenarios where $\epsilon_l$ is large (indicating lower accuracy in the language part) while $\epsilon_v$ is small (indicating higher accuracy in the vision part), it may be advisable to opt for vision-only embeddings.
% 
However, the learner should also consider the term $\sqrt{1 - \frac{1}{|S|}\sum_{i \in S} \langle \vz^v, \vz^l \rangle}$, which represents the alignment between the ground truth visual and language latent vectors, essentially reflecting the intrinsic quality of the data. If this term is already significant, relying solely on vision information as a proxy for language information could lead to suboptimal results.





\iffalse
Now we are ready to show the main advantage of our strategy compared to the random sampling. We start with the case that teacher model can recover both $\vz^v,\vz^l$ with low error $\epsilon_{vl} \to 0$ in Theorem~\ref{them: main strong teacher}. In this case, we shall use clip embedding form both image and text. Nevertheless, our empirical result \yifang{cite} shows that using clip embedding from both modal performs much worse than using image embedding only. We further interpret this phenomena in Theorem~\ref{them: main weak teacher}.

\begin{theorem}[Results under a strong teacher]
\label{them: main strong teacher}
    Let $\hat{G}_{vl}$ be the learnt representation from our selected subset $S$ and the $G_{vl}^{\text{random}}$ be the one from a random sampled subset under the same budget. We have that, \yifang{with high prob?}
    \begin{align*}
        &\gL(\hat{G}_{vl}^{\text{random}}) - \gL(\hat{G}_{vl}) \\
        &\geq \underbrace{\Tr \left( \Sigma_{\text{target}}(\Sigma_{\text{best}} - \Sigma_{\text{train}}) \right) }_{\text{best possible improvement}}
            + \underbrace{\Tr \left( \Sigma_{\text{target}}(\Sigma_S - \Sigma_{\text{best}}) \right) }_{\text{err from test distribution shits}} \\
        &\quad - \underbrace{\text{\yifang{TODO}}}_{\text{noise error}} 
          - \underbrace{\text{\yifang{TODO}}}_{\text{err from teacher model}}
    \end{align*}
    where $\Sigma_S = \frac{1}{|S|}\sum_{\vz^{vl} \in S} \vz^v (\vz^l)^\top$ is the variance of chosen subset $S$ and $\Sigma_\text{best}$ is the variance best subset we could choose under the same budget. Formally, it is defined as: 
    \begin{align*}
        & \Sigma_\text{best} = \argmax_{\Sigma} \mathrm{tr\left( \Sigma_{\text{target}}\Sigma \right)} \\
        \text{s.t.} \quad 
        & \Sigma = \frac{1}{|S'|}\sum_{\vz^{vl} \in S'} \vz^v (\vz^l)^\top,
          S' \subset D_{train}, |S'| = |S|
    \end{align*}
\end{theorem}

\paragraph{Discussion} 
\yifang{How test distribution affect}

\yifang{How quality $\text{Trace}(\Sigma)$ affect}

\yifang{Budget lower bound}

Above result will become meaningless when $\epsilon_l$ becomes larger. Fortunately, we are able to \textit{largely} reduce the error from teacher model in the sacrifice of a slightly increased error from test distribution shifts.

\begin{theorem}[Results under weak language modal teacher (Main)]
\label{them: main weak teacher}
    
\end{theorem}



\yifang{===== Below TODO ======}

Following \citep{nakada2023understanding, ji2023power}, we choose $R(G_1, G_2) = (\rho/2)\|G_1G_2^\top\|_F^2$ for some $\rho > 0$, which allows us to use Eckart-Young-Mirsky theorem [XXX] (Details in Appendix XXX) directly, and we can obtain the following closed-form solution
\begin{lemma}[Informal]\label{lemma:EYM}
    Let
    \begin{equation}
        \hat G_1, \hat G_2 = \arg \min_{G_1, G_2 \in \R^{d\times r}}\mathcal{L}(G_1,G_2)
    \end{equation}
    Then we have
    \begin{equation}
        \hat G_1 \hat G_2^\top = \frac{n}{\rho(n-1)}G_1^*V \cdot\Sigma\cdot V^\top (G_2^*)^\top + \text{noise}
    \end{equation}
    where
    \begin{equation}
        \Sigma :=\frac{1}{n}\sum_{l=1}^n\vy_i^{(1)}(\vy_{i}^{(2)})^\top
    \end{equation}
\end{lemma}

So the key points for improving the generalization error of $\hat G_1 \hat G_2^\top$ is to obtain benign $\Sigma$. If for any data point, $\vy^{(1)}$ aligns with $\vy^{(2)}$ well, then $\Sigma$ can be well diagonal and the generalization error is low. However, in the large scale training scenario of image-text foundation models, the data are always curated from web and thus low-qualitied, so the unfiltered dataset will result in non-diagonal terms in $\Sigma$ and performs badly. To formalize the context, we define:

\begin{definition}[Excess Risk]
    The excess risk on the test distribution is \yiping{If this definition is fine?}
    \begin{equation*}
        % E(G_1, G_2) = \E_{
        %     (\vx_i^{(1)},\vx_i^{(2)}), (\vx_j^{(1)},\vx_j^{(2)}) \sim \mathcal{P}^{te}_{X^2}
        % }[(s_{ij} - s^*_{ij})^2]
        ER(G_1, G_2) = \frac{1}{2}\E_{
            \vw_i, \vw_j\sim \mathcal{P}^{te}_{X^2}
        }\left[(s_{ij} - s^*_{ij})^2 + (s_{ji} - s^*_{ji})^2\right]
    \end{equation*}
\end{definition}
Then if we choose $\rho = n/(n-1)$, and note that the data generation for the two modality are symmetric, and thus $\Sigma$ is symmetric with high probability, then we can obtain
\begin{equation}\label{eq:ERapprox}
    ER(\hat G_1, \hat G_2) \approx 
    \mathop{\E}_{\vw_i, \vw_j\sim \mathcal{P}^{te}_{X^2}} [(\vy_i^{(1)})^\top (\Sigma - I_r)\vy_j^{(2)}]^2 
\end{equation}
% where $\vy^{(l)}$ is defined in Lemma~\ref{lemma:EYM}. 
Then from (\ref{eq:ERapprox}), we know that minimize the absolute value of the terms in the top left block of matrix $\Sigma - I_r$ will be more important than others because those terms corresponding to more frequently sampled features.

\yiping{TODO: Add another measurement to mimic imagenet classification error. Show that balance class can still be beneficial by maximize the cond}

\yiping{Maybe the results can be generalized to the case where the features of \textbf{downstream tasks} are give?}
\section{}

\fi



\iffalse
Define $\vx, \vy \in \R^d$ be the image and text inputs, and $\hat f, \hat g : \R^d \rightarrow \R^r$ as the image and text encoders, respectively. And we use $\vf_i := \hat{f}(\vx_i)/\|\hat{f}(\vx_i)\|_2$ to denote the normalized embedding for the $i$-th image inputs, and similar notation for $\vg_i$. Further let $\alpha_{ij} = \vf_i^\top \vg_j$ be the pairwise cosine similarity and $\beta_{ij} = \exp(\alpha_{ij}/\tau)$ be its exponentiation of with fixed temperature parameter $\tau$. Then we can then write the CLIP loss as
\begin{equation}\label{eq:CLIPloss}
    \mathcal{L} = -\frac{\tau}{2}\sum_{i=1}^n\left[\log(\frac{\beta_{ii}}{\sum_{j=1}^n\beta_{ij}})+\log(\frac{\beta_{ii}}{\sum_{j=1}^n\beta_{ji}})\right]
\end{equation}
We assume that the multi-modal data is generated by two different linear mapping with the same latent variables $\vz \in \R^r$, i.e.,
\begin{equation}
    \vx = F^* (\vz + \vvxi^{x}), \quad \vy = G^* (\vz + \vvxi^{y})
\end{equation}
where $F^*, G^* \in O_{d\times r}$ has orthonormal columns and $\vvxi^x, \vvxi^y \sim \mathcal{N}(0, \sigma^2 I_r), \sigma \ll 1$ are independent random noise. This assumption is widely used in previous works~\citep{XXX}.
Further, we use linear model  $\hat f(\vx) := \hat F^\top\vx, \hat g(\vy) := \hat G^\top\vy$ where $\hat F, \hat G \in \R^{d\times r}$, to minimize the contrastive loss. We use stochastic gradient descent with all the data in a batch to update the parameters, i.e., 
\begin{equation*}
    \hat F(t+1) = \hat F(t) - \frac{\eta}{n}\sum_{i=1}^n \vx_i(\left.\frac{\partial \mathcal{L}}{\partial \hat f(\vx_i)}\right|_t)^\top
\end{equation*}
\begin{equation*}
    \hat G(t+1) = \hat G(t) - \frac{\eta}{n}\sum_{i=1}^n \vy_i(\left.\frac{\partial \mathcal{L}}{\partial \hat g(\vy_i)}\right|_t)^\top
\end{equation*}

\section{Main Motivation}
We must mention that \emph{minimizing (\ref{eq:CLIPloss}) doesn't mean learning the ground truth head $F^*, G^*$}.
A simple example is  considering the case with $n=r$ samples for training, where $\vz_i = \ve_i, i \in [r-1]$ and $\vz_r = (1-\varepsilon)\ve_{r-1} + \varepsilon\ve_r$, $\varepsilon \ll 1$. It's clear that if $\hat F = F^*, \hat G = G^*$, we will have $\beta_{r-1,r}, \beta_{r,r-1}\approx \beta_{r-1,r-1}$, which means that $r-1$-th and $r$-th samples are confusing to the model. However, we can always find some rank-$r$ linear matrix $(\hat F)^\top F^*, (\hat G)^\top G^*$ to map any $r$ vectors onto $r$ orthogonal vectors, which means the learner $\hat F, \hat G$ can separate all the samples well and further minimize the CLIP loss. \yifang{I think it would be better to clearly define what is a good representation ? For example, previous work define a bad representation by saying under all possible linear classifier (the linear head), it is impossible to get good acc.}
\yiping{Yes, intuitionally the repr function that maps the input from different classes into a more separate space will have better downstream performance. I will add it soon. }

Following this observation, our motivation is that not all the classes are evenly distributed in the embedding space generated by the OpenAI CLIP model.\yiping{Need visualization}. Classes with many similar features are always generated by close latent variables, which will result in similar embeddings and take a much longer time for the learners to separate each other. This can happen even when the image and text encoders are perfectly aligned.

\begin{assumption}[Data Classes]\label{ass:classes}
Assume we have $r$ different classes and the sample number in the $i$-th class is $n_i$, so $n = \sum_i^r n_i$. The classes are determined by $r$ different latent variables $\{\bar\vz_{i}\}_1^{r}$ satisfies:  $\bar\vz_r := (1-\varepsilon)\bar\vz_{r-1} + \varepsilon\bar\vz'$, $\{\bar\vz_1, \ldots, \bar\vz_{r-1}, \bar\vz'\}$ are orthonormal vectors.
\end{assumption}
\begin{theorem}
    \yiping{Need further calculation}(Informal) Assume Assumption~\ref{ass:classes} holds with parameters $\{n_i\}_1^r, \varepsilon$. Then if $\hat F(0)^\top F^* \approx \hat G(0)^\top G^*$\yiping{This assumption should not be necessary}, we claim that $\hat F(t)^\top F^*\approx \hat G(t)^\top G^*$, $\alpha_{r,r-1}, \alpha_{r-1,r}$ decreasing in the rate of $O(\varepsilon\cdot(n_{r-1}+n_{r})/{n})$, while for all other $\alpha_{i,j}, i\neq j$, their decreasing rate is $O((n_{i}+n_{j})/{n})$
\end{theorem}

\yiping{Add class definition. $n_i$ is the number of samples for class $i$.}
\fi



% Acknowledgements should only appear in the accepted version.
% \section*{Acknowledgements}

% \textbf{Do not} include acknowledgements in the initial version of
% the paper submitted for blind review.

% If a paper is accepted, the final camera-ready version can (and
% probably should) include acknowledgements. In this case, please
% place such acknowledgements in an unnumbered section at the
% end of the paper. Typically, this will include thanks to reviewers
% who gave useful comments, to colleagues who contributed to the ideas,
% and to funding agencies and corporate sponsors that provided financial
% support.


% In the unusual situation where you want a paper to appear in the
% references without citing it in the main text, use \nocite

% \nocite{langley00}


==> icml_content/abstract.tex <==
\begin{abstract}
In recent years, data selection has emerged as a core issue for large-scale visual-language model pretraining, especially on noisy web-curated datasets. One widely adopted strategy assigns quality scores such as CLIP similarity for each sample and retains the data pairs with the highest scores. However, these approaches are agnostic of data distribution and always fail to select the most informative samples. 
To solve this problem, we propose a simple yet theoretically principled metric named \textbf{V}ariance \textbf{A}lignment \textbf{S}core (\textsf{VAS}), which has the form $\langle \Sigma_{\text{test}}, \Sigma_i\rangle$.
Here, $\Sigma_{\text{test}}$ represents the target (cross-)covariance matrix we aim to align, potentially based on prior knowledge, while $\Sigma_i$ denotes the tensor product of single or multi-modal representations for the $i$-th sample.
We further design a new data selection method that maximizes the total \textsf{VAS}.
We provide theoretical analysis in a simplified setting to demonstrate the theoretical advantage of \textsf{VAS} over random or other existing data selection.
Experimentally, applying VAS and CLIP scores together can outperform baselines by a margin of $1.3\%$ average on 38 evaluation sets for noisy dataset DataComp and $2.5\%$ on VTAB for high-quality dataset CC12M. Additionally, our ablation study also shows visual features are better than text for calculating VAS, and the related classical experimental design methods may fail under this context.
\end{abstract}

==> icml_content/conclusion.tex <==
\section{Conclusion}
In the paper, we propose a Variance Alignment Score (VAS) to measure the informativeness of each sample and show that VAS is a parallel metric to image-text alignment focused score like CLIP score. Based on VAS, we design a informative + quality focused strategy that achieves the best average performance over 38 downstream test tasks compared to various existing baseline. Moreover, we also provide a theoretical guarantees to explain the intuition behind our strategy.

==> icml_content/experiment_results.tex <==


% \begin{table}[h]
% \centering
% \caption{}
% \label{tab:example}
% \begin{tabular}{|c|c|}
% \hline
% \multirow{2}{*}{yyc} & 1 \\ \cline{2-2}
%  & 2 \\ \hline
% 3 & 4 \\
% \hline
% \end{tabular}
% \end{table}

\begin{table*}[ht]
\small
\centering
\vspace{-1em}
\caption{Results on DataComp. Comparison of performance of VAS filtering with data filtering methods presented in \cite{gadre2023datacomp} and $\mathbb{D}^2$\cite{maharana2023d2}. The number after the evaluation dataset means the number of tasks contained in this class. Higher is better. Here we compare the results under any dataset size. VAS(X) means using the variance matrix from datasets X. 
% \yifang{How about put VAS(ImageNet-1K) into the ablation study part? and only how the final valid results here ?} \yiping{ok, TODO}
}
\vspace{0.3em}
\label{tab:datacomp}
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}{*}{
\textbf{Filtering Strategy}} & \textbf{Dataset} & \textbf{ImageNet} & \textbf{ImageNet Dist. Shift} & \textbf{VTAB} & \textbf{Retrieval} & \textbf{Average} \\
 & \textbf{Size} & (1 sub-task) & (5) & (11) & (3) & (38)\\
\midrule
No filtering  & 12.8M & 2.5 & 3.3 & 14.5 & 10.5 & 13.2 \\
Text-based filtering  & 3.2M & 4.6 & 5.2 & 16.9 & 11.2 & 15.6 \\
Image-based filtering  & 3.0M & 4.3 & 4.7 & 17.8 & 11.2 & 15.8 \\
% \rowcolor[HTML]{EFEFEF} 
CLIP score (30\%)  & 3.8M & {5.1} & {5.5} & 19.0 & 10.8 & 17.2 \\
$\mathbb{D}^2$ Pruning (image+text)  & 3.8M & {5.1} & {5.6} & {18.2} & {11.7} & 17.0 \\
Image-based $\cap$ CLIP score (30\%) & 1.4M& 3.9& 4.5& 16.2& 8.9 & 14.4\\
% Image-based filtering \cite{gadre2023datacomp} (reproduced) & 3.0M & 4.1 & 4.6 & 17.5 & 11.6 & 15.7 \\
\midrule
CLIP score (30\%, reproduced) & 3.8M & {4.8} & 5.3 & 17.1 & 11.5 & 15.8 \\
Image-based $\cap$ CLIP score (45\%)  & 1.9M & 4.2 & 4.6& 17.4& 10.8 & 15.5 \\
$\mathbb{D}^2$ Pruning (image+text, reproduced) & 3.8M & 4.6 & 5.2 & {18.5} & 11.1 & 16.1 \\
CLIP score (45\%) & 5.8M & 4.5 & 5.1 & 17.9 & \textbf{12.3} & 16.1 \\
\midrule
\textbf{VAS} (ImageNet-1k) %\yiping{Need place this here?}
& 3.8M & 2.4& 3.1& 14.9& 10.4& 12.7 \\
\textbf{VAS} (ImageNet-1k) $\cap$ 
CLIP score 
(45\%) 
& 3.8M & \textbf{5.2} & \textbf{5.5} & \underline{19.0} & \underline{12.2} & \textbf{17.4} \\
% \textbf{VAS} (DataComp) & 3.8M & & & & & \\
\textbf{VAS} (DataComp) $\cap$ CLIP score 
(45\%)
& 3.8M & \underline{5.0} & \underline{5.4} & 17.9 & {12.1} & 16.2\\
% \textbf{VAS-D} (DataComp) & 3.8M & & & & & \\
\textbf{VAS-D} (DataComp) $\cap$ CLIP score 
(45\%) 
& 3.8M & 4.7 & \underline{5.4} & \textbf{19.7} & {11.7} & \underline{17.3} \\
\bottomrule
% \textsuperscript{D}2 PRUNING (image only) & 3.8M & 4.4 & 5.1 & 16.9 & 12.1 & 15.9 \\
% \textsuperscript{D}2 PRUNING (text only) & 3.8M & 4.9 & 5.5 & 17.0 & 12.3 & 16.6 \\ \bottomrule
\end{tabular}
\vspace{-1em}
\end{table*}


\begin{table*}[ht]
\small
\centering
\caption{Results for coreset selection on the high-quality dataset CC12M. Comparison of VAS filtering performance with data filtering methods presented in \cite{gadre2023datacomp} and $\mathbb{D}^2$\cite{maharana2023d2}. The number after the evaluation sets means the number of tasks contained in this class. Higher is better. And we compare the results under $2.8$M dataset size. VAS(X) means using the variance matrix from datasets X. }
\vspace{0.3em}
\label{tab:cc12m}
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}{*}{
\textbf{Filtering Strategy}} & \textbf{Dataset} & \textbf{ImageNet} & \textbf{ImageNet Dist. Shift} & \textbf{VTAB} & \textbf{Retrieval} & \textbf{Average} \\
 & \textbf{Size} & (1 sub-task) & (5) & (11) & (3) & (38) \\ \midrule
No filtering & 9.2M & 9.3 & 8.5 & 21.3 & 19.6 & 20.2 \\
% Text-based filtering \cite{gadre2023datacomp} & 9.2M & 9.3 & 8.5 & & & 20.2  \\
% Image-based filtering \cite{gadre2023datacomp} & 9.2M & 9.3 & 8.5 & & & 20.2  \\
% % \rowcolor[HTML]{EFEFEF} 
% CLIP score (30\%) \cite{gadre2023datacomp} & 2.8M & 7.8 & 7.4 & & & 17.3  \\
% $\mathbb{D}^2$ Pruning \cite{maharana2023d2} & 9.2M & 9.3 & 8.5 & & & 20.2  \\
% \midrule
CLIP score (50\%) & 4.6M & 7.8 & 8.7 & 20.3 & 18.0 & 18.8  \\
\midrule
CLIP score (30\%) & 2.8M & 7.8 & 7.4 & 18.8 & 15.2 & 17.3  \\
Image-based $\cap$ CLIP score (50\%)  & 2.6M & \textbf{10.6} & \textbf{9.0} & 20.0 & \textbf{16.8} & 19.1  \\
$\mathbb{D}^2$ Pruning (image+text) & 2.8M & 7.2 & 7.2 & {19.3} & 13.8 & 17.3 \\
\midrule
\textbf{VAS} (ImageNet-1k) & 2.8M & {9.6} & {8.5} & {20.4} & \underline{16.6} & {18.6}  \\
\textbf{VAS} (ImageNet-1k) $\cap$ CLIP score (50\%) & 2.8M & {9.7} & {8.7} & \underline{22.1} & {16.0} & \textbf{19.5}\\

% \textbf{VAS} (CC12M) & 2.8M & & & & &\\
\textbf{VAS} (CC12M) $\cap$ CLIP score (50\%) & 2.8M & {9.1} & {8.5} & {21.3} & {15.9} & \underline{19.2}  \\
% \textbf{VAS-D} (CC12M) & 2.8M & & & & &\\
\textbf{VAS-D} (CC12M) $\cap$ CLIP score (50\%) & 2.8M & \underline{9.9} & \underline{8.9} & \textbf{22.5} & 16.2 & \textbf{19.5}  \\
\bottomrule
% \textsuperscript{D}2 PRUNING (image only) & 3.8M & 4.4 & 5.1 & 16.9 & 12.1 & 15.9 \\
% \textsuperscript{D}2 PRUNING (text only) & 3.8M & 4.9 & 5.5 & 17.0 & 12.3 & 16.6 \\ \bottomrule
\end{tabular}
\vspace{-0.6em}
\end{table*}


\begin{table*}
\small
\centering
\caption{Ablation Study on the VAS and its variants on DataComp. All experiments commence by filtering out the top 45\% of data based on the CLIP score, followed by corresponding approaches to obtain 3.8M data.``image'' or ``text'' means using the variance of image or text embeddings to represent  $\bar\Sigma_{\text{test}}$, and ``image $\times$ text'' means representing $\bar\Sigma_{\text{test}}$ with the cross-covariance of image and text embeddings.}
\vspace{0.3em}
\label{tab:abla}
\begin{tabular}{@{}lccccc@{}}
\toprule
\textbf{Filtering Strategy} $\cap$ CLIP score (45\%)  &  \textbf{ImageNet} & \textbf{ImageNet Dist. Shift} & \textbf{VTAB} & \textbf{Retrieval} & \textbf{Average} \\ \midrule
Random Sampling & 4.2& 4.9& 17.2& 11.6& 15.6\\ \midrule
\textbf{VAS} (ImageNet-1k, image)  & \textbf{5.2} & \textbf{5.5} & \underline{19.0} & \textbf{12.2} & \textbf{17.4} \\
\textbf{VAS} (ImageNet-1k, text) & 3.9& 4.2& 16.3& 11.3& 14.9\\
\textbf{VAS} (ImageNet-1k, image $\times$ text) & 4.3& 4.9& 17.5& 11.8& 15.9\\
\midrule
\textbf{VAS} (DataComp, image) &  \underline{5.0} & \underline{5.4} & 17.9 & \underline{12.1} & 16.2 \\
\textbf{VAS} (DataComp, text) & 3.6& 4.1& 17.2& 10.9& 15.2\\
\textbf{VAS} (DataComp, image $\times$ text) & 4.0 & 4.6& 17.6& 11.7& 15.7\\
\midrule
\textbf{VAS-D} (DataComp, image) & 4.7 & \underline{5.4} & \textbf{19.7} & {11.7} & \underline{17.3} \\
\textbf{VAS-D} (DataComp, text) & 3.5 & 4.1& 16.7& 11.1& 15.4\\
\textbf{VAS-D} (DataComp, image $\times$ text) & 3.6& 4.2& 18.4& 11.1& 15.8\\
% \midrule
% \textbf{min-VAS} (ImageNet-1k, image) & 3.8M & 2.8& 3.5& 15.3& 9.9& 13.7\\
% \textbf{min-VAS} (ImageNet-1k, text) & 3.8M & 4.2& 4.8& 17.2& 11.8& 15.0\\
% \textbf{min-VAS} (ImageNet-1k, image $\times$ text) & 3.8M & 3.5& 4.0& 16.2& 10.7& 14.7\\
% \textbf{min-VAS-D} (DataComp, image) & 3.8M & 3.4 & 4.2 & 16.4 & 10.8 & 15.1 \\
% \textbf{min-VAS-D} (DataComp, text) & 3.8M & 4.6& 5.2& 17.1& 11.2& 16.3\\
% \textbf{min-VAS-D} (DataComp, image $\times$ text) & 3.8M & 3.9& 4.4& 15.8& 10.7& 14.8\\
\bottomrule
\end{tabular}
\vspace{-1em}
\end{table*}
\vspace{-0.5em}
\section{Experiments}
\label{sec: experiment}
In this section, we evaluate the performance of the VAS-based strategy in Algo.~\ref{algo: main}. We first show the effectiveness of our ultimately proposed strategy and then present our ablation study result to further validate our three key designs. Please refer to Appendix~\ref{sub: algo details} for the implementation details and Appendix~\ref{sub: hyperp} for the discussion of why our algorithm can be used with little or no hyperparameter tuning.
\vspace{-0.8em}
\subsection{Setup}
\paragraph{Training Configurations.} 
We adhere to the standardized training and evaluation procedures as outlined in Datacomp~\cite{gadre2023datacomp}, considering two distinct training datasets. One is small-scale DataComp set, which provides a substantial dataset comprising 12.8 million low-quality, web-curated image-text pairs. Another is CC12M~\cite{changpinyo2021conceptual}, which offers a collection of 12 million high-quality image-text pairs.
Our comparative setup varies across these two datasets:
(1) Within the DataComp framework, our objective is to maximize model performance, without imposing a fixed dataset size constraint. Conversely, (2) for CC12M, where data quality is generally high and its removal could potentially degrade model performance, our focus shifts to the \textit{subset selection} challenge, which comparing the strategy under the same budget (approximately 2.8 million in our experiment)\footnote{Owing to the limitations of the heuristic method `Image-based filtering' cited in \cite{gadre2023datacomp} in controlling subset size, the size for the `Image-based filter $\cap$ CLIP score method (50\%)' is marginally below 2.8 million, as detailed in Tab.~\ref{tab:cc12m}}. Details in Appendix~\ref{sub: config}.
\vspace{-0.8em}
\paragraph{Evaluation Datasets.} 
We evaluate our model on 38 datasets related to image classification and retrieval tasks adopted in DataComp. The image classification tasks 
% vary from visual recognition to distance prediction, 
contain ImageNet-1k~\cite{deng2009imagenet}, ImageNet distribution shifts~\cite{wang2019learning,pmlr-v97-recht19a,hendrycks2021natural,hendrycks2021many}, 11 datasets from the Visual Task Adaptation Benchmark (VTAB)~\cite{zhai2019large} and 3 datasets from  WILDS~\cite{koh2021wilds, sagawa2021extending}, which tests the robustness facing subpopulation shift and spurious correlation. Retrieval datasets contain Flickr30k~\cite{young-etal-2014-image} and MSCOCO~\cite{chen2015microsoft} which focus on image-text retrieval and WinoGAViL~\cite{bitton2022winogavil} related to commonsense association. 
% Details in Appendix~\ref{sub: eva datasets}.
% \vspace{-10px}
\subsection{Baselines}
We compare against several baselines from \citet{gadre2023datacomp} and \citet{maharana2023d2} in our paper. Here we give a summary for key baselines: (1) \textbf{CLIP score.} We simply select the data with the top CLIP score generated by OpenAI's CLIP ViT-L/14 model, to reduce the size of training pool to 30\% and 45\% for DataComp and 30\% for CC12M. (2) \textbf{Image-based filtering.} we use the method proposed in \citet{gadre2023datacomp} which use external ImageNet-1K as data prior for selecting data. (3) \textbf{$\mathbb{D}^2$ Pruning.}  \citet{maharana2023d2} proposes a method that selects the data by combining the difficulty and diversity by representing the dataset as an undirected graph. They use the CLIP score to initialize their graph. Please refer to Appendix~\ref{sub: baselines} for details of baselines.

% \begin{itemize}[leftmargin=*]
%     \item \textbf{CLIP score} We simple select the data with top CLIP score generated by OpenAI's CLIP ViT-L/14 model, to reduce the size of training pool to 30\% and 45\% for DataComp and 30\% for CC12M.
%     \item \textbf{Image-based filtering} we use the method proposed in \cite{gadre2023datacomp} which first filter the data by language (only Enligsh) and caption length (over two words and 5 characters), and then use external ImageNet-1K as data prior for selecting data. 
%     % \yiping{will determine keeping how much later.}
%     \item \textbf{$\mathbb{D}^2$ Pruning} We use the method proposed in \cite{maharana2023d2} which combine the difficulty and diversity by representing the dataset as an undirected graph. For our experiments, we adhere to the default hyperparameters of $\mathbb{D}^2$ on DataComp as specified in their official codebase. Additionally, we tune the number of nearest neighbors over $k = \{1,5,10,15\}$ on CC12M, following their recommendations in the paper.
% \end{itemize}
Here we reproduce CLIP score filtering and $\mathbb{D}^2$ pruning for DataComp in Tab.~\ref{tab:datacomp} because our reproducing results are different from the results of their original papers. The same reproducing issue has also been observed in \citet{maharana2023d2} and the reason may be that some URLs of data become invalid over time\footnote{
See https://github.com/mlfoundations/datacomp/issues/3
% Our download success rate is around 90\%.
}, and the smaller dataset is more sensitive to this problem.
% \simon{maybe link a git issue here.}


\subsection{Results and Discussions}

\paragraph{Results on DataComp and CC12M.}
We report our results for DataComp and CC12M in Tab.~\ref{tab:datacomp} and Tab.~\ref{tab:cc12m}, respectively. \textit{First}, compared with CLIP score or $\mathbb{D}^2$ pruning, directly applying VAS without using CLIP score performs significantly worse on DataComp but better on CC12M. This matches our expectations since VAS only measures the relevance of the visual information between training data and test prior, and doesn't consider the image-text quality. So using VAS alone should only perform well on high-quality datasets. 
% \yifang{Like I mentioned below, maybe it is better to put the first point in ablation study ?}
\textit{Second}, combining VAS(-D) filter with the CLIP score filter will consistently outperform all the baselines among two datasets except the image-based $\cap$ CLIP score on CC12M. Compared with just utilizing the CLIP score filter, it improves 1.3\% and 2.2\% averagely on 38 evaluation sets for DataComp and CC12M, respectively, demonstrating its capability to select the most informative data and enhance model performance. 
\textit{Third}, note that VAS-D, the heuristic method we proposed without any requirements on the external dataset,
% \yiping{this sentence maybe confusing} \yifang{Maybe just say "the heuristic method we proposed without any requirements on external dataset". No need to describe again since we already describe that in the strategy section. And you can put the detail implementation in appendix. }
achieves similar good results to that with the variance of ImageNet-1k. Actually, in Appendix~\ref{sec: add_vis}, we further show that in many cases, VAS(Traindata) will have similar scores to VAS(ImageNet-1k), which suggests that the variance of the train dataset itself can indicate information about which features are more useful in downstream test distribution.
Besides, VAS-D(Traindata) is better than VAS(Traindata) slightly, which means that the dynamic update process of variance may have the effect of removing the unrelated or noisy features that may exist in the initial variance matrix and thus improve the quality of VAS. Finally, we also compare the time cost of different approaches in Appendix~\ref{sub: time cost}.

% \paragraph{Ablation Study on Image and Text Embeddings}
% In addition to comparing our algorithm with established baselines, we extend our analysis to explore alternative formulations for the test prior variance matrix on DataComp. Specifically, we consider two alternative approaches, including: (1) \textit{variance on test embeddings}, implying that $\text{VAS} = \text{VAS}(l,l)$ as defined in Equation~(\ref{eq:def_VAS}), and we denote it as `text'; and (2) \textit{cross covariance on both image and test embeddings}, means that $\text{VAS} = \text{VAS}(l,v) = \text{VAS}(v,l)$ and denoted as `image $\times$ text'. We mark the original version as `image'. The results are comprehensively presented in Table~\ref{tab:abla}. Our findings reveal that across both VAS and VAS-D methods: (1) employing VAS with the variance derived from `text' significantly underperforms compared to using `image'; (2) while the incorporation of `image $\times$ text' shows a marginal improvement in performance over the sole use of `text', it still falls short compared to using `image' alone. This observation substantiates our assertion in Section~\ref{subsec: main strategy} and theoretical analysis (Theorem~\ref{them: main}), which posits that visual features inherently possess richer and more pertinent information about the latent embeddings of data, and it can be better recovered by the visual encoder of CLIP. Therefore, visual-only variance serves as a better prior for data selection.


\vspace{-0.8em}
\paragraph{Ablation study on image and text embeddings.}
We have already show the effective of choosing image-only embeddings for VAS, here we test on two alternative approaches of choosing VAS, including: (1) text embedding only (denoted as `text'), which is equivalent to $\text{VAS}(l,l)$ as defined in Equation~(\ref{eq:def_VAS}) ; and (2) cross covariance on both image and test embeddings (denoted as `image $\times$ text'), which is equivalent to $\text{VAS}(v,l)$. The results shown in Table~\ref{tab:abla} substantiates our vision-only assertion in Section~\ref{subsec: main strategy} and theoretical analysis (Theorem~\ref{them: main}). Specifically, it shows that (1) using `text' VAS significantly underperforms compared to using `image'; (2) using `image $\times$ text' VAS shows a marginal performance improvement over the sole use of `text', but still falls short compared to using `image' alone.
% \yifang{I rewrite this to be a little more concise, please check}
\vspace{-0.8em}
\paragraph{Relation to optimal experimental design.}
Although our VAS filtering has achieved great results, it seems to have a conflict to the idea of optimal experimental design:
\vspace{-3px}
\begin{align*}
    \text{A-optimality} \quad S&= \arg \min_{|S|=N} \Tr(\Sigma_S^{-1})\\
    \text{V-optimality} \quad S&= \arg\min_{|S|=N} \Tr(\Sigma_{\text{prior}}\Sigma_S^{-1})
\end{align*}
% \vspace{-3px}
\begin{table}[t]
\small
\centering
\vspace{-0.5em}
\caption{Relation to Optimal Experimental Design on CC12M. All experiments firstly filter out 50\% data with the top CLIP score and then use corresponding methods to obtain 2.8M data.}
\vspace{0.5em}
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Filtering Strategy}  & \textbf{ImageNet} & \textbf{VTAB} & \textbf{Retrieval} & \textbf{Avg.}\\ \midrule
CLIP score & 7.8& 18.8& 15.2& 17.3\\
Random Sampling & 8.5& 19.9& \textbf{16.3}& 18.1\\
\textbf{VAS-D} (image) & \textbf{9.9}& \textbf{22.5}& \underline{16.2} & \textbf{19.5}\\
\midrule
A-Optimal (image) & 8.2 & 19.2 & 15.6 &17.5\\ 
V-Optimal (image) & 5.1& 16.8& 14.8&15.7  \\
A-Optimal (text) & \underline{8.5} & \underline{20.7} & 15.8 & \underline{18.4}\\
V-Optimal (text) & 7.8 & 19.9 & 15.7 & 18.0\\
\bottomrule
\end{tabular}
\label{tab:oed}
\vspace{-1em}
\end{table}
Here $\Sigma$ is the variance matrix. We choose embeddings from ImageNet-1k as the test prior and compare the experimental design algorithms with our VAS-D in Tab.~\ref{tab:oed}. We can find that these methods perform badly, and V-optimality (image) even performs much worse than vanilla CLIP score filtering. Interestingly, optimal experiment design with text embeddings performs better than that with image embeddings, although they are still significantly inferior to our methods.




==> icml_content/impact_statement.tex <==
\newpage
\iffalse
\section{Impact statement}
This paper presents work whose goal is to find a better data selection method in curating pretraining data. The methods we designed does not have direct social consequence but it is true that all data selection method may have fairness issues or can be vulnerable to harmful data.
\fi

==> icml_content/introduction.tex <==
\section{Introduction}

Curating web-scale visual-language datasets for pretraining models has become a widely adopted approach to improve visual model performance. Many studies have demonstrated that, despite the use of fixed models and training methods, the final performance of a model is significantly impacted by the choice of data \cite{radford2021learning, schuhmann2022laion, cherti2023reproducible, bai2023qwen}. Consequently, various data selection strategies have been proposed to tackle the challenges posed by large datasets with varied data quality and limited computational resources. These strategies, also known as filtering, subset selection, or pruning in the literature, each focus on slightly different objectives. Some strategies prioritize screening out unhelpful samples to maximize the final model performance without budget constraints, while others aim to maximize performance compared to other randomly sampled subsets within the same budget limit. Practically, these strategies are not mutually exclusive, and in this paper, we will evaluate our proposed strategies in both contexts.
% 
% \yifang{Right now it is a little ambiguous when we say filtering/subset selection. In datacomp, seems our ultimate goal is filtering to achieve better performance than the pool but the method we are using is inspired by subset selection. On the cc12M we are strictly using subset selection setting. I plan to make it clear in the later introduction.}

One line of effective approaches treats each sample independently by assigning a quality score to each individual and only training on the samples that received the highest scores.
For example, the baseline CLIP score filtering method uses a pretrained CLIP model to calculate the cosine similarity score between image and text embeddings, and then discards those pairs that are less aligned. Some follow-up works \cite{nguyen2023improving,mahmoud2023sieve,maini2023t,fang2023data} which propose more advanced image-text alignment scoring methods by using other pretrained classification models or more carefully crafted rule-based approaches. Please refer to related works Sec.~\ref{sec: related work} for a more detailed description.

All those works, however, failed to consider the selection strategy from data distribution perspective. This disadvantage becomes more significant with limited computational resources, as high-quality data are not always the most informative or representative. In some cases, certain feature can be easily learnt under much less samples than other features, so adding more high quality data with such feature can hardly further improve the ultimate model. In other cases, certain features rarely occur in our targeted test distribution, and therefore, adding the corresponding samples will have less effect on test performance. Thus, our work proposes a \textit{data-distribution-aware} strategy that can be combined with existing strategies focused on individual data quality. 

One of the most relevant works to ours is \citet{maharana2023d2}, which also considers the example difficulty and  diversity by using forward and
reverse message passing over a constructed dataset graph.  Their approach, however, is designed for general learning frameworks for both supervised and unsupervised (i.e. contrastive) learning without considering the special impact of data distribution in \textit{multi-modal contrastive learning}. 
% 
Another relevant strategy is using the external image-set as data prior proposed by \citet{gadre2023datacomp}, which clusters the image embedding of the candidate pool and selects the samples whose cluster center is the nearest center for at least one ImageNet-1K training example. But this method also comes from more heuristic inspiration without considering the particular learning method, and is therefore more hyper-parameter sensitive.
% 
In contrast to both approaches, our strategy is inspired by recent theoretical progress in those contrastive representation learning works \cite{nakada2023understanding,ji2023power}. As a results, our work achieves much better average performance over the 38 downstream tasks compared to these two and is almost hyper-parameter-free.

\begin{figure*}[t]
    \centering
    \small
    \includegraphics[width=1.0\textwidth]{fig/vis3.pdf}
    \vspace{-1.2em}
    \caption{Illustration of our VAS on DataComp. $\bar f$ means the embeddings calculated by the pre-trained model, and $\Sigma_{\text{prior}}$ matrix is the test prior co-variance matrix, can be chosen as the co-variance matrix of the image embeddings from ImageNet-1k or DataComp itself. (a) Visualization of data with different Variance Alignment Score (VAS) and CLIP score in DataComp. CLIP score does not efficiently evaluate the informativeness of image-text pairs. Data from OCR tasks or unconventional visual tasks (Type 4) can have high quality but little useful visual information. However, VAS can select the data with more meaningful image features (Type 1 and Type 2).
    (b) Illustration of a rough comparison of sampling data for different filtering methods. Using VAS $\cap$ CLIP score filtering can balance the informativeness and quality and increase the proportion of Type 2 data, which are the most helpful data for training image-text models. Please refer to Appendix.~\ref{sec: add_vis} for more visualization results.}
    % \label{fig:vis}
    \label{fig:vas_cs}
    \vspace{-1.0em}
\end{figure*}


Specifically, we propose \textbf{V}ariance \textbf{A}lignment \textbf{S}core (\textsf{VAS}) which aims to find the most informative subset of the training data whose (cross-)covariance between the image-text pairs most aligns with the (cross-)covariance of a reference distribution.
For example, the reference distribution could be the entirety of the pool from which a subset is being chosen, or some other more task-dependent dataset.  
We also combine VAS with a method based on an individual quality metric as it provides a boost in performance empirically. (Sec.~\ref{sec: main})
To validate the effectiveness of our strategy, we primarily leverage the DataComp benchmark \cite{gadre2023datacomp}. Compared with the existing best strategies, it improves 1.3\% averagely on 38 evaluation sets for DataComp without budget constraints and improves averagely 0.4\% for CC12M with budget constraints (see Sec.~\ref{sec: experiment}).
% \yifang{I originally plan to talk about computational efficiency also but now I find the difference it not that significant? All the base-line method do selection < 1h. So I delete it.}
% \yiping{OK for me}


In addition to empirical results, we provide a theoretical justification for our strategy under a linear model assumption. Firstly, assuming we are given a perfect embedding model and proper data prior, we show that choosing the subset to minimize the multi-modal contrastive loss, including the CLIP loss, can be reduced to the problem of maximizing the total VAS score of the subset. Secondly, we prove a generalization bound when the embedding model and data prior are non-perfect (see Sec.~\ref{sec:theory}).

\iffalse
In addition to proposing this distribution-aware, multi-modal contrastive learning focused data selection strategy, we also gain several insights during the design:
\begin{itemize}[leftmargin=*] 
    \item We observe the widely-used CLIP score filtering does not have a close relation with the data informativeness. Therefore, we should be more careful when interpreting scores generated by some external embedding models.
    \item Our empirical findings confirm the previous result that the image embeddings from Imagnet-1K are effective data prior. Nevertheless, we also find a heuristic subset selection method which only relies on training data itself as detailed in equation~\ref{eq:tr_S}. We believe it worth further investigation in the future.\yiping{should we mention alation study and say image is better prior than text?} \yifang{Maybe.. Simon: do those are necessary ?}
    \item Furthermore, we find our strategy is principally contradict to the classical diversity-forced optimal design approach. In fact, we empirically show that the classical A-optimal and V-optimal approaches fails in CLIP training setting, which can be further investigated.
    % \yiping{Add, please check}
    % \yifang{Talk about how this contradicts the classical G-optimal design ?}
\end{itemize}
\fi

==> icml_content/problem_setup.tex <==
\vspace{-1em}
\section{Problem Setup}

We are given a training dataset $D_\text{train} = \{\vx^{v}, \vx^{l}\}$, where $\vx^{v}, \vx^{l} \in \R^d$ is the image-text (vision-language) training pair. For convenience, we will let subscript $vl$ denote either modal so that, for example, $\vx^{vl} \in \{\vx^{v}, \vx^{l}\}$. We aim to identify a subset $S \subset D_\text{train}$, with or without the subset size constraints, that maximizes zero-shot accuracy on some downstream tasks when $S$ is used to train a CLIP model.

\paragraph{CLIP score and embedding.} Recent efforts, such as LAION \cite{schuhmann2022laion} and DataComp \cite{gadre2023datacomp} used OpenAI’s CLIP ViT-L/14 model \cite{radford2021learning} as a teacher model to obtain quality score. Here we denote this vanilla CLIP model as $\bar{f}_{vl}$.
% 
For any pair $\vx^{vl}$, the model outputs a normalized unit-vector $\bar{f}_{vl}(\vx^{vl})$. 
Let $\bar{s}_{ij} := \langle  \bar{f}_v(\vx_i^v), \bar{f}_l(\vx_j^l) \rangle \in [-1,1]$ denote the pairwise cosine similarity between $i$-th image and $j$-th text. 
In the subsequent sections, we will refer to $\bar{s}_{ii}$ as the “CLIP score” from an existing-pretrained ``vanilla'' model publicly available. 
Intuitively, pairs with higher clip scores are more likely to be effective samples since the image is aligned with the text. However, as we will discuss later, this hypothesis is not always true. 
% \yiping{replace 'high quality' with 'helpful'? I think high CLIP score means high quality is fine, but not means informative}
\vspace{-1em}
\paragraph{Dataset and model.} Here we follow the pipeline of Datacomp \cite{gadre2023datacomp} to standardize the training and evaluation process. This is a testbed for dataset experiments aiming to open-source and further improve the vanilla CLIP model and is widely adopted in previous data selection papers~ \cite{nguyen2023improving,maharana2023d2,maini2023t,fang2023data,mahmoud2023sieve,bai2023qwen}. We will give more details in Sec.~\ref{sec: experiment}.
% \vspace{-1em}

==> icml_content/related_works.tex <==
\vspace{-0.5em}
\section{Related Works}
\label{sec: related work}

\paragraph{Distribution-agnostic filters.} 
Raw data crawled from the internet can be highly noisy -- some samples have text failing to describe their image part, and other samples have misleading elements in their image that we don't want the model to focus on. Many strategies have been proposed to algorithmically detect those corruption.
% 
\citet{nguyen2023improving, mahmoud2023sieve} both leverage a pre-trained visual-language model BLIP to caption the image and then compare their similarity with the original caption to detect the mismatch\footnote{Here \citet{nguyen2023improving} replaces the corrupted text with their newly generated caption instead of pruning the whole sample, but the high-level idea is similar.}. Rather than consider a sample level mapping, \citet{maini2023t} further looks into the detailed elements in the image. Their strategies remove images whose text inside is the only feature correlated with the caption by using off-the-shell OCR models. Notably, despite its effectiveness, it has a much higher computational cost than our strategy due to calling text detection models. Finally, instead of using existing models, \citet{fang2023data} proposes to train a data filtering network directly on existing high-quality data. 
% \vspace{-1.2em}
\paragraph{Distribution-aware data selection.}
% Filters focused on individual data as mentioned above naturally leads to varying dataset size that are hard to control. Therefore, it is worthwhile to consider the training data distribution in order to select out the most representative and informative data.  There exists many classical coreset selection results such as \cite{wei2015submodularity,raskutti2016statistical,coleman2019selection}.
There exists many classical coreset selection which select out the most representative and informative data by taking data distribution into control, including \citet{wei2015submodularity,raskutti2016statistical,coleman2019selection}. All those works, however, make the assumption that we are under a fixed budget and aims to increase the subset performance reach to the pool performance. 
There also exist some recent distribution-aware selection works for CLIP pretraining. \citet{wang2023too} first trained a codebook in replace of existing pretrained models like BLIP. Then they cluster the samples based on their image corresponding codes and selects a representative subset of samples from each cluster. 
Later \citet{maharana2023d2} considers the example difficulty and data diversity by using
forward and reverse message passing over a constructed
dataset graph.
% \vspace{-1.2em}
\paragraph{Dataset as prior.} 
Neither strategy mentioned above considers the distribution shift in test data. Although such downstream task is unknown in advance, it is possible to estimate via some proxy dataset as prior. This was first proposed in \citet{gadre2023datacomp} relying on sampling image text pairs that are semantically similar to diverse and curated datasets like ImageNet~\cite{deng2009imagenet}. Later \citet{xu2023cit} also use ImageNet as prior but measuring the similarity with both text and meta information. Their work focused on curation instead of subset selection but the high level idea is similar. 
% The potential disadvantage is that such subset will be biased towards those proxy dataset related models. Nevertheless, it is effective in practice, which may suggests that ImageNet is still a good proxy for most existing downstream benchmarks. We also use this in our paper and observe the similar phenomonom.


% \paragraph{Theoretical contrastive learning}
% \yifang{Is it necessary} \yiping{add relevant theoretical work for metric learning?}\yiping{Note that there is no concrete theory for CLIP score?}

==> icml_content/strategy_overview.tex <==
\section{Data Filtering Strategy}
\label{sec: main}
Fig.~\ref{fig:vas_cs} gives an overview of our strategy. We give more details below.


\subsection{Variance Alignment Score (VAS)}


Most existing data selection strategies focus on individual sample quality by measuring the similarity between image and text features (e.g., CLIP score). Yet, they fall short in evaluating how each data point contributes to the model's ability to learn meaningful representations in the context of a target distribution and \emph{other} points included in the set. To measure the informativeness of an individual sample for the overall multi-modal contrastive training, we introduce a novel, data-distribution-aware metric named Variance Alignment Score (VAS) defined as
\begin{align}\label{eq:def_VAS}
    & \text{VAS}_i(m_1,m_2) = \bar f_{m_1}(\vx_i^{m_1})^\top \bar{\Sigma}_\text{test} \bar f_{m_2}(\vx_i^{m_2}) \\
    & \text{where }
    \bar{\Sigma}_\text{test} =  \E_{\vx \sim \vD_\text{test\_proxy}} \bar{f}_{m_1}(\vx^{m_1}) \bar{f}_{m_2}(\vx^{m_2})^\top \nonumber
\end{align}
Here $m_1,m_2$ are the modalities we choose and can be visual or language. And $\vD_{\text{test\_proxy}}$ is some proxy test data distribution when the actual downstream tasks are unknown, which is also called ``data prior" in some previous work as we mentioned in Section~\ref{sec: related work}. 
%
The specific choice of $\bar{\Sigma}_{\text{test}}$ and $m_1,m_2$ is crucial and we left details in the next section~\ref{subsec: main strategy}. Here we provide a high level intuition behind VAS.

According to the no-free-lunch theorem, it is impossible to optimize the learning of every feature equally well within a limited budget. In other words, we cannot find a universally optimal strategy for any arbitrary test distribution. Therefore, we tend to select samples that contain effective features in test distributions. Given our focus on this particular multi-modal contrastive learning framework, we leverage insights from previous theoretical generalization bounds as discussed in \citet{ji2023power,nakada2023understanding}. These works suggest that, under a good embedding model $\Bar{f}$, the variance or cross-variance term, denoted as $\frac{1}{N}\sum_i\bar{f}_{m_1}(\vx_i^{m_1}) \bar{f}_{m_2}(\vx_i^{m_2})^\top$, is a suitable criterion for indicating informativeness.
% 
For the rigorous theoretical justification, please refer Lemma~\ref{lem: main} .


\subsection{Main Strategy}
\vspace{-0.5em}
\label{subsec: main strategy}
\begin{algorithm}
\caption{VAS-based strategy}
\label{algo: main}
\begin{algorithmic}[ht]
    \STATE \textbf{Step 1:} \textit{Conservatively} remove low CLIP score samples. (i.e., almost certain low-quality samples)
    \STATE \textbf{Step 2.1:} Choose proper $\vD_{\text{test\_proxy}}$
    \STATE \textbf{Step 2.2:} Select $S = \arg \max_{|S| = N} \sum_{i \in S}\text{VAS}_i(v,v)$
\end{algorithmic}
\end{algorithm}
\vspace{-0.8em}
We then propose a simple two-stage pruning strategy in Algo.\ref{algo: main} that considers both individual quality and overall distribution by combining the CLIP score with VAS. 

In step 1, we first remove those easily distinguishable low-quality samples, such as low-resolution images or mismatched text (Type 1 and Type 3 data in Fig.~\ref{fig:vas_cs}).
% \simon{we can refer to Figure 1 left here.}\yiping{fix} 
However, unlike the native CLIP score filter in \citet{gadre2023datacomp}, which greedy eliminates 70\% of the data in both DataComp and CC12M datasets, we remove much less data (e.g. around half of the data). Note the overall performance is not sensitive to small variation in removal ratio. 
Subsequently, in step 2, we select a data prior, $\vD_{\text{test\_proxy}}$, either by choosing the external ImageNet-1K or heuristically selecting a subset from the training set which only contains high-frequency features (Details in Eqn.~\ref{eq:tr_S} and \ref{eq:tr_S2}). Based on the selected $\vD_{\text{test\_proxy}}$, we compute the vision-only VAS score and select a subset of size $N$ with the highest scores. Detailed discussions and ablation study results are provided to highlight the significance of these three designs.
\vspace{-0.8em}
\paragraph{CLIP score does not indicate informativeness.} While it is intuitive that extremely low CLIP scores suggest low sample quality, the converse that high CLIP scores suggest high sample quality is not necessarily true. 
For example, if an image contains words that also appear in the caption, that may produce a high CLIP score but not necessarily the kind of relationship between image and caption that we hope to learn. 
In Fig.~\ref{fig:vas_cs}, we observe that data with similar CLIP scores can obtain very different VAS. Some high CLIP score samples can have low VAS and these samples are more related to OCR tasks and unconventional visual features which are intuitively non-helpful.
Therefore, we adopt a two-stage approach wherein the first stage we remove samples with very low CLIP scores, and then apply VAS to the remaining data to perform a more fine-grained selection.

\vspace{-0.8em}
\paragraph{Choice of $\bar{\Sigma}_\text{test}$.} Although the resulting model is evaluated over 38 different downstream tasks that are unknown to the learner in advance, we find out that using ImageNet-1k \cite{deng2009imagenet} as the test proxy achieves good performance. Similar effectiveness has also been observed in \citet{gadre2023datacomp, xu2023cit}. We conjecture that this due to the similar variance distribution between ImageNet-1k and other downstream tasks. In other words, despite different tasks, they all share similar effective features. 

% \kevin{This is a mess and I predict reviewers will not like it, but maybe its just me.}\yiping{just rewrite, is it better?}
Besides using the external dataset ImageNet-1k, we also propose a heuristic method called VAS-D (dynamic) which \textit{only} uses the training data itself as prior. We called it ``dynamic'' because in this method we have that $\bar{\Sigma}_\text{test}$ is dynamically updating based on selected $S$ as in Eqn.~\ref{eq:tr_S}. The high-level principle is still similar. For some hyper-parameter $N$, 
\begin{align}\label{eq:tr_S}
    % & S = \arg \max_{|S| = N} \sum_{i \in S}\Tr\left(\bar f_v(\vx_i^v)^\top \bar{\Sigma}_{\text{test}} \bar f_v(\vx_i^v)\right) \\ \label{eq:tr_S}
    % & \bar{\Sigma}_{\text{test}} = \sum_{j \in S}\bar f_v(\vx_j^v)\bar f_v(\vx_j^v)^\top
    & S = \arg \max_{|S| = N} \sum_{i \in S}\bar f_v(\vx_i^v)^\top \bar{\Sigma}_{\text{test}} \bar f_v(\vx_i^v) \\ 
    & \bar{\Sigma}_{\text{test}} = \frac{1}{|S|}\sum_{j \in S}\bar f_v(\vx_j^v)\bar f_v(\vx_j^v)^\top \nonumber
\end{align}
And it is obviously that (\ref{eq:tr_S}) is equivalent to
% \yiping{No $\sum_i$ ?}
% \yiping{If $\bar\Sigma_{\text{test}}^2$ is better?}
\begin{equation}\label{eq:tr_S2}
    S = \arg \max_{|S| = N} 
    % \sum_{i \in S} 
    \Tr\left((\sum_{j \in S}\bar f_v(\vx_j^v)\bar f_v(\vx_j^v)^\top)^2\right)
\end{equation}
Surprisingly, (\ref{eq:tr_S2}) is conflicted with the general principle in target-agnostic optimal experiment design, which emphasizes the diversity of selected data~\cite{pukelsheim2006optimal}. However, in the Experimental parts (Sec.~\ref{sec: experiment}) we will show that in the context of data selection for training CLIP, the idea of optimal experiment design does not work well.
For the theoretical justification on how the choice of $\bar{\Sigma}_\text{test}$ affects the final performance, please refer to Theorem~\ref{them: main}. 

\vspace{-0.8em}
\paragraph{Necessity of using visual-only information.} The $\vx^{vl}$ we observed comes from the high dimensional representation function mapping from low-dimensional latent vectors. The motivation behind using VAS relies on a good embedding model $\bar{f}_{vl}$ that can recover this latent vector. Hence, if there exists some perfect $\bar{f}_{vl}$, then choosing both visual and language information (i.e. $m_1,m_2 = v,l$) leads to best selection. In practice, however, we found out that visual CLIP model yield much better performance, which may suggest the text embedding is less accurate in recovery. Therefore, we choose to use vision-only information. Also, for the rigorous theoretical justification on how the performance of teacher CLIP model affect the final performance, please refer to  Theorem~\ref{them: main} in Section~\ref{sec:theory}.  

\iffalse
\yifang{========Below subject to further modification =============}
Since CLIP score just measures the relevance between image and text embedding, it does not evaluate the information of each data to help the model learn useful representation. We enhance a non-negative quantity named visual \emph{ variance alignment score (VAS)}  defined as:
\begin{equation}
    \text{VAS}(\Sigma, i) = \langle\bar f(\vx_i^v), \Sigma \bar f(\vx_i^v)\rangle
\end{equation}
We denote $\Sigma_{\text{self}}$ and $\Sigma_{\text{img1k}}$ as the variance matrix for image embedding of the training data from the training set itself and external ImageNet-1K datasets, respectively. Thus, VAS measures how well the visual features of the data match the visual distribution of the particular datasets.
And in Fig.~\ref{fig:vas_cs} we visualize the data pairs in the top \yiping{TODO} \% ratio data, and it simply convey two message:
\begin{enumerate}
    \item \emph{Data with similar CLIP scores can obtain very different VAS}. Yhid means that they have different level of useful visual features. For example, the data contain abundant words or unconventional features are always less helpful for training CLIP model.
    \item \emph{DataComp produces similar VAS compared with ImageNet-1k.} Although the data from DataComp may be very different compared with ImageNet-1k, they still have similar variance distribution, which means that they recognize some similar visual features to be the most effective.
\end{enumerate}

In general, we first use the CLIP score filter to filter out some data that has a strong mismatch between image and text, and then select the data with top VAS, i.e.,  curate the subset by 
\begin{equation}\label{eq:obj}
    S_{\text{VAS}} = \arg \max_{|S| = N} \sum_{i \in S}\text{VAS}(\Sigma, i)
\end{equation}
\yiping{Need more illustration, will add soon.}

If we choose $\Sigma = \Sigma_{\text{self}}$, then we can choose a variant of our original object function call as \emph{VAS-D (dynamic)}. To capture the more useful variance direction, we remove the data with low VAS one by one and then change $\Sigma_{\text{self}}$ as the variance matrix of the subset, which means that
\begin{eqnarray}
    S_{\text{VAS-D}} &=& \arg \max_{|S| = N} \sum_{i \in S}\text{VAS}(\Sigma_{S}, i)\\
    &=&\arg \max_{|S| = N}  \sum_{i \in S}\Tr(\Sigma_{S}\cdot \bar f(\vx_i^v) \bar f(\vx_i^v)^\top)\\
    &=& \arg \max_{|S| = N} \Tr(\Sigma_{S}^2) \label{eq:tr_S}
\end{eqnarray}
And we use the greedy remove method to achieve (\ref{eq:tr_S}). Obviously, if we set the greedy step to only one, VAS-D will return to the vanilla VAS method. In the later parts, we will show that this simple algorithm is not only effective but theoretically provable.

\fi

==> icml_content/theory.tex <==

\section{Theoretical Interpretation}\label{sec:theory}
In this section, we give a theoretical justification on the Step 2.1, 2.2 of our proposed strategy under the linear model assumptions when low quality image and mismatched text has already been removed.
\vspace{-0.5em}
\subsection{Theoretical Setup}

\paragraph{Training data.} For any $\vx^{v}, \vx^{l} \in \R^d$ observable image and text training pairs, we define $\vz^{v}, \vz^{l}$ to be the corresponding latent vectors which contain all semantically pertinent information about our tasks of interest. Similar to previous theoretical work \cite{nakada2023understanding},
we assume each i.i.d pair $\vz^{vl}$ follows zero-mean sub-gaussian distribution whose cross-covariance satisfies
\begin{align*}
    & \text{Cov}(\vz^v,\vz^l) 
    % = \E_{\vz^v_i,\vz^l_j \sim \gD_\text{train}} \left[\vz^v (\vz^l)^\top\right]
    = \Sigma_\text{train} = \text{diag}(\sigma_1,\sigma_2, \ldots),
    & \|\vz^{vl}\| = 1
\end{align*}
and each $\vx^{vl}$ is generated based on a linear model such that
\begin{align*}
    \vx^{vl} = G^*_{vl} \vz^{vl} + \vxi^{vl}.
\end{align*}
Here $G^*_{vl} \in O_{d\times r}$ is the othonormal ground truth representation mapping from the latent vector space to the input space, and $\xi^{vl} \sim \mathcal{N}(0, I_d)$ are \textit{i.i.d.} random noise. 

Also we denote the cross covariance of any finite dataset $S'$ (e.g. the given train set $D_\text{train}$) as $\Sigma_{S'}$.

\paragraph{Test data.} For any zero-shot downstream task, we assume it shares almost same data generation process as the training set, except its the cross-covariance $\Sigma_\text{test}$ does not necessarily equal $\Sigma_\text{train}$, which necessitate the choice of $\Bar{\Sigma}_{\text{test\_proxy}}$.


% \paragraph{CLIP embedding model as teacher} Unlike classical data selection problem where we can only observe $x$ (i.e image, text), here we have a teacher model $\bar{G}_{vl}$, whose generated clip embedding can partially recover the ground truth hidden vector $\vz^{vl}$ with error $\epsilon_{vl}$,
% \begin{align*}
%     \E_{\vz^{vl}, \vx^{vl} \sim \gD_\text{train}} \langle \bar{G}_{vl}\vx^{vl}, \vz^{vl} \rangle \geq 1-\epsilon_{vl}
% \end{align*}
% \yifang{TODO: norm matters if choose 1}
% where $\gD_\text{train}$ is the join training distribution as described in the training data generation process. When $\bar{G}_{vl} = \bar{G}_{vl}^*$, the clip embedding is equivalent to hidden vector. 
% \yifang{Expectation is not strong enough.. maybe need to define over any $|S|$ sampling}

\paragraph{CLIP embedding model as teacher.} Under the linear model assumption, we have a teacher model $\bar{f}_{vl} = \bar{G}_{vl}$, whose generated clip embedding can partially recover the ground truth hidden vector $\vz^{vl}$ with error. 

Formally, we say teacher has $\epsilon_{v}^n$ error if for all possible $n$ budget subsets $S \subset D_\text{train}$,
\begin{align*}
    \frac{1}{|S|} \left\| \sum_{\vx^{vl} \in S} \bar{G}_v^\top \vx^v (\vx^v)^\top \Bar{G}_v - \sum_{\vx^{vl} \in S} \vz^v (\vz^v)^\top \right\|_* \leq \epsilon_{v}^n
\end{align*}
where the same notation applies for the language modal. 
By the orthonormal assumption on the ground truth matrix $G_{vl}^*$, we see that $\bar{G}_v^\top$ is aiming to inverting the map.
In addition, we say the teacher has $\epsilon_{v*l}^n$ cross modal error
\begin{align*}
   \frac{1}{|S|}\| \sum_{\vx^{vl} \in S} \bar{G}_v^\top \vx^v (\vx^l)^\top \Bar{G}_l - \sum_{\vx^{vl} \in S} \vz^v (\vz^l)^\top \|_*  \leq \epsilon_{v*l}^n
\end{align*}
When all $\epsilon_v^n, \epsilon_l^n, \epsilon_{v*l}^n \to 0$ as $n \rightarrow \infty$, then we say the teacher is strong for both modalities. But it might also be possible that only one modal, for example, visual is strong. That is $\epsilon_v^n \to 0,  \epsilon_l^n, \epsilon_{v*l}^n \gg \epsilon_v^n$.
% \footnote{It is possible to represent $\epsilon_{v*l}^n$ using $\epsilon_v^n, \epsilon_l^n$. However, our primary objective in this section is to conceptually interpret our empirical results. Therefore, we will maintain this simpler version for ease of understanding.}




\paragraph{Model and training.} 
According to Lemma 4.1 in \citet{nakada2023understanding}, using the CLIP loss to optimize the linear model has approximately the same training dynamics as using the regularized linear loss. Therefore, here we assume that we are learning $G_v, G_l$ by maximizing the clip score gap between the contrastive pairs, plus a regularizer, 
\begin{align*}\label{eq:linearloss}
    \min_{G_v, G_l} \gL_S^\rho (G_v, G_l)
    % & := \min_{G_v, G_l} \frac{\sum_{i \in S} \sum_{j \in S \setminus \{i\}}(s_{ij} - s_{ii})}{n(n-1)} 
    % + R(G_v, G_l) 
    := \min_{G_v, G_l} \frac{\sum_{i \in S} \sum_{j \in S}(s_{ij} - s_{ii})}{|S|(|S|-1)} 
    +  \frac{\rho}{2}\frac{|S|}{|S|-1}\|G_vG_l^\top\|_F^2
\end{align*}
where  $s_{ij} := \langle  G_v^\top \vx^v_i, G_l^\top \vx^l_j \rangle$ and $\rho > 0$ is some regularizer-related \textit{constant}.
Note that this objective maximizes self-similarity and minimizes similarity between disparate pairs. 
Note that this ``loss'' can be negative, avoiding the trivial null solution of all zeros. 
We denote this training process from any given $S$ as $G_{vl} = \gA^\rho(S)$.


\paragraph{Goal and metric.} 
Under the same principle as our training loss function, we measure the performance of any learnt $G_v, G_l$ on some downstream task with distribution $\gD_\text{test}$ as test loss $\gL_{\text{test}} (G_v, G_l):=$
\begin{align*} 
     \E_{\substack{\vx^{vl}\sim \gD_\text{test}\\\vx^{vl}_2 \sim \gD_\text{test}}} (\langle G_v^\top\vx^v, G_l^\top\vx_2^{l}\rangle- \langle G_v^\top\vx^v, G_l^\top\vx^l\rangle) 
\end{align*}
% Here $ \gD_\text{test}^\epsilon$ denotes the discretized $\epsilon$-covering of continuous distribution  $ \gD_\text{test}$. 
% \yifang{TODO: Simon can you check if this notation is right ? or can we just use $\E_{\vx^{vl} \sim \gD_\text{test}} \E_{\vx^{vl}_2 \sim \gD_\text{test}}$}
This is inspired by the following classification accuracy. Assume that the test data including $C$ class, and the class distribution is $\mathcal{C}$. For every class $c$, the training data $\vx = (\vx^v, \vx^l)$ satisfies distribution $\mathcal{P}_c$. We further assume the corresponding classification templates are $\{\vx_c\}_{c=1}^C$. Thus we define classification accuracy as
% \begin{equation*}
%     \text{AC}(G_v, G_l) = \E_{c \sim \mathcal{C}}\left[\E_{\vx_i \sim \mathcal{P}_c}\mathbf{1} [s_{ic} > \max_{c' \neq c }\{s_{ic'}\}]\right]
% \end{equation*}
\begin{equation*}
    \text{AC}(G_v, G_l) = \E_{c,c' \sim \mathcal{C} \times  \mathcal{C}}\left[\E_{\vx_i \sim \mathcal{P}_c} \mathbf{1}[s_{ic} > s_{ic'}]\right]
\end{equation*}
Therefore our goal is to minimize its gap between the best hind-side subset, for any $\rho$, without budget constraints,
\begin{align*}
    \Delta^\rho(S) = \gL_\text{test}(\hat{G}_{vl}) - \min_{S' \in D_\text{train}} \gL_\text{test}(\gA^\rho(S')), \hat{G}_{vl} = \gA^\rho(S)
\end{align*}
\vspace{-1em}
% We will show that it's connected to the classification accuracy. Assume that there are T tasks distribution over $D_\text{task}$,  each task a binary class, and the class distribution is $C_t$. For every class $c \in \{0,1\}$, the training data $\vx = (\vx^v, \vx^l)$ satisfies distribution $\mathcal{P}_c^t$. We further assume the corresponding classification templates are $\mathcal{A}_C :=\{\vx_c\}_{c=1}^C$. And we defined classification accuracy as
% \begin{equation*}
%     \text{AC}(G_v, G_l) = \E_{t \sim D_\text{task}}\E_{c \sim C_t}\left[\E_{\vx_i \sim \mathcal{P}_c^t}\Pr (s_{ic} > \max_{c' \neq c }\{s_{ic'}\})\right]
% \end{equation*}
% Therefore let $\hat{G}_{vl}$ be the learnt representation from our selected subset $S$ and the $G_{vl}^{\text{random}}$ be the one from a random sampled subset under the same budget, our goal is to maximize
% \begin{align*}
%     \Delta(S) = \gL_\text{test}(\hat{G}_{vl}^{\text{random}}) - \gL_\text{test}(\hat{G}_{vl})
% \end{align*}
% \kevin{So we're committing to compariing ourselves to an IID sample versus the ``best'' subset? This leaves us somewhat vulnerable to the criticism that the CLIP screening could perform even better we just don't know} \yifang{Working on it}

% \yifang{I think another way to write this is as follows.}
% {
% \color{olive}

% Instead of define $\Sigma_\text{best}$ as in the current lemma, we define it as
% \begin{align*}
%         & \Sigma_\text{best} = \argmax_{\Sigma} [\Tr \left( \Sigma_{\text{test}}\Sigma \right)
%             - \frac{...}{\sqrt{|S|}}]\\
%         \text{s.t.} \quad 
%         & \Sigma = \frac{1}{|S|}\sum_{\vz^{vl} \in S} \vz^v (\vz^l)^\top,
%           S\subset D_{train}.
% \end{align*}
% here $-\frac{...}{\sqrt{|S|}}$ comes from noisy $\xi$. In this case we are considering all the possible subset without fixing budget. But we can argue that the first term will decrease when the $-\frac{...}{\sqrt{|S|}}$ increase but with decreasing increase rate. So after surpassing certain $|S|$ budget, the first term become dominating and we can regard this as a fixed budget subset selection problem.
% }
\vspace{-1em}
\subsection{Generalization Guarantees}

We now provide theoretical guarantees and postpone our proof into Appendix~\ref{app: proof}.
\textbf{Firstly, we are going to prove the intuition behind VAS score.} 
% by decomposing $\Delta(S)$ into the error from strategy term where VAS comes from and the unavoidable terms from the natural hardness of the problem itself.

\begin{lemma}[Intuition behind VAS]
\label{lem: main}
    With high probability at least $1-\frac{1}{|S|d}$, suppose the  hind-side best subset has at least $\underline{n}$ number of samples, then we have 
    % \begin{align*}
    %     \Delta^\rho(S) 
    %     &= \underbrace{\frac{1}{\rho}\max_{S' \in D_\text{train}} \left( \Tr\left( \Sigma_{\text{test}} (\Sigma_{S'} - \Sigma_{S}) \right) \right)}_\text{VAS related term}\\
    %     & + \quad \underbrace{\gO \left(\sqrt{\frac{d\log(d|S|)}{\underline{n}}} + \sqrt{\frac{d\log(d|S|)}{|S|}}\right)}_\text{noise}
    % \end{align*}
    \begin{align*}
        \Delta^\rho(S) 
        &= \underbrace{\frac{1}{\rho}\max_{S' \in D_\text{train}} \left( \Tr\left( \Sigma_{\text{test}} (\Sigma_{S'} - \Sigma_{S}) \right) \right)}_\text{VAS related term}+ \quad \underbrace{\gO \left(\sqrt{\frac{d\log(d|S|)}{\underline{n}}} + \sqrt{\frac{d\log(d|S|)}{|S|}}\right)}_\text{noise}
    \end{align*}
\end{lemma}

\begin{proof} [Proof sketch]
% (Sketch version)\\
    \ding{182} Under the assumption that both $\vz^{vl}, \xi_{vl}$ is zero-mean, maximizing the clip score gap is equivalent to maximizing the clip score of the same sample. 
    \vspace{-3px}
    \begin{align*}
         \gL_{\text{test}} (\hat{G}_v, \hat{G}_l):= - \E_{\vx^{vl} \sim \vD_\text{test}}\langle \hat{G}_v^\top\vx^v, \hat{G}_l^\top \vx^l \rangle
    \end{align*}
    \ding{183} By minimizing the regularized training loss $\gL_S^\rho (G_v, G_l)$ using Eckart-Young-Mirsky Theorem, we get a closed form solution of $\hat{G}$ as 
    \vspace{-3px}
    \begin{align*}
        \hat G_v \hat G_l^\top \approx \frac{1}{\rho} G_v^* \Sigma_S \cdot (G_l^*)^\top + \text{noise depend on $S$}
    \end{align*}
     \ding{184} Combining the result in \ding{183} and \ding{182}, we have 
     \vspace{-3px}
    \begin{align*}
        & \gL_{\text{test}} (\hat{G}_{vl}) \approx  - \frac{1}{\rho}\Tr\left( \Sigma_{\text{test}}\Sigma_S \right) -\text{noise depend on $S$}
    \end{align*}
    The same analysis can be applied on $\min_{S' \in D_\text{train}} \gL_\text{test}(\gA(S'))$ as well. Rearranging these two equations gives us the final result.
\end{proof}

This lemma shows the the $\Delta(S)$ is depend on the VAS-related term and the noise term which comes from $\xi$. When $\underline{n}$ and $|S|$ is large enough, then the VAS-related term will become dominant. This aligns with our practice experience that the final performance is less sensitive to the small variation in the number of select data as long as that is sufficient.
% 
Moreover, in some special cases where test distribution has identity cross-variance, then sampling by greedily choosing CLIP score might be enough.

\textbf{Now we are ready to give a proof on the choice of $\bar{\Sigma}_{\text{test}}$ and visual-only information.}
Specifically, the strategy error mainly comes from (1). The unknown test distribution shift from training. (2). The unobservable ground truth $\Sigma_S$. To tackle error (1), we assume some prior knowledge on test by using the proxy test variance $\bar{\Sigma}_{\text{test}}$. To tackle the error (2), there are two possible solutions as shown below. Based on the theoretical interpretation, we should choose different strategy based on the property of the teacher embedding model.
\vspace{-5px}
\begin{align*}
    & S_{\text{vision+language}} = \argmax_{S} \Tr\left(\bar{\Sigma}_{\text{test}} (\sum_{\vx^{vl} \in S} \bar{G}_v^\top \vx^v (\vx^l)^\top \Bar{G}_l) \right)  \\
    &  S_{\text{vision only}} = \argmax_{S} \Tr\left(\bar{\Sigma}_{\text{test}} (\sum_{\vx^{vl} \in S} \bar{G}_v^\top \vx^v (\vx^v)^\top \Bar{G}_v) \right)
\end{align*}


\begin{theorem}[Main] 
\label{them: main}
    Under the assumption of Lemma~\ref{lem: main},
    \begin{align*}
       \Delta^\rho(S)
        & \leq \text{noise} +  \frac{1}{\rho}\|\bar{\Sigma}_{\text{test}} - \Sigma_{\text{test}} \| \|\Sigma_S - \Sigma_{\text{best}}\|_* \\
        & + \frac{1}{\rho}
        \begin{cases}
            \epsilon_{v * l}^S  \quad \text{(vision+language)} \\
            \epsilon_v^S +  \sqrt{1 - \frac{1}{|S|}\sum_{i \in [S]} \langle \vz^v,\vz^l \rangle)} \quad \text{(vision only)}
        \end{cases}
    \end{align*}
\end{theorem}

Firstly, it is evident that the greater the difference between $\bar{\Sigma}_{\text{test}}$ and $\Sigma_{\text{test}}$, the less improvement we can expect. Moreover, in scenarios where $\epsilon_l$ is large (indicating lower accuracy in the language part) while $\epsilon_v$ is small (indicating higher accuracy in the vision part), it may be advisable to opt for vision-only embeddings.
% 
However, the learner should also consider the term $\sqrt{1 - \frac{1}{|S|}\sum_{i \in S} \langle \vz^v, \vz^l \rangle}$, which represents the alignment between the ground truth visual and language latent vectors, essentially reflecting the intrinsic quality of the data. If this term is already significant, relying solely on vision information as a proxy for language information could lead to suboptimal results.





\iffalse
Now we are ready to show the main advantage of our strategy compared to the random sampling. We start with the case that teacher model can recover both $\vz^v,\vz^l$ with low error $\epsilon_{vl} \to 0$ in Theorem~\ref{them: main strong teacher}. In this case, we shall use clip embedding form both image and text. Nevertheless, our empirical result \yifang{cite} shows that using clip embedding from both modal performs much worse than using image embedding only. We further interpret this phenomena in Theorem~\ref{them: main weak teacher}.

\begin{theorem}[Results under a strong teacher]
\label{them: main strong teacher}
    Let $\hat{G}_{vl}$ be the learnt representation from our selected subset $S$ and the $G_{vl}^{\text{random}}$ be the one from a random sampled subset under the same budget. We have that, \yifang{with high prob?}
    \begin{align*}
        &\gL(\hat{G}_{vl}^{\text{random}}) - \gL(\hat{G}_{vl}) \\
        &\geq \underbrace{\Tr \left( \Sigma_{\text{test}}(\Sigma_{\text{best}} - \Sigma_{\text{train}}) \right) }_{\text{best possible improvement}}
            + \underbrace{\Tr \left( \Sigma_{\text{test}}(\Sigma_S - \Sigma_{\text{best}}) \right) }_{\text{err from test distribution shits}} \\
        &\quad - \underbrace{\text{\yifang{TODO}}}_{\text{noise error}} 
          - \underbrace{\text{\yifang{TODO}}}_{\text{err from teacher model}}
    \end{align*}
    where $\Sigma_S = \frac{1}{|S|}\sum_{\vz^{vl} \in S} \vz^v (\vz^l)^\top$ is the variance of chosen subset $S$ and $\Sigma_\text{best}$ is the variance best subset we could choose under the same budget. Formally, it is defined as: 
    \begin{align*}
        & \Sigma_\text{best} = \argmax_{\Sigma} \mathrm{tr\left( \Sigma_{\text{test}}\Sigma \right)} \\
        \text{s.t.} \quad 
        & \Sigma = \frac{1}{|S'|}\sum_{\vz^{vl} \in S'} \vz^v (\vz^l)^\top,
          S' \subset D_{train}, |S'| = |S|
    \end{align*}
\end{theorem}

\paragraph{Discussion} 
\yifang{How test distribution affect}

\yifang{How quality $\text{Trace}(\Sigma)$ affect}

\yifang{Budget lower bound}

Above result will become meaningless when $\epsilon_l$ becomes larger. Fortunately, we are able to \textit{largely} reduce the error from teacher model in the sacrifice of a slightly increased error from test distribution shifts.

\begin{theorem}[Results under weak language modal teacher (Main)]
\label{them: main weak teacher}
    
\end{theorem}



\yifang{===== Below TODO ======}

Following \cite{nakada2023understanding, ji2023power}, we choose $R(G_1, G_2) = (\rho/2)\|G_1G_2^\top\|_F^2$ for some $\rho > 0$, which allows us to use Eckart-Young-Mirsky theorem [XXX] (Details in Appendix XXX) directly, and we can obtain the following closed-form solution
\begin{lemma}[Informal]\label{lemma:EYM}
    Let
    \begin{equation}
        \hat G_1, \hat G_2 = \arg \min_{G_1, G_2 \in \R^{d\times r}}\mathcal{L}(G_1,G_2)
    \end{equation}
    Then we have
    \begin{equation}
        \hat G_1 \hat G_2^\top = \frac{n}{\rho(n-1)}G_1^*V \cdot\Sigma\cdot V^\top (G_2^*)^\top + \text{noise}
    \end{equation}
    where
    \begin{equation}
        \Sigma :=\frac{1}{n}\sum_{l=1}^n\vy_i^{(1)}(\vy_{i}^{(2)})^\top
    \end{equation}
\end{lemma}

So the key points for improving the generalization error of $\hat G_1 \hat G_2^\top$ is to obtain benign $\Sigma$. If for any data point, $\vy^{(1)}$ aligns with $\vy^{(2)}$ well, then $\Sigma$ can be well diagonal and the generalization error is low. However, in the large scale training scenario of image-text foundation models, the data are always curated from web and thus low-qualitied, so the unfiltered dataset will result in non-diagonal terms in $\Sigma$ and performs badly. To formalize the context, we define:

\begin{definition}[Excess Risk]
    The excess risk on the test distribution is \yiping{If this definition is fine?}
    \begin{equation*}
        % E(G_1, G_2) = \E_{
        %     (\vx_i^{(1)},\vx_i^{(2)}), (\vx_j^{(1)},\vx_j^{(2)}) \sim \mathcal{P}^{te}_{X^2}
        % }[(s_{ij} - s^*_{ij})^2]
        ER(G_1, G_2) = \frac{1}{2}\E_{
            \vw_i, \vw_j\sim \mathcal{P}^{te}_{X^2}
        }\left[(s_{ij} - s^*_{ij})^2 + (s_{ji} - s^*_{ji})^2\right]
    \end{equation*}
\end{definition}
Then if we choose $\rho = n/(n-1)$, and note that the data generation for the two modality are symmetric, and thus $\Sigma$ is symmetric with high probability, then we can obtain
\begin{equation}\label{eq:ERapprox}
    ER(\hat G_1, \hat G_2) \approx 
    \mathop{\E}_{\vw_i, \vw_j\sim \mathcal{P}^{te}_{X^2}} [(\vy_i^{(1)})^\top (\Sigma - I_r)\vy_j^{(2)}]^2 
\end{equation}
% where $\vy^{(l)}$ is defined in Lemma~\ref{lemma:EYM}. 
Then from (\ref{eq:ERapprox}), we know that minimize the absolute value of the terms in the top left block of matrix $\Sigma - I_r$ will be more important than others because those terms corresponding to more frequently sampled features.

\yiping{TODO: Add another measurement to mimic imagenet classification error. Show that balance class can still be beneficial by maximize the cond}

\yiping{Maybe the results can be generalized to the case where the features of \textbf{downstream tasks} are give?}
\section{}

\fi



\iffalse
Define $\vx, \vy \in \R^d$ be the image and text inputs, and $\hat f, \hat g : \R^d \rightarrow \R^r$ as the image and text encoders, respectively. And we use $\vf_i := \hat{f}(\vx_i)/\|\hat{f}(\vx_i)\|_2$ to denote the normalized embedding for the $i$-th image inputs, and similar notation for $\vg_i$. Further let $\alpha_{ij} = \vf_i^\top \vg_j$ be the pairwise cosine similarity and $\beta_{ij} = \exp(\alpha_{ij}/\tau)$ be its exponentiation of with fixed temperature parameter $\tau$. Then we can then write the CLIP loss as
\begin{equation}\label{eq:CLIPloss}
    \mathcal{L} = -\frac{\tau}{2}\sum_{i=1}^n\left[\log(\frac{\beta_{ii}}{\sum_{j=1}^n\beta_{ij}})+\log(\frac{\beta_{ii}}{\sum_{j=1}^n\beta_{ji}})\right]
\end{equation}
We assume that the multi-modal data is generated by two different linear mapping with the same latent variables $\vz \in \R^r$, i.e.,
\begin{equation}
    \vx = F^* (\vz + \vvxi^{x}), \quad \vy = G^* (\vz + \vvxi^{y})
\end{equation}
where $F^*, G^* \in O_{d\times r}$ has orthonormal columns and $\vvxi^x, \vvxi^y \sim \mathcal{N}(0, \sigma^2 I_r), \sigma \ll 1$ are independent random noise. This assumption is widely used in previous works~\cite{XXX}.
Further, we use linear model  $\hat f(\vx) := \hat F^\top\vx, \hat g(\vy) := \hat G^\top\vy$ where $\hat F, \hat G \in \R^{d\times r}$, to minimize the contrastive loss. We use stochastic gradient descent with all the data in a batch to update the parameters, i.e., 
\begin{equation*}
    \hat F(t+1) = \hat F(t) - \frac{\eta}{n}\sum_{i=1}^n \vx_i(\left.\frac{\partial \mathcal{L}}{\partial \hat f(\vx_i)}\right|_t)^\top
\end{equation*}
\begin{equation*}
    \hat G(t+1) = \hat G(t) - \frac{\eta}{n}\sum_{i=1}^n \vy_i(\left.\frac{\partial \mathcal{L}}{\partial \hat g(\vy_i)}\right|_t)^\top
\end{equation*}

\section{Main Motivation}
We must mention that \emph{minimizing (\ref{eq:CLIPloss}) doesn't mean learning the ground truth head $F^*, G^*$}.
A simple example is  considering the case with $n=r$ samples for training, where $\vz_i = \ve_i, i \in [r-1]$ and $\vz_r = (1-\varepsilon)\ve_{r-1} + \varepsilon\ve_r$, $\varepsilon \ll 1$. It's clear that if $\hat F = F^*, \hat G = G^*$, we will have $\beta_{r-1,r}, \beta_{r,r-1}\approx \beta_{r-1,r-1}$, which means that $r-1$-th and $r$-th samples are confusing to the model. However, we can always find some rank-$r$ linear matrix $(\hat F)^\top F^*, (\hat G)^\top G^*$ to map any $r$ vectors onto $r$ orthogonal vectors, which means the learner $\hat F, \hat G$ can separate all the samples well and further minimize the CLIP loss. \yifang{I think it would be better to clearly define what is a good representation ? For example, previous work define a bad representation by saying under all possible linear classifier (the linear head), it is impossible to get good acc.}
\yiping{Yes, intuitionally the repr function that maps the input from different classes into a more separate space will have better downstream performance. I will add it soon. }

Following this observation, our motivation is that not all the classes are evenly distributed in the embedding space generated by the OpenAI CLIP model.\yiping{Need visualization}. Classes with many similar features are always generated by close latent variables, which will result in similar embeddings and take a much longer time for the learners to separate each other. This can happen even when the image and text encoders are perfectly aligned.

\begin{assumption}[Data Classes]\label{ass:classes}
Assume we have $r$ different classes and the sample number in the $i$-th class is $n_i$, so $n = \sum_i^r n_i$. The classes are determined by $r$ different latent variables $\{\bar\vz_{i}\}_1^{r}$ satisfies:  $\bar\vz_r := (1-\varepsilon)\bar\vz_{r-1} + \varepsilon\bar\vz'$, $\{\bar\vz_1, \ldots, \bar\vz_{r-1}, \bar\vz'\}$ are orthonormal vectors.
\end{assumption}
\begin{theorem}
    \yiping{Need further calculation}(Informal) Assume Assumption~\ref{ass:classes} holds with parameters $\{n_i\}_1^r, \varepsilon$. Then if $\hat F(0)^\top F^* \approx \hat G(0)^\top G^*$\yiping{This assumption should not be necessary}, we claim that $\hat F(t)^\top F^*\approx \hat G(t)^\top G^*$, $\alpha_{r,r-1}, \alpha_{r-1,r}$ decreasing in the rate of $O(\varepsilon\cdot(n_{r-1}+n_{r})/{n})$, while for all other $\alpha_{i,j}, i\neq j$, their decreasing rate is $O((n_{i}+n_{j})/{n})$
\end{theorem}

\yiping{Add class definition. $n_i$ is the number of samples for class $i$.}
\fi



% Acknowledgements should only appear in the accepted version.
% \section*{Acknowledgements}

% \textbf{Do not} include acknowledgements in the initial version of
% the paper submitted for blind review.

% If a paper is accepted, the final camera-ready version can (and
% probably should) include acknowledgements. In this case, please
% place such acknowledgements in an unnumbered section at the
% end of the paper. Typically, this will include thanks to reviewers
% who gave useful comments, to colleagues who contributed to the ideas,
% and to funding agencies and corporate sponsors that provided financial
% support.


% In the unusual situation where you want a paper to appear in the
% references without citing it in the main text, use \nocite

% \nocite{langley00}


==> icml_content/theory_archive.tex <==
\section{Theoretical interpretation}\label{sec:theory}
In this section, we give a theoretical justification on the second phase \yifang{right word ?} of our proposed strategy under the linear model assumptions when their is no corrupted or contaminated samples (e.g. low quality image, mismatched text) 

\subsection{Theoretical setup}
We give a rigorous theoretical interpretation on our learning problem as follows.

\paragraph{Training data generation}
For any $\vx^{v}, \vx^{l} \in \R^d$ observable image and text training pairs, we define $\vz^{v}, \vz^{l}$ to be the corresponding latent vectors which contains all the information we cared about. Similar to previous theoretical work \yifang{cite},
each pair of $(\vz_v,\vz_l)$ is an independent zero-mean sub-gaussian vector satisfies
\begin{align*}
    & \text{Cov}(\vz_v,\vz_l) 
    = \E_{\vz_v,\vz_l \sim \gD_\text{train}} \left[\vz_v \vz_l^\top\right]
    = \Gamma_\text{train},
    & \|\vz_{vl}\| = 1
\end{align*}
and $\vx^{vl}$ is generated based on a linear model that
\begin{align*}
    \vx^{vl} = G^*_{vl} \vz^{vl} + \vxi^{vl}.
\end{align*}
Here $G^*_l \in O_{d\times r}$ is the ground truth representation that maps from the latent vector space to the signal part of the input space, and $\xi^{vl} \sim \mathcal{N}(0, \sigma_{\xi}^2I_d)$ are \textit{i.i.d.} random noise, with $\sigma_{\xi} \ll 1$. 
For $n$ \textit{i.i.d.} samples, we denote $X^{vl} = (\vx^{vl}_1,\ldots, \vx^{vl}_n)^\top \in \R^{n \times d}$, $Z^{vl} := (\vz_1^{vl}, \ldots, \vz_n^{vl})^\top \in \R^{n \times r}$ 
and $\Xi^{vl} := (\vxi^{vl}_1,\ldots,\vxi^{vl}_n)^\top \in \R^{n \times d}$ to be the stacked matrix of inputs, embeddings and noise. 


\paragraph{Test data generation}
For any zero-shot downstream task, we assume it share the same linear representation and noise as train set. But the distribution of zero-mean normalized subgaussian latent vectors $\vz^{vl}$ might be different. That is, the cross-covariance $\Gamma_\text{test}$ does not necessary equal to $\Gamma_\text{train}$. We will discuss the impact of different distribution in the theorem section. 


% \paragraph{CLIP embedding model as teacher} Unlike classical data selection problem where we can only observe $x$ (i.e image, text), here we have a teacher model $\bar{G}_{vl}$, whose generated clip embedding can partially recover the ground truth hidden vector $\vz^{vl}$ with error $\epsilon_{vl}$,
% \begin{align*}
%     \E_{\vz^{vl}, \vx^{vl} \sim \gD_\text{train}} \langle \bar{G}_{vl}\vx^{vl}, \vz^{vl} \rangle \geq 1-\epsilon_{vl}
% \end{align*}
% \yifang{TODO: norm matters if choose 1}
% where $\gD_\text{train}$ is the join training distribution as described in the training data generation process. When $\bar{G}_{vl} = \bar{G}_{vl}^*$, the clip embedding is equivalent to hidden vector. 
% \yifang{Expectation is not strong enough.. maybe need to define over any $|S|$ sampling}

\paragraph{CLIP embedding model as teacher} Unlike classical data selection problem where we can only observe $x$ (i.e image, text), here we have a teacher model $\bar{G}_{vl}$, whose generated clip embedding can partially recover the ground truth hidden vector $\vz^{vl}$ with error. 

Formally, we say teacher has $\epsilon_{v}^n$ error if for all possible $n$ budget subet $S \subset D_\text{train}$,
\begin{align*}
    \frac{1}{|S|} \left\| \sum_{\vx_{vl} \in S} \bar{G}_v^\top \vx_v \vx_v^\top \Bar{G}_v - \sum_{\vx_{vl} \in S} \vz_v \vz_v^\top \right\|_* \leq \epsilon_{v}^n
\end{align*}
the same notation applies for language modal. In addition, we say teacher has $\epsilon_{v*l}^n$ cross modal error
\begin{align*}
   \frac{1}{n}\| \sum_{\vx_{vl} \in S} \bar{G}_v^\top \vx_v \vx_l^\top \Bar{G}_l - \sum_{\vx_{vl} \in S} \vz_v \vz_l^\top \|_*  \leq \epsilon_{v*l}^n
\end{align*}
When all $\epsilon_v^n, \epsilon_l^n, \epsilon_{v*l}^n \to 0$ , then the teacher is strong for both modal. But it might also be possible that only one modal, for example, visual is strong. That is $\epsilon_v^n \to 0,  \epsilon_l^n, \epsilon_{v*l}^n \gg \epsilon_v^n$.
\footnote{It is possible to represent $\epsilon_{v*l}^n$ using $\epsilon_v^n, \epsilon_l^n$. However, our primary objective in this section is to conceptually interpret our empirical results. Therefore, we will maintain this simpler version for ease of understanding.}




\paragraph{Model and training}
According to Lemma 4.1 in \cite{nakada2023understanding}, using the CLIP loss to optimize the linear model has approximately the same training dynamics as using the regularized linear loss. Therefore, here we assume that we are learning $G_v, G_l$ by maximizing the clip score gap between same-sample pairs and the contrastive pairs, plus the some regularization, 
\begin{align*}\label{eq:linearloss}
    & \min_{G_v, G_l} \gL_S (G_v, G_l) \\
    & := \min_{G_v, G_l} \frac{\sum_{i \in S} \sum_{j \in S \setminus \{i\}}(s_{ij} - s_{ii})}{n(n-1)} 
    + R(G_v, G_l) \\
    & = \min_{G_v, G_l} \frac{\sum_{i \in S} \sum_{j \in S}(s_{ij} - s_{ii})}{n(n-1)} 
    + R(G_v, G_l)
\end{align*}
where  $s_{ij} := \langle  G_v^\top \vx^v_i, G_l^\top \vx^l_j \rangle$ and $\gS$ is the $n$ size dataset after filtering. Notice here we abuse notation a little bit between indices $i,j$ and the actual sample $\vx^{vl}_i$. This format was also used in \yifang{cite}.

\paragraph{Goal and metric}
Under the same principle as our training loss function, we measure the performance of any learnt $G_v, G_l$ on some downstream task with distribution $\gD_\text{test}$ as test loss $\gL_{\text{test}} (G_v, G_l):=$
\begin{align*}
     \E_{\substack{\vx_{vl}\sim \gD_\text{test}\\\vx_{vl}' \sim \gD_\text{test}}} (\langle G_v^\top\vx_v, G_l^\top\vx_l'\rangle- \langle G_v^\top\vx_v, G_l^\top\vx_l\rangle) 
\end{align*}
% Here $ \gD_\text{test}^\epsilon$ denotes the discretized $\epsilon$-covering of continuous distribution  $ \gD_\text{test}$. 
% \yifang{TODO: Simon can you check if this notation is right ? or can we just use $\E_{\vx_{vl} \sim \gD_\text{test}} \E_{\vx_{vl}' \sim \gD_\text{test}}$}
\yifang{Double check if this is true}
Therefore let $\hat{G}_{vl}$ be the learnt representation from our selected subset $S$ and the $G_{vl}^{\text{random}}$ be the one from a random sampled subset under the same budget, our goal is to maximize
\begin{align*}
    \Delta(S) = \gL_\text{test}(\hat{G}_{vl}^{\text{random}}) - \gL_\text{test}(\hat{G}_{vl})
\end{align*}



\subsection{Generalization guarantees}
\yifang{Rewriting the whole structure....}



Based on the previous setting, we provide a theoretical guarantees in this section and discuss their connection to the actual algorithm we implemented in \yifang{cite}. We postpone our proof into Appendix~\ref{app: proof}.

Here we decompose the results into three items. The best possible improvement term stands for the for the optimal subset selection if we know the test distribution $\Gamma_{\text{test}}$ in advance, and the error from noise terms stands for the estimation error under any fixed budget $|S|$. Both of term characterize the natural hardness of the problem that it inevitable. 

\begin{theorem}[A simplified version of test loss]
\label{them: simplified test loss}
    Under the assumption that both $\vz_{vl}, \xi_{vl}$ is zero-mean, maximizing the clip score gap is equivalent to maximize the clip score of the same sample. 
     \begin{align*}
         \gL_{\text{test}} (G_v, G_l):= - \E_{\vx_{vl} \sim \gD_\text{test}}\langle G_v^\top\vx_v, G_l^\top \vx_l \rangle
     \end{align*}
\end{theorem}
\yifang{Maybe add some discussion say if the test data are high quality, then $\hat{G} = G^*$ is the best thing we could get. Otherwise, recovering $G^*$ might not be the best option. So we should use contrastive learning instead of directly do supervised learning on the teacher clip model.}

The improvement $\Delta(S) > 0$ is not always possible. We first characterize the hardness of the problem by decomposing $\Delta(S)$ into different sources.
\begin{lemma}[Hardness of the problem]
\label{lem: hardness}
    \yifang{With high prob?}, the improvement of our strategy compared to randomness sampling as 
    \begin{align*}
        &\Delta(S) 
        \geq \underbrace{\Tr \left( \Gamma_{\text{test}}(\Gamma_S - \Gamma_{\text{best}}) \right) }_{\text{err from our strategy} < 0} 
         + \text{hardness} \\
        & \text{hardness}:= \underbrace{\Tr \left( \Gamma_{\text{test}}(\Gamma_{\text{best}} - \Gamma_{\text{train}}) \right) }_{\text{best possible improvement}}
            - \underbrace{\text{\yifang{TODO}}}_{\text{err from noise}}
    \end{align*}
    where $\Gamma_S = \frac{1}{|S|}\sum_{\vz_{vl} \in S} \vz_v \vz_l^\top$ is the variance of chosen subset $S$ and $\Gamma_\text{best}$ is the variance best subset we could choose under the same budget. Formally, it is defined as: 
    \begin{align*}
        & \Gamma_\text{best} = \argmax_{\Gamma} \mathrm{tr\left( \Gamma_{\text{test}}\Gamma \right)} \\
        \text{s.t.} \quad 
        & \Gamma = \frac{1}{|S'|}\sum_{\vz_{vl} \in S'} \vz_v \vz_l^\top,
          S' \subset D_{train}, |S'| = |S|
    \end{align*}
The random sampling is unbeatable when 
$\text{hardness}< 0$
\end{lemma}

\begin{proof} 
(Sketch version)\\
\textbf{Step 1: Simplified the loss} 

    
\end{proof}
Here we decompose the results into three items. The best possible improvement term stands for the for the optimal subset selection if we know the test distribution $\Gamma_{\text{test}}$ in advance, and the error from noise terms stands for the estimation error under any fixed budget $|S|$. Both of term characterize the natural hardness of the problem that it inevitable. 



\begin{figure*}[ht]
\vskip 0.2in
\begin{center}
\begin{subfigure}
	\centering
\includegraphics[width=\columnwidth]{fig/vas_cs_f0.451.png}
\end{subfigure}
\begin{subfigure}
	\centering
\includegraphics[width=\columnwidth]{fig/vas_cs_f0.451_text.png}
\end{subfigure}
% \vskip -0.2in
% \centerline{\includegraphics[width=\columnwidth]{Figures/heatmap_L1toL2_final_20.0.pdf}}
\caption{Image features are more concentrated than text features.\yiping{Should I add this kind of pic here? Just draft now.}} \yifang{What conclusion do you want to show ?}
\label{fig:img_txt}
\end{center}
\vskip -0.2in
\end{figure*}


Therefore, we should focus on the term `` error from our strategy". Such error mainly comes from (1) The unknown test distribution shift from training. (2) The unobservable ground truth $\Gamma_S$ as shown below. To tackle error (1), we assume some prior knowledge on test by using the proxy test variance $\bar{\Gamma}_{\text{test}}$. \yifang{TODO: say more} To tackle the error (2), we propose two solutions with theoretical interpretation as below. Based on the theoretical interpretation, we should choose different strategy based on the property of clip score.
\begin{align*}
    & S_{\text{Option 1}} = \argmax_{S} \Tr\left(\bar{\Gamma}_{\text{test}} (\sum_{\vx_{vl} \in S} \bar{G}_v^\top \vx_v \vx_l^\top \Bar{G}_l) \right)  \\
    &  S_{\text{Option 2}} = \argmax_{S} \Tr\left(\bar{\Gamma}_{\text{test}} (\sum_{\vx_{vl} \in S} \bar{G}_v^\top \vx_v \vx_v^\top \Bar{G}_v) \right)
\end{align*}


\begin{theorem}[Main]
\label{them: main}
    \begin{align*}
       \Delta(S)
        & \geq \text{hardness} -  \|\bar{\Gamma}_{\text{test}} - \Gamma_{\text{test}} \| \|\Gamma_S - \Gamma_{\text{best}}\| \\
        & \quad - 
        \begin{cases}
            \epsilon_{v * l}^S  \quad \text{(Option 1)} \\
            \epsilon_v^S +  \frac{1}{|S|}\| \sum_{\vx_{vl} \in S} \vz_v \vz_v^\top -  \Gamma_S\|_* \quad \text{(Option 2)}
        \end{cases}
    \end{align*}
\end{theorem}



\yifang{TODO: add discussion of $\bar{\Gamma}_{\text{test}}$}
It is easy to see that, when $\epsilon_l$ is large \yifang{More specific ?}, as shown in \yifang{Empirical evidence}, using image focused filtering is a better.





\iffalse
Now we are ready to show the main advantage of our strategy compared to the random sampling. We start with the case that teacher model can recover both $\vz_v,\vz_l$ with low error $\epsilon_{vl} \to 0$ in Theorem~\ref{them: main strong teacher}. In this case, we shall use clip embedding form both image and text. Nevertheless, our empirical result \yifang{cite} shows that using clip embedding from both modal performs much worse than using image embedding only. We further interpret this phenomena in Theorem~\ref{them: main weak teacher}.

\begin{theorem}[Results under a strong teacher]
\label{them: main strong teacher}
    Let $\hat{G}_{vl}$ be the learnt representation from our selected subset $S$ and the $G_{vl}^{\text{random}}$ be the one from a random sampled subset under the same budget. We have that, \yifang{with high prob?}
    \begin{align*}
        &\gL(\hat{G}_{vl}^{\text{random}}) - \gL(\hat{G}_{vl}) \\
        &\geq \underbrace{\Tr \left( \Gamma_{\text{test}}(\Gamma_{\text{best}} - \Gamma_{\text{train}}) \right) }_{\text{best possible improvement}}
            + \underbrace{\Tr \left( \Gamma_{\text{test}}(\Gamma_S - \Gamma_{\text{best}}) \right) }_{\text{err from test distribution shits}} \\
        &\quad - \underbrace{\text{\yifang{TODO}}}_{\text{err from noise}} 
          - \underbrace{\text{\yifang{TODO}}}_{\text{err from teacher model}}
    \end{align*}
    where $\Gamma_S = \frac{1}{|S|}\sum_{\vz_{vl} \in S} \vz_v \vz_l^\top$ is the variance of chosen subset $S$ and $\Gamma_\text{best}$ is the variance best subset we could choose under the same budget. Formally, it is defined as: 
    \begin{align*}
        & \Gamma_\text{best} = \argmax_{\Gamma} \mathrm{tr\left( \Gamma_{\text{test}}\Gamma \right)} \\
        \text{s.t.} \quad 
        & \Gamma = \frac{1}{|S'|}\sum_{\vz_{vl} \in S'} \vz_v \vz_l^\top,
          S' \subset D_{train}, |S'| = |S|
    \end{align*}
\end{theorem}

\paragraph{Discussion} 
\yifang{How test distribution affect}

\yifang{How quality $\text{Trace}(\Gamma)$ affect}

\yifang{Budget lower bound}

Above result will become meaningless when $\epsilon_l$ becomes larger. Fortunately, we are able to \textit{largely} reduce the error from teacher model in the sacrifice of a slightly increased error from test distribution shifts.

\begin{theorem}[Results under weak language modal teacher (Main)]
\label{them: main weak teacher}
    
\end{theorem}



\yifang{===== Below TODO ======}

Following \cite{nakada2023understanding, ji2023power}, we choose $R(G_1, G_2) = (\rho/2)\|G_1G_2^\top\|_F^2$ for some $\rho > 0$, which allows us to use Eckart-Young-Mirsky theorem [XXX] (Details in Appendix XXX) directly, and we can obtain the following closed-form solution
\begin{lemma}[Informal]\label{lemma:EYM}
    Let
    \begin{equation}
        \hat G_1, \hat G_2 = \arg \min_{G_1, G_2 \in \R^{d\times r}}\mathcal{L}(G_1,G_2)
    \end{equation}
    Then we have
    \begin{equation}
        \hat G_1 \hat G_2^\top = \frac{n}{\rho(n-1)}G_1^*V \cdot\Gamma\cdot V^\top (G_2^*)^\top + \text{noise}
    \end{equation}
    where
    \begin{equation}
        \Gamma :=\frac{1}{n}\sum_{l=1}^n\vy_i^{(1)}(\vy_{i}^{(2)})^\top
    \end{equation}
\end{lemma}

So the key points for improving the generalization error of $\hat G_1 \hat G_2^\top$ is to obtain benign $\Gamma$. If for any data point, $\vy^{(1)}$ aligns with $\vy^{(2)}$ well, then $\Gamma$ can be well diagonal and the generalization error is low. However, in the large scale training scenario of image-text foundation models, the data are always curated from web and thus low-qualitied, so the unfiltered dataset will result in non-diagonal terms in $\Gamma$ and performs badly. To formalize the context, we define:

\begin{definition}[Excess Risk]
    The excess risk on the test distribution is \yiping{If this definition is fine?}
    \begin{equation*}
        % E(G_1, G_2) = \E_{
        %     (\vx_i^{(1)},\vx_i^{(2)}), (\vx_j^{(1)},\vx_j^{(2)}) \sim \mathcal{P}^{te}_{X^2}
        % }[(s_{ij} - s^*_{ij})^2]
        ER(G_1, G_2) = \frac{1}{2}\E_{
            \vw_i, \vw_j\sim \mathcal{P}^{te}_{X^2}
        }\left[(s_{ij} - s^*_{ij})^2 + (s_{ji} - s^*_{ji})^2\right]
    \end{equation*}
\end{definition}
Then if we choose $\rho = n/(n-1)$, and note that the data generation for the two modality are symmetric, and thus $\Gamma$ is symmetric with high probability, then we can obtain
\begin{equation}\label{eq:ERapprox}
    ER(\hat G_1, \hat G_2) \approx 
    \mathop{\E}_{\vw_i, \vw_j\sim \mathcal{P}^{te}_{X^2}} [(\vy_i^{(1)})^\top (\Gamma - I_r)\vy_j^{(2)}]^2 
\end{equation}
% where $\vy^{(l)}$ is defined in Lemma~\ref{lemma:EYM}. 
Then from (\ref{eq:ERapprox}), we know that minimize the absolute value of the terms in the top left block of matrix $\Gamma - I_r$ will be more important than others because those terms corresponding to more frequently sampled features.

\yiping{TODO: Add another measurement to mimic imagenet classification error. Show that balance class can still be beneficial by maximize the cond}

\yiping{Maybe the results can be generalized to the case where the features of \textbf{downstream tasks} are give?}
\section{}

\fi



\iffalse
Define $\vx, \vy \in \R^d$ be the image and text inputs, and $\hat f, \hat g : \R^d \rightarrow \R^r$ as the image and text encoders, respectively. And we use $\vf_i := \hat{f}(\vx_i)/\|\hat{f}(\vx_i)\|_2$ to denote the normalized embedding for the $i$-th image inputs, and similar notation for $\vg_i$. Further let $\alpha_{ij} = \vf_i^\top \vg_j$ be the pairwise cosine similarity and $\beta_{ij} = \exp(\alpha_{ij}/\tau)$ be its exponentiation of with fixed temperature parameter $\tau$. Then we can then write the CLIP loss as
\begin{equation}\label{eq:CLIPloss}
    \mathcal{L} = -\frac{\tau}{2}\sum_{i=1}^n\left[\log(\frac{\beta_{ii}}{\sum_{j=1}^n\beta_{ij}})+\log(\frac{\beta_{ii}}{\sum_{j=1}^n\beta_{ji}})\right]
\end{equation}
We assume that the multi-modal data is generated by two different linear mapping with the same latent variables $\vz \in \R^r$, i.e.,
\begin{equation}
    \vx = F^* (\vz + \vvxi^{x}), \quad \vy = G^* (\vz + \vvxi^{y})
\end{equation}
where $F^*, G^* \in O_{d\times r}$ has orthonormal columns and $\vvxi^x, \vvxi^y \sim \mathcal{N}(0, \sigma^2 I_r), \sigma \ll 1$ are independent random noise. This assumption is widely used in previous works~\cite{XXX}.
Further, we use linear model  $\hat f(\vx) := \hat F^\top\vx, \hat g(\vy) := \hat G^\top\vy$ where $\hat F, \hat G \in \R^{d\times r}$, to minimize the contrastive loss. We use stochastic gradient descent with all the data in a batch to update the parameters, i.e., 
\begin{equation*}
    \hat F(t+1) = \hat F(t) - \frac{\eta}{n}\sum_{i=1}^n \vx_i(\left.\frac{\partial \mathcal{L}}{\partial \hat f(\vx_i)}\right|_t)^\top
\end{equation*}
\begin{equation*}
    \hat G(t+1) = \hat G(t) - \frac{\eta}{n}\sum_{i=1}^n \vy_i(\left.\frac{\partial \mathcal{L}}{\partial \hat g(\vy_i)}\right|_t)^\top
\end{equation*}

\section{Main Motivation}
We must mention that \emph{minimizing (\ref{eq:CLIPloss}) doesn't mean learning the ground truth head $F^*, G^*$}.
A simple example is  considering the case with $n=r$ samples for training, where $\vz_i = \ve_i, i \in [r-1]$ and $\vz_r = (1-\varepsilon)\ve_{r-1} + \varepsilon\ve_r$, $\varepsilon \ll 1$. It's clear that if $\hat F = F^*, \hat G = G^*$, we will have $\beta_{r-1,r}, \beta_{r,r-1}\approx \beta_{r-1,r-1}$, which means that $r-1$-th and $r$-th samples are confusing to the model. However, we can always find some rank-$r$ linear matrix $(\hat F)^\top F^*, (\hat G)^\top G^*$ to map any $r$ vectors onto $r$ orthogonal vectors, which means the learner $\hat F, \hat G$ can separate all the samples well and further minimize the CLIP loss. \yifang{I think it would be better to clearly define what is a good representation ? For example, previous work define a bad representation by saying under all possible linear classifier (the linear head), it is impossible to get good acc.}
\yiping{Yes, intuitionally the repr function that maps the input from different classes into a more separate space will have better downstream performance. I will add it soon. }

Following this observation, our motivation is that not all the classes are evenly distributed in the embedding space generated by the OpenAI CLIP model.\yiping{Need visualization}. Classes with many similar features are always generated by close latent variables, which will result in similar embeddings and take a much longer time for the learners to separate each other. This can happen even when the image and text encoders are perfectly aligned.

\begin{assumption}[Data Classes]\label{ass:classes}
Assume we have $r$ different classes and the sample number in the $i$-th class is $n_i$, so $n = \sum_i^r n_i$. The classes are determined by $r$ different latent variables $\{\bar\vz_{i}\}_1^{r}$ satisfies:  $\bar\vz_r := (1-\varepsilon)\bar\vz_{r-1} + \varepsilon\bar\vz'$, $\{\bar\vz_1, \ldots, \bar\vz_{r-1}, \bar\vz'\}$ are orthonormal vectors.
\end{assumption}
\begin{theorem}
    \yiping{Need further calculation}(Informal) Assume Assumption~\ref{ass:classes} holds with parameters $\{n_i\}_1^r, \varepsilon$. Then if $\hat F(0)^\top F^* \approx \hat G(0)^\top G^*$\yiping{This assumption should not be necessary}, we claim that $\hat F(t)^\top F^*\approx \hat G(t)^\top G^*$, $\alpha_{r,r-1}, \alpha_{r-1,r}$ decreasing in the rate of $O(\varepsilon\cdot(n_{r-1}+n_{r})/{n})$, while for all other $\alpha_{i,j}, i\neq j$, their decreasing rate is $O((n_{i}+n_{j})/{n})$
\end{theorem}

\yiping{Add class definition. $n_i$ is the number of samples for class $i$.}
\fi



% Acknowledgements should only appear in the accepted version.
% \section*{Acknowledgements}

% \textbf{Do not} include acknowledgements in the initial version of
% the paper submitted for blind review.

% If a paper is accepted, the final camera-ready version can (and
% probably should) include acknowledgements. In this case, please
% place such acknowledgements in an unnumbered section at the
% end of the paper. Typically, this will include thanks to reviewers
% who gave useful comments, to colleagues who contributed to the ideas,
% and to funding agencies and corporate sponsors that provided financial
% support.


% In the unusual situation where you want a paper to appear in the
% references without citing it in the main text, use \nocite

% \nocite{langley00}


==> nips_content/related_works.tex <==
\vspace{-0.5em}
\section{Related Works}
\label{sec: related work}

\paragraph{Methods exclusively rely on training dataset and OAI CLIP model}
Traditional methods solely relied on the training data and the OAI CLIP model which used to extract embedding from it. The most basic methods is using CLIPScore, which measures the similarity between the text and image embedding of the same sample and filter out low-matched samples as we already described in the introduction. Recently, \citet{maharana2023d2} considers the example difficulty and data diversity by using forward and reverse message passing over a constructed dataset graph, which is not only for data filtering, but can also used in fixed budget coreset selections. In addition, there exists many classical coreset selection which select out the most representative and informative data, including \citet{wei2015submodularity,raskutti2016statistical,coleman2019selection}, but none of those methods achieve a good performance under this DataComp (i.e. data filtering for pretraining CLIP model) setting.

\paragraph{Methods using prior knowledge of downstream tasks}
Many works proposed target-aware methods when the prior of downstream tasks are available.

\paragraph{Methods requires external model or datasets}
Recent leading works leverages the external high quality data or external models to further leverage the performance.

\iffalse

\paragraph{Distribution-agnostic filters.} 
Raw data crawled from the internet can be highly noisy -- some samples have text failing to describe their image part, and other samples have misleading elements in their image that we don't want the model to focus on. Many strategies have been proposed to algorithmically detect those corruption.
% 
\citet{nguyen2023improving, mahmoud2023sieve} both leverage a pre-trained visual-language model BLIP to caption the image and then compare their similarity with the original caption to detect the mismatch\footnote{Here \citet{nguyen2023improving} replaces the corrupted text with their newly generated caption instead of pruning the whole sample, but the high-level idea is similar.}. Rather than consider a sample level mapping, \citet{maini2023t} further looks into the detailed elements in the image. Their strategies remove images whose text inside is the only feature correlated with the caption by using off-the-shell OCR models. Notably, despite its effectiveness, it has a much higher computational cost than our strategy due to calling text detection models. Finally, instead of using existing models, \citet{fang2023data} proposes to train a data filtering network directly on existing high-quality data. 
% \vspace{-1.2em}
\paragraph{Distribution-aware data selection.}
% Filters focused on individual data as mentioned above naturally leads to varying dataset size that are hard to control. Therefore, it is worthwhile to consider the training data distribution in order to select out the most representative and informative data.  There exists many classical coreset selection results such as \cite{wei2015submodularity,raskutti2016statistical,coleman2019selection}.
There exists many classical coreset selection which select out the most representative and informative data by taking data distribution into control, including \citet{wei2015submodularity,raskutti2016statistical,coleman2019selection}. All those works, however, make the assumption that we are under a fixed budget and aims to increase the subset performance reach to the pool performance. 
There also exist some recent distribution-aware selection works for CLIP pretraining. \citet{wang2023too} first trained a codebook in replace of existing pretrained models like BLIP. Then they cluster the samples based on their image corresponding codes and selects a representative subset of samples from each cluster. 
Later \citet{maharana2023d2} considers the example difficulty and data diversity by using
forward and reverse message passing over a constructed
dataset graph.
% \vspace{-1.2em}
\paragraph{Dataset as prior.} 
Neither strategy mentioned above considers the distribution shift in test data. Although such downstream task is unknown in advance, it is possible to estimate via some proxy dataset as prior. This was first proposed in \citet{gadre2023datacomp} relying on sampling image text pairs that are semantically similar to diverse and curated datasets like ImageNet~\cite{deng2009imagenet}. Later \citet{xu2023cit} also use ImageNet as prior but measuring the similarity with both text and meta information. Their work focused on curation instead of subset selection but the high level idea is similar. 
% The potential disadvantage is that such subset will be biased towards those proxy dataset related models. Nevertheless, it is effective in practice, which may suggests that ImageNet is still a good proxy for most existing downstream benchmarks. We also use this in our paper and observe the similar phenomonom.


% \paragraph{Theoretical contrastive learning}
% \yifang{Is it necessary} \yiping{add relevant theoretical work for metric learning?}\yiping{Note that there is no concrete theory for CLIP score?}

\fi
